SNOWMASS Neutrino Frontier NF10 Topical Group Report: Neutrino Detectors

We discuss here future neutrino detectors with physics goals ranging from the eV to the EeV scale. The focus is on future enabling technologies for such detectors, rather than existing detectors or those under construction. The report includes methodologies across the broad spectrum of neutrino physics: liquid noble and other cryogenic detectors, includin LAr and LXe TPCs; photon-based detectors including technologies enabling hybrid Cherenkov/scintillation detectors; low-threshold detectors which use a wide variety of technologies to probe physics like coherent neutrino-nucleus scattering or detection of cosmic background neutrinos; and ultra-high energy detectors including optical and radio detectors, as well as tracking detectors for use at the forward physics facility of the LHC

==> common/defs.tex <==
% This holds definitions of macros to enforce consistency in names.

% This file is the sole location for such definitions.  Check here to
% learn what there is and add new ones only here.  

% also see units.tex for units.  Units can be used here.

%%% Common terms

% Check here first, don't reinvent existing ones, add any novel ones.
% Use \xspace.

\def\expshort{Workshop\xspace}
\def\explong{White Paper on New Opportunities at the Next-Generation Neutrino Experiments\xspace}



\newcommand{\bigo}[1]{\ensuremath{\mathcal{O}(#1)}}


% Things about oscillation
%
\newcommand{\numu}{\ensuremath{\nu_\mu}\xspace}
\newcommand{\nue}{\ensuremath{\nu_e}\xspace}
\newcommand{\nutau}{\ensuremath{\nu_\tau}\xspace}

\newcommand{\anumu}{\ensuremath{\bar\nu_\mu}\xspace}
\newcommand{\anue}{\ensuremath{\bar\nu_e}\xspace}
\newcommand{\anutau}{\ensuremath{\bar\nu_\tau}\xspace}

\newcommand{\dm}[1]{\ensuremath{\Delta m^2_{#1}}\xspace} % example: \dm{12}

\newcommand{\sinst}[1]{\ensuremath{\sin^2\theta_{#1}}\xspace} % example \sinst{12}
\newcommand{\sinstt}[1]{\ensuremath{\sin^22\theta_{#1}}\xspace}  % example \sinstt{12}

\newcommand{\deltacp}{\ensuremath{\delta_{\rm CP}}\xspace}   % example \deltacp
\newcommand{\mdeltacp}{\ensuremath{\delta_{\rm CP}}}   %%%%%%%%%%  <--- missing something; what's the m for?

\newcommand{\nuxtonux}[2]{\ensuremath{\nu_{#1} \to \nu_{#2}}\xspace}  % example \nuxtonux23 (no {...} )
\newcommand{\numutonumu}{\nuxtonux{\mu}{\mu}}
\newcommand{\numutonue}{\nuxtonux{\mu}{e}}
% Add chi sqd MH?  avg delta chi sqd?

% atmospheric neutrinos and PDK
\newcommand{\ptoknubar}{\ensuremath{\rightarrow K^+ \overline{\nu}}\xspace}
\newcommand{\ptoepizero}{\ensuremath{p^+ \rightarrow e^+ \pi^0}\xspace}

% Names of expts or detectors
\newcommand{\cherenkov}{Cherenkov\xspace}
\newcommand{\icecube}{IceCube\xspace}
\newcommand{\tevatron}{Tevatron\xspace}
\newcommand{\kamland}{KamLAND\xspace}
\newcommand{\kkande}{Kamiokande\xspace}  %%%% <---- changed to make shorter
\newcommand{\superk}{Super--Kamiokande\xspace}
\newcommand{\hyperk}{Hyper--Kamiokande\xspace}
\newcommand{\lsnd}{LSND\xspace}
\newcommand{\miniboone}{MiniBooNE\xspace}
\newcommand{\microboone}{MicroBooNE\xspace}
\newcommand{\minerva}{MINER$\nu$A\xspace}
\newcommand{\minosplus}{MINOS+\xspace}
\newcommand{\minos}{MINOS\xspace}
\newcommand{\nova}{NO$\nu$A\xspace}
\newcommand{\coherent}{COHERENT\xspace}
\newcommand{\numi}{NuMI\xspace}
\newcommand{\lariat}{LArIAT\xspace}
\newcommand{\argoneut}{ArgoNeuT\xspace}
\newcommand{\dune}{DUNE\xspace}
\newcommand{\cosine}{COSINE--100\xspace}
\newcommand{\dayabay}{Daya~Bay\xspace}
\newcommand{\bugey}{Bugey\xspace}
\newcommand{\babar}{BaBar\xspace}

% Random
\newcommand{\lartpc}{LArTPC\xspace}
\newcommand{\globes}{GLoBES\xspace}
\newcommand{\larsoft}{LArSoft\xspace}
\newcommand{\snowglobes}{SNOwGLoBES\xspace}
\newcommand{\docdb}{DUNE DocDB\xspace}
\newcommand{\lhc}{LHC\xspace}
% Isotopes
\def\argon40{$^{40}$Ar}  %%%%%       <--- \Ar40 doesn't work; don't know why
\def\Ar39{$^{39}$Ar}
\def\Cl40{$^{40}$Cl}
\def\K40{$^{40}$K}
\def\B8{$^{8}$B}
\newcommand\isotope[2]{\textsuperscript{#2}#1} % use as, e.g.,: \isotope{Si}{28}

% Parameters common to SP DP
\def\fdfiducialmass{\SI{40}{\kt}\xspace}
\def\driftvelocity{\SI{1.6}{\milli\meter/\micro\second}\xspace} % same for sp and dp?
\def\lartemp{\SI{88}\,K\xspace}
\def\larmass{\SI{17.5}{\kt}\xspace} % full mass in cryostat
\def\tpcheight{\SI{12}{\meter}\xspace} % height of SP TPC, APA, CPA and of DP TPC
\def\cryostatht{\SI{14.1}{\meter}\xspace} % height of cryostat
\def\cryostatlen{\SI{62.0}{\meter}\xspace} % height of cryostat
\def\cryostatwdth{\SI{14.0}{\meter}\xspace} % height of cryostat
\def\nominalmodsize{\SI{10}{kt}\xspace} % nominal module size 10 kt

\def\dunelifetime{\SI{20}{years}\xspace} % nominal operational life time of DUNE experiment
\def\beamturnon{{2026}\xspace} % the year we expect beam to turn on
\def\firstfdmodstartinstall{{2022}\xspace} % the year we expect to start install of 1st FD moc
\def\maincavernstartexc{{2019}\xspace} % the year we expect to start cavern excavation
\def\pipiibeampower{\SI{1.2}{MW}\xspace} 


% Parameters SP
\def\spmaxfield{\SI{500}{\volt/\centi\meter}} % SPfield strength
\def\spactivelarmass{\SI{10}{\kt}\xspace} % active mass in cryostat
\def\spmaxdrift{\SI{3.52}{\m}\xspace}
\def\sptpclen{\SI{58}{\meter}\xspace} % length of SP TPC, APA, CPA
\def\apacpapitch{\SI{2.32}{\meter}\xspace} % pitch of SP CPAs and APAs
\def\spfcmodlen{\SI{3.5}{\m}} % length of SP FC module
\def\spnumch{\num{384000}\xspace} % total number of APA readout channels 
\def\spnumpdch{\num{6000}\xspace} % total number of PD readout channels 
\def\planespace{\SI{4.75}{\milli\meter}\xspace}
\def\sptargetdriftvoltpos{\SI{180}{kV}\xspace} % target drift voltage - positive

% Parameters DP
\def\dpactivelarmass{\SI{12.096}{\kt}\xspace} % active mass in cryostat
\def\dpfidlarmass{\SI{10.643}{\kt}\xspace} % fiducial mass in cryostat
\def\dpmaxdrift{\SI{12}{\m}\xspace} % max drift length
\def\dptpclen{\SI{60}{\meter}\xspace} % length of TPC
\def\dptpcwdth{\SI{12}{\meter}\xspace} % width of TPC
\def\dpswchpercrp{\num{36}\xspace} % number of anode/lem sandwiches per CRP 
\def\dpnumswch{\num{2880}\xspace} % total number of anode sandwiches in module
\def\dptotcrp{\num{80}\xspace} % total number of CRPs in module
\def\dpchpercrp{\num{1920}\xspace} %  channels per CRP
\def\dpnumcrpch{\num{153600}\xspace} % total number of CRP channels in module
\def\dpchperchimney{\num{6400}\xspace} %  channels per chimney
\def\dpnumpmtch{\num{720}\xspace} % number of PMT channels
\def\dpstrippitch{\SI{3.125}{\milli\meter}\xspace} % pitch of anode strips
\def\dpnumfcmod{\num{244}\xspace} % number of FC modules
\def\dpnumfcres{\num{240}\xspace} % number of FC resistors
\def\dpnumfcrings{\num{60}\xspace} % number of FC rings
\def\dpnominaldriftfield{\SI{500}{\volt/\cm}\xspace} % nominal drift voltage per cm
\def\dptargetdriftvoltpos{\SI{600}{\kV}\xspace} % target drift voltage - positive
\def\dptargetdriftvoltneg{\SI{-600}{\kV}\xspace} % target drift voltage - negative

% Nominal readout window time
%% SP has 2.25ms drift time.  The readout is 2*dt + 20%*dt extra.
\def\spreadout{\SI{5.4}{\ms}\xspace}
%% DP has 7.5 ms drift time.  The same (over generous) rule gives 16.5ms
\def\dpreadout{\SI{16.4}{\ms}\xspace}
% Supernova Neutrino Burst buffer and readout window time
\def\snbtime{\SI{30}{\s}\xspace}
% interesting amount of time we might have SNB neutrinos but not yet
% enough to trigger.
\def\snbpretime{\SI{10}{\s}\xspace}
% SP SNB dump size. MUST KEEP THIS MANUALLY IN SYNC 1.5 TB/s * \snbtime
\def\spsnbsize{\SI{45}{\TB}\xspace}

% keep these three numerically in sync
\def\offsitepbpy{\SI{30}{\PB/\year}\xspace}
\def\offsitegbyteps{\SI{1}{\GB/\s}\xspace}
\def\offsitegbps{\SI{8}{\Gbps}\xspace}

\def\surffnalbw{\SI{100}{\Gbps}\xspace}
\newcommand{\fnal}{Fermilab\xspace}
\newcommand{\surf}{SURF\xspace}
\newcommand{\bnl}{BNL\xspace}
\newcommand{\anl}{ANL\xspace}

% New from Anne March/April 2018
%physics terms
\newcommand{\efield}{E field\xspace}
\newcommand{\lbl}{long-baseline\xspace}
\newcommand{\Lbl}{Long-baseline\xspace}
\newcommand{\rms}{RMS\xspace} % Might want this small caps?
\newcommand{\threed}{3D\xspace}
\newcommand{\twod}{2D\xspace}

%detectors and modules
\newcommand{\fardet}{Far Detector\xspace}
\newcommand{\detmodule}{detector module\xspace}
\newcommand{\dual}{DP\xspace}
\newcommand{\Dual}{DP\xspace}
\newcommand{\single}{SP\xspace}
\newcommand{\Single}{SP\xspace}
\newcommand{\dpmod}{DP detector module\xspace}
\newcommand{\spmod}{SP detector module\xspace}
\newcommand{\lar}{LAr\xspace}
\newcommand{\lntwo}{LN$_2$\xspace}

% Top-level requirements and specifications
% 1 Minimum drift field
\def\mindriftfield{\SI{250}{\volt/\cm}\xspace}
\def\mindriftfieldgoal{\SI{500}{\volt/\cm}\xspace}
% 2 FE elec noise
\def\elecnoisefe{ \num{1000} enc\xspace}
% 3 light yield
\def\lightyield{\SI{0.5}{pe/\MeV}\xspace}
\def\lightyieldgoal{\SI{5}{pe/\MeV}\xspace}
% 4 time resolution
\def\timeres{\SI{1}{\micro/\second}\xspace}
\def\timeresgoal{\SI{100}{ns}\xspace}
% 5 LAr purity
\def\larpurity{\SI{100}{ppt}\xspace}
\def\larpuritygoal{\SI{30}{ppt}\xspace}
% 6 APA gaps
\def\apagapsame{\SI{15}{\milli\m}\xspace}
\def\apagapdiff{\SI{30}{\milli\m}\xspace}
% 7 drift field uniformity (from component positioning)
\def\fielduniformity{\SI{1}{\%}\xspace}
% 8a APA collection wire angle
\def\apacollwireangle{$\SI{0}{^\circ}$\xspace}
% 8b APA induction wire angle
\def\apainducwireangle{$\pm\SI{35.7}{^\circ}$\xspace}
% 9a APA wire pitch - U,V
\def\uvpitch{\SI{4.669}{\milli\meter}\xspace}
% 9b APA wire pitch - X, G
\def\xgpitch{\SI{4.790}{\milli\meter}\xspace}
% 10 APA wire position tolerance
\def\wirepitchtol{$\pm$\SI{0.5}{\milli\meter}\xspace}
% 11 drift field uniformity (from HVS)
\def\fielduniformityhv{\SI{1}{\%}\xspace}
% 12 HV PS ripple contrib to noise
\def\hvripplenoise{\SI{100}{enc}\xspace}
% 13 FE peaking time
\def\fepeaktime{\SI{1}{\micro\second}\xspace}
% 14 signal saturation level (SP)
\def\spsignalsat{\num{500000} electrons\xspace}
% 15 LAr N contamination
\def\nitrogencontam{\SI{25}{ppm}\xspace}
% 16 detector dead time
\def\deadtime{\SI{0.5}{\%}\xspace}
% Engineering
% 17 Cathode resistivity
\def\cathodemegohm{\SI{1}{\mega\ohm/square}\xspace}
\def\cathodegigohm{\SI{1}{\giga\ohm/square}\xspace}
% 
%\def\{\xspace}
% 19 ADC sampling frequency
\def\samplingfreq{\SI{2}{\mega\hertz}\xspace}
% 20 ADC dynamic range
\def\adcdynrange{\num{12} bits}  %{3000}:\num{1}\xspace}
\def\adcdynrangegoal{\num{13} bits} %{4070}:\num{1}\xspace}
% 21 CE power consumption (SP)
\def\cepower{\SI{50}{mW/channel}\xspace}
% 22 data to tape
\def\dataratetotape{\SI{30}{PB/year}\xspace}
% 23 SNB trigger
\def\snbtriggereff{90\% efficiency\xspace}
%\def\snbtriggervisenergy{90\% efficiency \xspace}
% 24 local E fields
\def\localefield{\SI{30}{\kV/\cm}\xspace}
% 25 non-FE noise contributions
\def\elecnoisenonfe{$\ll$ \SI{1000}{enc}\xspace}
% 26 impurity contrib from components
\def\larpuritycomps{$\ll$ \SI{30}{ppt}\xspace}
% 28 dead channels
\def\deadchannels{\SI{1}{\%}\xspace}


%detector components SP and DP
\newcommand{\dss}{DSS\xspace}
\newcommand{\hv}{high voltage\xspace}
\newcommand{\fcage}{field cage\xspace}
\newcommand{\fc}{FC\xspace}
\newcommand{\fdth}{feedthrough\xspace}
\newcommand{\fcmod}{FC module\xspace}  %%%   don't need?
\newcommand{\topfc}{top FC\xspace}
\newcommand{\botfc}{bottom FC\xspace}
\newcommand{\ewfc}{endwall FC\xspace}
\newcommand{\pdsys}{PD system\xspace}
\newcommand{\phdet}{photon detector\xspace}
\newcommand{\sipm}{SiPM\xspace}
\newcommand{\pmt}{PMT\xspace}
\newcommand{\phel}{photoelectron\xspace}
\newcommand{\pwrsupp}{power supply\xspace}
\newcommand{\pwrsupps}{power supplies\xspace}
\newcommand{\frfour}{FR-4\xspace}

% For interface tables in TDR:  (Brett put in dune.cls instead)
%\newcommand{\citedocdb}[2]{
%\href{http://docs.dunescience.org/cgi-bin/ShowDocument?docid=#1\&version=#2}{DocDB {#1}} \cite{bib:docdb#1}\xspace}  % example of use: \citedocdb{6745}{1}

% The following from phys ch-bsm 1/3/19 (was in their cls file)
\newcommand{\lsim}{{\;\raise0.3ex\hbox{$<$\kern-0.75em\raise-1.1ex\hbox{$\sim$}}\;}}
\newcommand{\gsim}{{\;\raise0.3ex\hbox{$>$\kern-0.75em\raise-1.1ex\hbox{$\sim$}}\;}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\DF}{\Delta_{4}}
\mathchardef\minus="002D
\newcommand{\dk}[1]{\textcolor{red}{#1}}
\newcommand{\dkc}[1]{\textbf{\textcolor{red}{(#1 --DK)}}}
\newcommand{\dd}[1]{\textcolor{blue}{#1}}

% other things
\newcommand{\bsm}{BSM\xspace}
\newcommand{\snowmass}{Snowmass\xspace}

\newcommand\snowmasstitle{\begin{center}\rule[-0.2in]{\hsize}{0.01in}\\\rule{\hsize}{0.01in}\\
\vskip 0.1in Submitted to the  Proceedings of the US Community Study\\ 
on the Future of Particle Physics (Snowmass 2021)\\ 
\rule{\hsize}{0.01in}\\\rule[+0.2in]{\hsize}{0.01in} \end{center}}

%Boschi
\newcommand{\np}[1]{10\textsuperscript{#1}}


==> common/final.tex <==
    % this is added just after end of document

% end stuff from init
%\cleardoublepage
%\renewcommand{\bibname}{References}
\renewcommand{\refname}{References}

\printglossary

%\bibliographystyle{apsrev4-1}
\bibliographystyle{utphys}
% To understand the style chosen, see:
% https://arxiv.org/hypertex/bibstyles/ (very bottom -- additions) and
% https://www.sharelatex.com/learn/Bibtex_bibliography_styles
% July 2017, AH and BV (and AM)

%\begin{multicols}{2}[\printbibheading]
\bibliography{common/tdr-citedb}
%\printbibliography
%\end{multicols}


==> common/glossary.tex <==
% See dune-words.tex for detailed explanation.

% http://mirrors.ctan.org/macros/latex/contrib/glossaries/glossaries-user.pdf

% \usepackage[acronyms,toc]{glossaries}
\usepackage[toc]{glossaries}
\makeglossaries


% for terms with acronyms
\newcommand{\dshort}[1]{\glsentrytext{#1}}
\newcommand{\dshorts}[1]{\glsentryshortpl{#1}}
\newcommand{\dlong}[1]{\glsentrylong{#1}}
\newcommand{\dlongs}[1]{\glsentrylongpl{#1}}

% force the "first time" behavior
\newcommand{\dfirst}[1]{\glsfirst{#1}}
\newcommand{\dfirsts}[1]{\glsfirstplural{#1}}

\newcommand{\dword}[1]{\gls{#1}}
\newcommand{\dwords}[1]{\glspl{#1}}
\newcommand{\Dword}[1]{\Gls{#1}}
\newcommand{\Dwords}[1]{\Glspl{#1}}


% use this to define terms that do NOT have acronyms.
% \newduneword{label}{term}{description}
\newcommand{\newduneword}[3]{
    \newglossaryentry{#1}{
        text={#2},
        long={#2},
        name={\glsentrylong{#1}},
        first={\glsentryname{#1}},
        firstplural={\glsentrylong{#1}\glspluralsuffix},
        description={#3}
    }
}

% use this to define terms that DO have acronyms.
%                 1      2     3       4 
% \newduneabbrev{label}{abbrev}{term}{description}
\newcommand{\newduneabbrev}[4]{
  \newglossaryentry{#1}{
    text={#2},
    long={#3},
    shortplural={{#2}\glspluralsuffix},
    longplural={{#3}\glspluralsuffix{}},
    name={\glsentrylong{#1}{} (\glsentrytext{#1}{})},
    first={\glsentryname{#1}},
    firstplural={\glsentrylong{#1}\glspluralsuffix{} (\glsentrytext{#1}\glspluralsuffix{})},
    description={#4}
  }
}

%% If plural needs special spelling besides adding an "s"
%                 1      2     3       4        5
% \newduneabbrev{label}{abbrev}{term}{terms}{description}
\newcommand{\newduneabbrevs}[5]{
  \newglossaryentry{#1}{
    text={#2},
    long={#3},
    plural={#4},
    shortplural={{#2}\glspluralsuffix},
    longplural={#4},
    name={\glsentrylong{#1}{} (\glsentrytext{#1}{})},
    first={#3 (#2)},
    firstplural={#4 (\glsentrytext{#1}\glspluralsuffix{})},
    description={#5}
  }
}


% tres meta
\newduneword{dword}{DUNE Word}{A term in the DUNE lexicon}

%%%%%%     START ADDING WORDS, IN ALPHABETICAL ORDER IF POSSIBLE!    %%%%%%%%
%near detector
\newduneabbrev{nd}{ND}{near detector}{Refers to the detector(s) %or more  generally the experimental site
 installed close to the neutrino source at \fnal }

%far detector
\newduneabbrev{fd}{FD}{far detector}{Refers to the \fdfiducialmass fiducial mass DUNE detector %or more generally the experimental 
  to be installed at the far site at \surf in
  Lead, SD, to be composed of four \nominalmodsize modules}

%single-phase
\newduneabbrev{sp}{SP}{single-phase}{Distinguishes one of the DUNE far detector technologies by the fact that it operates using argon in its liquid phase only
  %Distinguishes one of the four  \SI{10}{\kton} \glspl{detmodule} of the DUNE far detector by the  fact that it operates using argon in just its liquid phase}
  }

%dual-phase
\newduneabbrev{dp}{DP}{dual-phase}{Distinguishes one of the DUNE far detector technologies by the fact that it operates using argon %Distinguishes one of the four \SI{10}{\kton} \glspl{detmodule} of the DUNE far detector by the fact that it operates using argon 
 in both gas and liquid phases}

%photon detection system
\newduneabbrev{pds}{PDS}{photon detection system}{The detector 
  subsystem sensitive to light produced in the \lar }

%time projection chamber
\newduneabbrev{tpc}{TPC}{time projection chamber}{The portion of each
  DUNE \gls{detmodule} that records ionization electrons
  after they drift away from a cathode through the \lar, and also
  through gaseous argon in a \dual module. 
  The activity is recorded by digitizing the waveforms of current
  induced on the anode as the distribution of ionization charge passes by
  or is collected on the electrode}

%anode plane assembly
\newduneabbrevs{apa}{APA}{anode plane assembly}{anode plane assemblies}{A unit of the \single
  detector module containing the elements sensitive to ionization in the \lar. 
  It contains two faces each of three planes of wires, and interfaces to the cold
  electronics and photon detection system} 

%charge readout
\newduneabbrev{cro}{CRO}{charge readout}{The system for detecting
  ionization charge distributions in a \dual detector module}

%light readout
\newduneabbrev{lro}{LRO}{light readout}{The system for detecting
  scintillation photons in a \dual  detector module}

%safe high voltage
\newduneabbrev{shv}{SHV}{safe high voltage}{Type of bayonet mount
connector used on coaxial cables that has additional insulation 
compared to standard BNC and MHV connectots that makes it safer
for handling high voltage by preventing accidental contact with the
live wire connector in an unmated connector or plug}

%front-end
\newduneabbrev{fe}{FE}{front-end}{The front-end refers a point that is
  ``upstream'' of the data flow for a particular subsystem. 
  For example the front-end electronics is where the cold electronics
  meet the sense wires of the TPC and the front-end DAQ is where the
  DAQ meets the output of the electronics}

\newduneabbrev{daqrou}{RU}{DAQ readout units}{The first element in the data flow of the DAQ.}

\newduneabbrev{cots}{COTS}{commercial off-the-shelf}{Items, typically hardware such as computers, which may be purchased whole, without any custom design or fabrication and thus at normal consumer prices and availability.}


%analog digital converter
\newduneabbrev{adc}{ADC}{analog-to-digital converter}{A sampling of a voltage
  resulting in a discrete integer count corresponding in some way to
  the input}

%data acquisition
\newduneabbrev{daq}{DAQ}{data acquisition}{The data acquisition system
  accepts data from the detector FE electronics, buffers
  the data, performs a \gls{trigdecision}, builds events from the selected
  data and delivers the result to the offline \gls{diskbuffer}}

%detector module
\newduneword{detmodule}{detector module}{The entire DUNE far detector is
  segmented into four modules, each with a nominal \SI{10}{\kton}
  fiducial mass}

%detector unit
\newduneword{detunit}{detector unit}{A \gls{submodule} may be partitioned
  into a number of similar parts. 
  For example the single-phase TPC \gls{submodule} is made up of APA
  units}

%secondary DAQ buffer
\newduneword{diskbuffer}{secondary DAQ buffer}{A secondary
  \dshort{daq} buffer holds a small subset of the full rate as
  selected by a \gls{trigcommand}. 
  This buffer also marks the interface with the DUNE Offline}

%online  monitoring
\newduneabbrev{om}{OM}{online monitoring}{Processes that run inside
  the DAQ on data ``in flight,'' specifically before landing on the
  offline disk buffer, and that provide feedback on the operation of
  the DAQ itself and the general health of the data it is marshalling}

%data quality monitoring
\newduneabbrev{dqm}{DQM}{data quality monitoring}{Analysis of the raw
  data to monitor the integrity of the data and the performance of the
  detectors and their electronics. This type of monitoring may be
  performed in real time, within the \gls{daq} system, or in later
  stages of processing, using disk files as input}

%DAQ dump buffer
\newduneword{dumpbuffer}{DAQ dump buffer}{This \dshort{daq} buffer
  accepts a high-rate data stream, in aggregate, from an associated
  \gls{submodule} sufficient to collect all data likely relevant to
  a potential \gls{snb}}

%Global Trigger Logic
\newduneabbrev{etl}{ETL}{external trigger logic}{Trigger processing
  that consumes \gls{detmodule} level \gls{trignote} information
  and other global sources of trigger input and emits
  \gls{trigcommand} information back to the \glspl{mtl}}

%trigger notification
\newduneword{trignote}{trigger notification}{Information provided by
  \gls{mtl} to \gls{etl} about \gls{trigdecision} its processing}

%trigger primitive
\newduneword{trigprimitive}{trigger primitive}{Information derived by
  the DAQ \gls{fe} hardware that describes a region of space (e.g.,
  one or several neighboring channels) and time (e.g., a contiguous set
  of ADC sample ticks) associated with some activity}

%external trigger candidate
\newduneword{externtrigger}{external trigger candidate}{Information
  provided to the \gls{mtl} about events external to a
  \gls{detmodule} so that it may be considered in forming
  \glspl{trigcommand}}

%Out-of-band trigger command dispatcher
\newduneabbrev{daqoob}{OOB dispatcher}{out-of-band trigger command
  dispatcher}{This component is responsible for dispatching a \gls{snb} dump
  command to all \glspl{daqfer} in the \gls{detmodule}}

%module trigger logic
\newduneabbrev{mtl}{MTL}{module trigger logic}{Trigger processing
  that consumes \gls{detunit} level \gls{trigcommand} information
  and emits \glspl{trigcommand}. 
  It provides the \gls{etl} with \glspl{trignote} and receives back any
  \glspl{externtrigger}}

%octant
\newduneword{octant}{octant}{Any of the eight parts into which 4$\pi$
  is divided by three mutually perpendicular axes. 
  In particular in referencing the value for the mixing angle
  $\theta_{23}$}

%sub-detector ??? %%%%%%%%%%%%%%%%%%%      Why not ``subdet''? (Anne)  %%%%%% ???????
\newduneword{submodule}{subdetector}{A detector unit of granularity less
  than one \gls{detmodule} such as the TPC of either a \single or \dual 
  module}

%trigger candidate
\newduneword{trigcandidate}{trigger candidate}{Summary information derived
  from the full data stream and representing a contribution toward
  forming a \gls{trigdecision}}

%trigger command
\newduneword{trigcommand}{trigger command}{Information derived from
  one or more \glspl{trigcandidate}  that directs elements of the
  \gls{detmodule} to read out a portion of the data stream}

%trigger command message
\newduneabbrev{tcm}{TCM}{trigger command message}{A message flowing
  down the trigger hierarchy from global to local context.  Also see \gls{tpm}}

%trigger decision
\newduneword{trigdecision}{trigger decision}{The process by which
  \glspl{trigcandidate} are converted into \glspl{trigcommand}}

%trigger primitive message
\newduneabbrev{tpm}{TPM}{trigger primitive message}{A message flowing
  up the trigger hierarchy from local to global context.  Also see \gls{tcm}}

\newduneabbrev{ipc}{IPC}{inter-process communication}{A system for software elements to exchange information between threads, local processes or across a data network.  An IPC system is typically specified in terms of protocols  composed of message types and their associated data schema.}

\newduneword{daqdispre}{discovery and presence}{As used in the context of the \gls{ipc}, a system which provides mechanisms for a node on a communication network to learn of the existence of peers and their identity (discovery) as well as determine if they are currently operational or have become unresponsive (presence).}

\newduneabbrev{pubsub}{PUB/SUB}{publish-subscribe communication pattern}{An \gls{ipc} communication pattern where one element, the publisher, sends data to all connected elements, the subscribers.  Each subscriber may connect to multiple publishers.  A variant is PUB/SUB with topics where a subscriber may register an identifier, the topic, to limit the information received to just an associated subset.}

%event builder
\newduneabbrev{eb}{EB}{event builder}{A software agent servicing one
  \gls{detmodule} by executing \glspl{trigcommand} by reading out
  the requested data}

\newduneabbrev{daqdfo}{DFO}{dataflow orchestration}{The process by which trigger commands are executed in parallel and asynchronous manner by the back-end output subsystem of the DAQ.}

% yes, this is a silly name
\newduneabbrev{daqfbi}{FBI}{front-end buffer interface}{The process which provides read-only access to data residing in a front-end's buffers to processes on the network.}

%cluster on board
\newduneabbrev{cob}{COB}{cluster on board}{An ATCA motherboard housing four RCEs}

%reconfigurable computing element
\newduneabbrev{rce}{RCE}{reconfigurable computing element}{Data processor located outside of the cryostat on a \gls{cob} which contains \gls{fpga}, RAM and SSD resources, responsible for buffering data, producing trigger primitives, responding to triggered requests for data and sinking \gls{snb} dumps}

%bump on wire
\newduneabbrev{bow}{BOW}{Bump On Wire}{A working name for the front-end readout computing elements used in the nominal DAQ design to interface the \dual  crates to the DAQ front-end computers}

%advanced telecommunication computing architecture
\newduneabbrev{atca}{ATCA}{Advanced Telecommunications Computing
  Architecture}{An advanced computer architecture specification developed for the telecommunications, military, and aerospace industries that incorporates the latest trends high-speed interconnect technologies, next-generation processors, and improved reliability, availability and serviceability} 

%Micro Telecommunications Computing Architecture
\newduneabbrev{utca}{$\mu$TCA}{Micro Telecommunications Computing Architecture}{The computer architecture specification followed by the crates that house charge and light readout electronics in the dual-phase module} %A computer architecture. Vertical card-edge connectors, Amphenol ICC }%,  \url{https://www.amphenol-icc.com/product-series/micro-tca-card-edge.html}}

%user datagram protocol
\newduneabbrev{udp}{UDP}{user datagram protocol}{A simple,
  connectionless Internet protocol that supports data integrity
  checksums, requires no handshaking, and does not guarantee packet delivery}

%advanced meazzanine card
\newduneabbrev{amc}{AMC}{advanced mezzanine card}{Holds digitizing
  electronics and lives in \gls{utca} crates}

%radio frequency
\newduneabbrev{rf}{RF}{radio frequency}{Electromagnetic emissions
  that are within the (radio) frequency band of sensitivity of the detector
  electronics}

%field programmable gate array
\newduneabbrev{fpga}{FPGA}{field programmable gate array}{An
integrated circuit technology that allows the hardware to be reconfigured to
execute different algorithms after its manufacture and deployment}

\newduneabbrev{fmc}{FMC}{FPGA mezzanine card}{Boards holding FPGA and other integrated circuitry which attach to a motherboard.}

%Front-End Link eXchange
\newduneabbrev{felix}{FELIX}{Front-End Link eXchange}{A
  high-throughput interface between front-end and trigger electronics
  and the standard PCIe computer bus}

%DAQ partition
\newduneword{daqpart}{DAQ partition}{A cohesive and
 coherent collection of DAQ hardware and software working together to trigger and read out some portion of one detector module; it consists of an integral number of \glspl{daqfrag}. 
 Multiple DAQ partitions may operate simultaneously, but each instance operates independently}

%front-end computer
\newduneabbrev{fec}{FEC}{front-end computer}{The portion of one
  \gls{daqpart} that hosts the \gls{daqdr}, \gls{daqbuf} and
  \gls{daqds}.  It hosts the \gls{daqfer} and corresponding portion of the \gls{daqbuf}.}

%DAQ front-end fragment
\newduneword{daqfrag}{DAQ front-end fragment}{The portion of one
  \gls{daqpart} relating to a single \gls{fec} and corresponding to an
  integral number of \glspl{detunit}.  See also \gls{datafrag}}

%data fragment
\newduneword{datafrag}{data fragment}{A block of data read out from a single \gls{daqfrag} that
span a contiguous period of time as requested by a \gls{trigcommand}}

%DAQ front-end redout
\newduneabbrev{daqfer}{FER}{DAQ front-end readout}{The portion of a
  \gls{daqfrag} that accepts data from the detector electronics and
  provides it to the \gls{fec}.}

%DAQ data receiver
\newduneabbrev{daqdr}{DDR}{DAQ data receiver}{The portion of the
  \gls{daqfrag} that accepts data from the \gls{daqfer}, emits
  trigger candidates produced from the input trigger primitives, and
  forwards the full data stream to the \gls{daqbuf}}

%primary DAQ buffer
\newduneabbrev{daqbuf}{primary buffer}{DAQ primary buffer}{The portion
  of the \gls{daqfrag} that accepts full data stream from the
  corresponding \gls{detunit} and retains it sufficiently long for it
  to be available to produce a \gls{datafrag}}

%data selector
\newduneword{daqds}{data selector}{The portion of the \gls{daqfrag}
  that accepts \glspl{trigcommand} and returns the corresponding
  \gls{datafrag}.  Not to be confused with \gls{daqdsn}.}

\newduneword{daqdsn}{data selection}{The process of forming a trigger decision for selecting a subset of detector data for output by the DAQ from the content of the detector data itself.  Not to be confused with \gls{daqds}.}

\newduneabbrev{daqros}{RO}{DAQ readout sub-system}{The sub-system of the DAQ for accepting and buffering data input from detector electronics.}

\newduneabbrev{daqdss}{DS}{DAQ data selection sub-system}{The sub-system of the DAQ responsible for forming a trigger decision based on a portion of the input data stream.  The majority subset of the \gls{daqtrs}.}
\newduneabbrev{daqtrs}{TS}{DAQ trigger sub-system}{The sub-system of the DAQ responsible for forming a trigger decision.}
\newduneabbrev{daqbes}{BE}{DAQ back-end sub-system}{The portion of the DAQ which is generally toward its output end.  It is responsible for accepting and executing trigger commands and marshaling the data they address to output storage buffers.}
\newduneabbrev{daqtss}{TSS}{DAQ timing and synchronization sub-system}{The portion of the DAQ which provides for timing and synchronization to various components.}


%front-end mother board
\newduneabbrev{femb}{FEMB}{front-end mother board}{Refers a unit of
  the \gls{sp} cold electronics that contains the front-end amplifier
  and ADC ASICs covering 128 channels}

%application-specific integrated circuit
\newduneword{asic}{ASIC}{application-specific integrated circuit}

%low voltage
\newduneword{lv}{LV}{low voltage}

%iceberg
\newduneword{iceberg}{ICEBERG}{Integrated Cryostat and Electronics Built for Experimental Research Goals:
a new double wall cryostat build at Fermilab and installed in the Proton Assembly Building meant for 
liquid Argon detector R\&D and for testing of DUNE detector components}

%coldadc
\newduneword{coldadc}{ColdADC}{newly developed 16-channels ASIC providing analog to digital conversion}

%coldata
\newduneword{coldata}{COLDATA}{a 64-channels control and communications ASIC}
%\newduneabbrev{coldata}{COLDATA}{a 64-channel control and communications ASIC}{A key component of the 128-channel \gls{femb} that provides a control and communication interface between cold \gls{lvds} channels and warm electronics external to the cryostat}

%cryo
\newduneword{cryo}{CRYO}{integrated ASIC including front-end circuitry providing signal amplification and pulse shaping, analog to digital conversion, and control and communication functionalities for 64 channels}

%liquid argon application-specific integrated circuit
\newduneword{larasic}{LArASIC}{A 16-channels front-end ASIC that provides signal amplification and pulse shaping}

%complementary metal-oxide-semiconductor
\newduneword{cmos}{CMOS}{Complementary metal-oxide-semiconductor}

%equivalent noise charge
\newduneword{enc}{ENC}{equivalent noise charge}

%equivalent number of bits
\newduneword{enob}{ENOB}{effective number of bits}

%dynamic range enhancement
\newduneword{dre}{DRE}{dynamic range enhancement}

%successive approximation register
\newduneword{sar}{SAR}{successive approximation register}

%protodune
\newduneword{protodune}{ProtoDUNE}{Either of the two DUNE prototype detectors constructed at CERN and operated in
  a CERN test beam (expected fall 2018). 
  One prototype implements \single and the other \dual technology}

%the single-phase ProtoDUNE detector
\newduneword{pdsp}{ProtoDUNE-SP}{The \single ProtoDUNE detector}

%the dual-phase ProtoDune detector
\newduneword{pddp}{ProtoDUNE-DP}{The \dual ProtoDUNE detector}

%WA105 dual-phase demonstrator
\newduneword{wa105}{WA105 DP demonstrator}{The \SI[product-units=power]{3x1x1}{m} WA105 dual-phase prototype detector at CERN}

%data aquisition event block --- includes dirty word: "event"
\newduneword{rawevent}{DAQ event block}{The unit of data output by the
  DAQ. 
  It contains trigger and detector data spanning a unique, contiguous
  time period and a subset of the detector channels.}

%solid-state disk
\newduneabbrev{ssd}{SSD}{solid-state disk}{Any storage device that
  may provide sufficient write throughput to receive, both collectively and
  distributed, the sustained full rate of data from a \gls{detmodule}
  for many seconds}

%high-level trigger --- fixme: this needs improvement
\newduneabbrev{hlt}{HLT}{high-level trigger}{This is actually a filter applied to data which has been triggered and aggregated in order to further reduce or characterize it.}

%particle identification
\newduneabbrev{pid}{PID}{particle ID}{Particle identification}

%readout window
\newduneword{readout window}{readout window}{A fixed, atomic and
  continuous period of time over which data from a \gls{detmodule}, in
  whole or in part, is recorded. 
  This period may differ based on the trigger that initiated the
  readout}

%zero-suppression
\newduneabbrev{zs}{ZS}{zero-suppression}{Used to delete some portion of a
  data stream that does not significantly deviate from zero or
  intrinsic noise levels. 
  It may be applied at different granularity from per-channel to per
  \dword{detunit}}

%run control ------- fixme: maybe another sentence
\newduneabbrev{rc}{RC}{run control}{The system for configuring,
  starting and terminating the DAQ}

\newduneabbrev{daqccm}{CCM}{DAQ control, configuration and monitoring sub-system}{A system for controlling, configuring and monitoring other systems in particular those that make up the DAQ where the CCM encompasses \gls{rc}.}

\newduneword{daqrun}{DAQ run}{A period of time over which relevant data taking conditions and DAQ configuration are asserted to be unchanged. 
  Multiple DAQ runs may occur simultaneously when multiple \glspl{daqpart} are active. 
  This term should not be confused with DUNE experiment or beam ``runs'' which typically span many DAQ runs.}
\newduneword{daqrunnum}{DAQ run number}{A monotonic increasing count which uniquely and globally identifies a \gls{daqrun}.}

%supernova neutrino burst  
\newduneabbrev{snb}{SNB}{supernova neutrino burst}{A prompt 
  increase in the flux of low-energy neutrinos emitted in the first few seconds of a core-collapse supernova.  It can also refer to a trigger command type that may be due to an SNB,
  or detector conditions that mimic its interaction signature}

%supernova burst and low energy
\newduneabbrev{snble}{SNB/LE}{supernova neutrino burst and low
  energy}{Supernova neutrino burst and low-energy physics program}

%supernova early warning system
\newduneabbrev{snews}{SNEWS}{SuperNova Early Warning System}{A global
  supernova neutrino burst trigger formed by a coincidence of SNB
  triggers collected from participating experiments}

%one pulse per second signal
\newduneabbrev{pps}{1PPS signal}{one-pulse-per-second signal}{An
  electrical signal with a fast rise time and that arrives in real
  time with a precise period of one second}

%spill location system
\newduneabbrev{sls}{SLS}{spill location system}{A system residing at
  the DUNE far detector site that provides information, possibly
  predictive, indicating periods of time when neutrinos are being
  produced by the \fnal Main Injector beam spills}

%warm interface board
\newduneabbrev{wib}{WIB}{warm interface board}{Digital electronics
  situated just outside the \single cryostat that receives digital data
  from the FEMBs over cold copper connections and sends it to the RCE
  FE readout hardware}

\newduneabbrev{gps}{GPS}{Global Positioning System}{A satellite-based system that provides a highly accurate \gls{pps} which may be used to synchronize clocks and determine the location.}

\newduneabbrev{ntp}{NTP}{Network Time Protocol}{A networking protocol which allows synchronizing of clocks to within a few \si{\milli\second} of a time standard on a local network and within a few tens of \si{\milli\second} over the Internet.} 

\newduneabbrev{irig}{IRIG}{inter-range instrumentation group}{A standards body which defined a time code standard for transferring timing information.}

%network interfce controller
\newduneabbrev{nic}{NIC}{network interface controller}{Hardware for controlling the interface to a communication network.  Typically, one that obeys the Ethernet protocol}

%warm interface electronics crate
\newduneabbrev{wiec}{WIEC}{warm interface electronics crate}{Crates mounted on the signal flanges that contain the warm interface boards}

%power and timing cards
\newduneabbrev{ptc}{PTC}{power and timing cards}{Cards that provide further processing and distribution of the signals entering and exiting the \single cryostat}

%silicon photomultipler
\newduneabbrev{sipm}{SiPM}{silicon photomultiplier}{A solid-state
  avalanche photodiode sensitive to single \phel signals}

%cryogenic instrumentation and slow control
\newduneabbrev{cisc}{CISC}{cryogenic instrumentation and slow controls}{A DUNE
  consortium responsible for the cryogenic instrumentation and slow controls components}

%consortium
\newduneword{consortium}{consortium}{A unit of organization in the
  DUNE project focused on one major component of the far detector}

%art 
\newduneword{art}{\textit{art}}{A software framework implementing an
  event-based execution paradigm} %http://art.fnal.gov/

%sequential access via metadata  
\newduneabbrev{sam}{SAM}{sequential
  access via metadata}{A data-handling system to store and retrieve
  files and associated metadata, including a complete record of the
  processing that has used the files}

%art data aquisition
\newduneword{artdaq}{\textit{art}DAQ}{A general-purpose \fnal data acquisition framework for distributed data combination and processing. 
It is designed to exploit the parallelism that is possible with
modern multi-core and networked computers}

%big-O notation
\newduneword{order}{$\mathcal{O}(n)$}{of order $n$}

%\newduneword{3d}{3D}{3 dimensional (also 1D, 2D, etc.)} % not phys 
%(Use defs.tex version}
%.........

%beamline
\newduneword{beamline}{beamline}{A sequence of control and monitoring devices used for the formation of a directed collection of particles}
%conceptual design report
\newduneabbrev{cdr}{CDR}{conceptual design report}{A formal project
  document %required by funding agencies
   that describes the experiment
  at a conceptual level}

%conventional facilities
\newduneabbrev{cf}{CF}{conventional facilities}{Pertaining to
  construction and operation of buildings or caverns and conventional infrastructure}

%charge parity
\newduneabbrev{cp}{CP}{charge parity}{Product of charge and parity
  transformations}

%product of charge, parity and time-reversal
\newduneword{cpt}{CPT}{product of charge, parity
  and time-reversal transformations}

%charge-parity symmetry violation
\newduneabbrev{cpv}{CPV}{charge-parity symmetry violation}{Lack of
  symmetry in a system before and after charge and parity
  transformations are applied}

%us department of energy
\newduneword{doe}{DOE}{U.S. Department of Energy}

%deep underground neutrino experiment
\newduneword{dune}{DUNE}{Deep Underground Neutrino Experiment}

%environment, safety and health
\newduneword{esh}{ES\&H}{Environment, Safety and Health}

%fine-grained tracker
\newduneabbrev{fgt}{FGT}{fine-grained tracker}{A near detector module ??}

%far site conventional facilities
\newduneabbrev{fscf}{FSCF}{far site conventional facilities}{The
  \gslpl{cf} at the DUNE far detector site, \surf}
  
%near site conventional facilities
\newduneabbrev{nscf}{NSCF}{near site conventional facilities}{The
  \gslpl{cf} at the DUNE near detector site, \fnal}

%grand unified theory
\newduneabbrev{gut}{GUT}{grand unified theory}{A class of theories that
  unifies the electro-weak and strong forces}

%liquid argon
\newduneabbrev{lar}{LAr}{liquid argon}{The liquid phase of argon}

%liquid argon time-projection chamber
\newduneabbrev{lartpc}{LArTPC}{liquid argon time-projection chamber}{A
  class of detector technology that forms the basis for the DUNE far
  detector modules. 
  It typically entails observation of ionization activity by
  electrical signals and of scintillation by optical signals}

%long-baseline
\newduneabbrev{lbl}{LBL}{long-baseline}{Refers to the distance between the 
  neutrino source  and the far detector.  It can also refer to the distance between the near and far detectors. 
  The ``long'' designation is an approximate and relative distinction. For DUNE, this distance  (between \fnal and \surf) is approximately \SI{1300}{km}}

%long-baseline neutrino facility
\newduneabbrev{lbnf}{LBNF}{Long-Baseline Neutrino Facility}{The
  organizational entity responsible for developing the neutrino beam, the cryostats
  and cryogenics systems, and the conventional facilities for DUNE}

\newduneabbrev{lbnc}{LBNC}{Long-Baseline Neutrino Committee}{The
  organizational entity responsible for overseeing the LBNF and DUNE projects. The committee reports to the \fnal director.}

\newduneabbrev{ncg}{NCG}{Neutrino Cost Group}{The
  organizational entity responsible for reviewing and scrutinizing the DUNE project cost. The committee reports to the \fnal director.}

%mass hierarchy
\newduneabbrev{mh}{MH}{mass hierarchy}{Describes the separation
  between the mass squared differences related to the solar and
  atmospheric neutrino problems}

%fnal main injector
\newduneabbrev{mi}{MI}{\fnal Main Injector}{An accelerator at
  \fnal that provides a beam of high-energy protons that upon
  striking a target produce secondaries that decay to provide the
  neutrinos directed toward the DUNE far detector}

%protons on target
\newduneabbrev{pot}{POT}{protons on target}{Typically used as a unit
  of normalization for the number of protons striking the neutrino
  production target}

%quality assurance
\newduneabbrev{qa}{QA}{quality assurance}{The process by which quality is maintained so as to preserve
high availability and precise function}

%quality control
\newduneabbrev{qc}{QC}{quality control}{A system of maintaining
  quality through testing products against a specification}

%standard model
\newduneabbrev{sm}{SM}{Standard Model}{Refers to a theory describing
  the interaction of elementary particles}

%technical design report
\newduneabbrev{tdr}{TDR}{technical design report}{A formal project
  document %required by funding agencies 
  that describes the experiment at a technical level}

%interim design report
\newduneabbrev{tp}{IDR}{interim design report}{An intermediate
milestone on the path to a full \gls{tdr}} % changed from ``technical proposal'' 6/6/2018

%%%%%%%%%%%%% PROJECT AND PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%
\newduneabbrev{ckm}{CKM matrix}{Cabibbo-Kobayashi-Maskawa
  matrix}{Refers to the matrix describing the mixing between mass and
  weak eigenstates of quarks}

\newduneabbrev{cl}{CL}{confidence level}{Refers to a probability
  used to determine the value of a random variable given its
  distribution}

\newduneabbrev{pmns}{PMNS matrix}{Pontecorvo-Maki-Nakagawa-Sakata
  matrix}{Describes the mixing between mass and weak eigenstates of
  the neutrino}



%%%%%%%%%%%%%%%%%.....................

%%%%%%%%%%%%% PROJECT AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%

% fixme: should not have degenerate definition.  This also should be an abbrev.
%\newduneword{blm}{BLM}{(in Volume 4) beamline measurement (system); (in Volume 3) beam loss monitor} (not used -- yet! Anne 10 May 2018)
%omit trailing period in newduneabbrev(s) and newduneword, glossaries package will append the end of sentence period - Ddm

\newduneabbrevs{cpa}{CPA}{cathode plane assembly}{cathode plane assemblies}{The component of the \single detector module that provides the drift HV cathode}

\newduneabbrev{fc}{FC}{field cage}{The component of a LArTPC that contains and shapes the applied \efield}

\newduneword{cpafc}{CPA/FC}{A pair of \gls{cpa} panels and the top and bottom \gls{fc} portions that attach to the pair; an intermediate assembly for installation into the \gls{spmod} }

\newduneabbrev{topfc}{top FC}{top field cage}{The horizontal portions of the \single FC on the top}

\newduneabbrev{botfc}{bottom FC}{bottom field cage}{The horizontal portions of the \single FC on the bottom}

\newduneabbrev{ewfc}{endwall FC}{endwall field cage}{The vertical portions of the \single FC near the wall}

\newduneabbrev{gp}{GP}{ground plane}{An electrode that is held to be
  electrically neutral relative to Earth ground voltage}

  \newduneword{gg}{ground grid}{An electrode that is held to be
  electrically neutral relative to Earth ground voltage  ??}


\newduneabbrev{alara}{ALARA}{as low as reasonably
  achievable}{Typically used with regard management of radiation
  exposure but may be used more generally. It means making every
  reasonable effort to maintain e.g., exposures, to as far below the
  limits as practical, consistent with the purpose for that the
  activity is undertaken}

\newduneabbrev{ecal}{ECAL}{electromagnetic calorimeter}{A detector
  component that measures energy deposition of traversing particles}

\newduneabbrev{hv}{HV}{high voltage}{Generally describes a voltage
  applied to drive the motion of free electrons through some media}

% can also use in the text: \dword{sp} \dword{detmodule} 
\newduneword{spmod}{SP module}{single-phase detector module}
\newduneword{dpmod}{DP module}{dual-phase detector module}
\newduneword{dsp}{DUNE-SP}{The \single DUNE detector}
\newduneword{ddp}{DUNE-DP}{The \dual DUNE detector}

\newduneabbrev{tcoord}{TC}{technical coordinator}{Responsible for organization of
the project effort. Is a member of the \dword{dune} management team}

\newduneword{tc}{TCn}{technical coordination}

\newduneabbrev{exb}{EB}{executive board}{The highest level DUNE
  decision making body for the collaboration}

\newduneabbrev{tb}{TB}{technical board}{The DUNE organization responsible for
  evaluating technical decisions}

\newduneabbrev{rrb}{RRB}{resource review board}{The organization of DUNE funding agencies responsible for funding decisions}


%%%%%%%%%%%%% PHYSICS AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%

\newduneabbrev{cc}{CC}{charged current}{Refers to an interaction
  between elementary particles where a charged weak force carrier
  ($W^+$ or $W^-$) is exchanged}


\newduneabbrev{dis}{DIS}{deep inelastic scattering}{Refers to
  interaction of an elementary charged particle with a nucleus in an
  energy range where the interaction can be modeled as being with
  individual nucleons}

\newduneabbrev{fsi}{FSI}{final-state interactions}{Refers to
  interactions between elementary or composite particles subsequent to
  the initial, fundamental particle interaction, such as may occur as
  the products exit a nucleus}

\newduneabbrev{geant4}{Geant4}{GEometry ANd Tracking, version 4}{A
  software toolkit for the simulation of the passage of particles
  through matter using Monte Carlo methods}

\newduneabbrev{genie}{GENIE}{Generates Events for Neutrino Interaction
  Experiments}{Software providing an object-oriented neutrino
  interaction simulation resulting in kinematics of the products of
  the interaction}

\newduneabbrev{mc}{MC}{Monte Carlo}{Refers to a method of numerical
  integration that entails the statistical sampling of the integrand
  function. 
  Forms the basis for some types of detector and physics simulations}

\newduneabbrev{qe}{QE}{quasi-elastic}{Refers to interaction between
  elementary particles and a nucleus in an energy range where the
  interaction can be modeled as occurring between constituent quarks
  of one nucleon and resulting in no bulk recoil of the resulting
  nucleus}

%%%%%%%%%%%%%%%%%%%%%%%%% PROJECT VOLUME list for acronyms below %%%%%%%%%%%%%%%

\newduneabbrev{mou}{MoU}{memorandum of understanding}{A document
  summarizing an agreement between two or more parties}

\newduneabbrev{pip2}{PIP-II}{Proton Improvement Plan II}{A plan for
  improving the protons on target delivered for the DUNE neutrino
  production beam. 
  This is revision two of this plan and is planned to be followed by a PIP-III}

\newduneabbrev{sdsta}{SDSTA}{South Dakota Science and Technology
  Authority}{The legal entity that manages the Sanford Underground
  Research Facility, \surf, in Lead, S.D}

\newduneabbrev{wbs}{WBS}{work breakdown structure}{An organizational
  project management tool by which the tasks to be performed are
  partitioned in a hierarchical manner}

%%%%%%%%%%%%%%%%%%%%%%%%% PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%%%%
\newduneabbrev{br}{BR}{branching ratio}{A fractional probability for a
  decay of a composite particle to occur into some specified set or
  sets of products}

\newduneabbrev{dm}{DM}{dark matter}{The term given to the unknown
  matter or force that explains measurements of motion of galaxies
  that are otherwise inconsistent with the amount of mass associated
  with observed amount of photon production}

\newduneabbrev{dsnb}{DSNB}{Diffuse Supernova Neutrino Background}{The
  term describing the pervasive, constant flux of neutrinos due to all
  past supernova neutrino bursts}

\newduneabbrev{globes}{GLoBES}{General Long-Baseline Experiment
  Simulator}{A software package for simulating energy spectra of
  neutrino flux, interaction and measured (after application of some
  model of a detector response) energy spectra}


% are these really used anywhere?
%\newduneword{l/e}{L/E}{length-to-energy ratio}
%\newduneword{lri}{LRI}{long-range interactions}
%\newduneword{solarmass}{$M_{\odot}$}{solar mass}

\newduneabbrev{nc}{NC}{neutral current}{Refers to an interaction
  between elementary particles where a neutrally charged weak force carrier
  ($Z^0$) is exchanged}

\newduneabbrev{nh}{NH}{normal hierarchy}{Refers to the neutrino mass
  eigenstate ordering whereby the sign of the mass squared difference
  associated with the atmospheric neutrino problem is positive}

\newduneabbrev{ih}{IH}{inverted hierarchy}{Refers to the neutrino mass
  eigenstate ordering whereby the sign of the mass squared difference
  associated with the atmospheric neutrino problem is negative}

\newduneabbrev{nsi}{NSI}{nonstandard interactions}{A general class of
  theory of elementary particles other than the Standard Model}

\newduneabbrev{msw}{MSW}{Mikheyev-Smirnov-Wolfenstein effect}{Explains
  the oscillatory behavior of neutrinos produced inside the sun as
  they traverse the solar matter}

% \newduneword{sme}{SME}{Standard-Model Extension}

\newduneabbrev{susy}{SUSY}{supersymmetry}{Theoretical symmetry between a fermion and a boson}

\newduneabbrev{wimp}{WIMP}{weakly-interacting massive particle}{A
  hypothesized particle that may be a component of dark matter}

%%%%%%%%%%%%%%%%%%%%%%%%% DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%%%%

\newduneabbrev{ce}{CE}{cold electronics}{Refers to readout electronics that operate at cryogenic temperatures}

\newduneabbrev{crp}{CRP}{charge-readout plane}{In the \dual technology, a  collection of
  electrodes in a planar arrangement placed at a particular voltage
  relative to some applied \efield such that drifting electrons
  may be collected and their number and time may be measured}

\newduneabbrev{dram}{DRAM}{dynamic random access memory}{A computer memory technology}

% these should be abbrev and maybe combined.
\newduneword{fermilab}{\fnal}{Fermi National Accelerator Laboratory (in Batavia, IL, the Near Site)}
\newduneword{fnal}{FNAL}{see \fnal}


\newduneabbrev{fs}{FS}{full stream}{Relates to a data stream that has not undergone selection, compression or other form of reduction}

\newduneabbrev{lem}{LEM}{large electron multiplier}{A micro-pattern detector suitable for use in ultra-pure argon vapor; LEMs consist of copper-clad PCB boards with sub-millimeter-size holes through which electrons undergo amplification}
%\newduneabbrev{lem}{LEM}{large electron multiplier}{A technique of electron multiplication via avalanche in sub-millimeter-size holes in a
%millimeter-thick printed circuit board where electric fields are understood}
\newduneabbrev{lng}{LNG}{liquefied natural gas}{Pertaining to natural gas in its liquid phase}

% this is pretty generic and isn't referenced.
%\newduneword{mesh}{mesh screen}{A fine mesh screen, glued directly to
%  the steel frame on both sides of each APA in the single-phase TPC,
% creates a uniform ground layer beneath the wire planes}

\newduneabbrev{mip}{MIP}{minimum ionizing particle}{Refers to a
  momentum traversing some medium such that the particle is losing
  near the minimum amount of energy per distance traversed} % some \mip and some \dword{mip}. If time, rectify. ??

%\newduneword{abc}{MTS}{Materials Test Stand}
%\newduneword{muid}{MuID}{muon identifier (detector)}

%\newduneword{abc}{OPERA}{Oscillation Project with Emulsion-Racking Apparatus (experiment at LNGS)}
%\newduneword{abc}{NND}{(used only in Volume 4 Chapter 7) near neutrino detector, same as ND}
%\newduneword{abc}{OD}{outer diameter}

% there is also pds
\newduneabbrev{pd}{PD}{photon detector}{Refers to the detector
  elements involved in measurement of number and arrival times of
  optical photons produced in a detector module} %volume}

\newduneabbrev{pmt}{PMT}{photomultiplier tube}{A device that makes use
  of the photoelectric effect to produce an electrical signal from the
  arrival of optical photons}

\newduneabbrev{ppm}{ppm}{parts per million}{A number equal to $10^{-6}$}
\newduneabbrev{ppb}{ppb}{parts per billion}{A number equal to $10^{-9}$}
\newduneabbrev{ppt}{ppt}{parts per trillion}{A number equal to $10^{-12}$}

\newduneword{rio}{RIO}{reconfigurable input output}

\newduneword{rpc}{RPC}{resistive plate chamber}
\newduneword{s/n}{S/N}{signal-to-noise (ratio)}
\newduneword{ssp}{SSP}{SiPM signal processor}
\newduneword{sbn}{SBN}{Short-Baseline Neutrino program (at \fnal)}
\newduneword{stt}{STT}{straw tube tracker}
%\newduneword{abc}{SURF (also Sanford Lab)}{Sanford Underground Research Facility (in Lead, SD, the Far Site)}
\newduneword{tr}{TR}{transition radiation}
%\newduneword{abc}{W}{Watt (also mW, kW, MW) }
%\newduneword{abc}{WA105}{Single-Phase LArTPC and the Long Baseline Neutrino Observatory Demonstration}
\newduneword{wire board}{wire board}{At the head end of the APA in the \single TPC, stacks of electronics boards referred to as ``wire boards'' are arrayed to anchor the wires.  They also provide the connection between the wires and the cold electronics} %?? long for a word. ??

\newduneabbrev{wls}{WLS}{wavelength shifting}{A material or process by
  which incident photons are absorbed by a material and photons are
  emitted at a different, typically longer, wavelength}

\newduneabbrev{tpb}{TPB}{tetra-phenyl butadiene}{A type of wavelength shifting material}

\newduneabbrev{sft}{SFT}{signal feedthrough}{A cryostat penetration allowing for the passage of cables or other extended parts}
\newduneabbrev{sftchimney}{SFT chimney}{signal feedthrough chimney}{In the \dual technology, a volume above the cryostat penetration used for a signal feedthrough}


\newduneword{catiroc}{CATIROC}{charge and time integrated readout chip}

\newduneabbrev{wr}{WR}{White Rabbit}{A component of the timing system that forwards clock signal and time-of-day reference data to the master timing unit}

\newduneabbrev{mch}{MCH}{MicroTCA Carrier Hub}{An network switching device}

\newduneabbrev{wrmch}{WR-MCH}{White Rabbit \gls{utca} Carrier Hub}{add def} %??

\newduneword{cmp}{CMP}{configuration management plan}

\newduneword{qap}{QAP}{quality assurance plan} %{A project management device for planning \gls{qa}}

\newduneword{ieshp}{IESHP}{integrated environmental, safety and health plan}%{Refers to the LBNF/DUNE project planning instrument}

\newduneword{dmp}{DMP}{data management plan} %{A project management device to state how the experimental data will be managed}

\newduneword{qam}{QAM}{quality assurance manager} %{The manager of \gls{qa} for the LBNF/DUNE project}

\newduneabbrev{dss}{DSS}{detector support system}{The system used to support the \single detector within the cryostat}

\newduneabbrev{itf}{ITF}{integration and test facility}{A facility where various detector components will be tested prior to installation}

\newduneabbrev{tco}{TCO}{temporary construction opening}{An opening in the side of a cryostat through which detector elements are brought into the cryostat; utilized during construction and installation}

\newduneabbrev{sit}{SIT}{surface installation team}{An organizational unit responsible for logistics and integration in South Dakota}

\newduneabbrev{uit}{UIT}{underground installation team}{An organizational unit responsible for installation in the underground area at the \surf site}

\newduneabbrev{cmgc}{cmgc}{construction manager/general contractor}{The organizational unit responsible for management of the construction of conventional facilities at the underground area at the \surf site}

\newduneabbrev{pdr}{PDR}{preliminary design review}{A project management device by which an early design is reviewed}
\newduneabbrev{fdr}{FDR}{final design review}{A project management device by which a final design is reviewed}
\newduneabbrev{prr}{PRR}{production readiness review}{A project management device by which the production readiness is reviewed}
\newduneabbrev{orr}{ORR}{operational readiness review}{A project management device by which the operational readiness is reviewed}
\newduneabbrev{ppr}{PPR}{production progress review}{A project management device by which the progress of production is reviewed}
\newduneabbrev{edms}{EDMS}{engineering document management system}{A computerized system developed at CERN by which documents, drawings and models are managed}

\newduneword{wrgm}{WR grandmaster}{White Rabbit grandmaster}


%%%%% Software and computing %%%%

\newduneword{larsoft}{\larsoft}{Liquid Argon Software (\larsoft),  a shared base of physics software across \lartpc experiments}
\newduneword{nova}{\nova}{The \nova off-axis neutrino oscillation experiment at \fnal }
\newduneword{minerva}{\minerva}{The \minerva neutrino cross sections experiment at \fnal }
\newduneword{microboone}{\microboone}{The \lartpc-based \microboone neutrino oscillation experiment at \fnal }
\newduneword{wirecell}{wire-cell}{A tomographic automated \threed neutrino event reconstruction method for \lartpc{}s}
\newduneword{ftslite}{F-FTS-lite}{Light-weight version of the \fnal File Transfer system used for rapid data transfers out of the online systems}
\newduneword{fts}{FTS}{File Transfer System developed at \fnal to catalog and move data to permanent storage}

%%% new ones that I haven't categorized (Anne)
\newduneword{35t}{35 ton prototype}{The 35 ton prototype cryostat and \gls{sp} detector built at \fnal before the \gls{protodune} detectors}

\newduneabbrev{cuc}{CUC}{central utility cavern}{The central underground cavern  containing utilities such as central cryogenics and other systems, and the underground data center and control room}
\newduneabbrev{cfd}{CFD}{computational fluid dynamics}{High performance computer-assisted modeling of fluid dynamical systems}
\newduneword{vuv}{VUV}{vacuum ultra-violet}
\newduneword{tallbo}{TallBo}{A cylindrical cryostat at \fnal primarily used for developing scintillation light collection technologies for \lartpc detectors}

\newduneabbrev{eos}{EOS}{EOS}{The XRootD based distributed file system developed by CERN}
\newduneabbrev{ehn1}{EHN1}{Experiment Hall North One}{Location at CERN of the ProtoDUNE experiments}
\newduneword{led}{LED}{Light-emitting diode}
\newduneword{rtd}{RTD}{Cryostat level and temperature monitoring devices}
\newduneword{swc}{SWC}{Software \& Computing}
\newduneabbrev{las}{LAS}{LEM-anode Sandwich}{In the \dual technology, a \gls{lem} and its corresponding anode are mounted together in a module called a LEM-anode sandwich}

\newduneword{roi}{ROI}{region of interest}
\newduneword{hpc}{HPC}{high-performance computing facilities; generally computing facilities emphasizing parallel computing with aggregate power of more than a teraflop}


\newduneword{comfund}{common fund}{The shared resources of the collaboration}
\newduneabbrev{ims}{IMS}{integrated master schedule}{A project management device consisting of linked tasks and milestones}

\newduneword{hvdb}{HVDB}{dual-phase HV divider board}
\newduneword{sas}{SAS}{A pass-through chamber used to ensure safe transfer of materials, avoiding contamination in both directions}

\newduneword{fea}{FEA}{finite element analysis}

\newduneword{fss}{FSS}{field shaping strips}
\newduneword{lvds}{LVDS}{low-voltage differential signaling}


%electrostatic discharge
\newduneword{esd}{ESD}{electrostatic discharge}%{ESD is the sudden flow of electricity between two electrically charged objects caused by contact, an electrical short, or dielectric breakdown. ESD can cause failure of electronic components such as integrated circuits}

\newduneabbrev{rp}{RP}{resistive panel}{Resistive panels form the constant potential surfaces for a \gls{spmod} \gls{cpa}; they are composed of a thin layer of carbon-impregnated Kapton and laminated to both sides of a \frfour sheet. }

\newduneword{uhmwpe}{UHMWPE}{ultra-high molecular weight polyethylene}

\newduneword{cts}{CTS}{Cryogenic Test System}
\newduneword{plc}{PLC}{programmable logic controller}

\newduneword{mppc}{MPPC}{\SI{6}{mm}$\times$\SI{6}{mm} Multi-Pixel Photon Counters produced by Hamamatsu\texttrademark{} Photonics K.K.}

\newduneabbrev{sfp}{SFP}{small form-factor pluggable (SFP)}{a particular standard for optical transceivers}

\newduneabbrev{minipod}{MiniPOD}{miniature parallel optical device}{a family of types of multi-channel optical transceivers}

\newduneword{ccc}{CCC}{configuration change command}
\newduneword{act}{ACT}{activation time stamp}
\newduneword{lcm}{LCM}{light calibration module}
\newduneword{lpm}{LPM}{light pulser module}
\newduneword{dac}{DAC}{digital-to-analog converter}
\newduneword{sarapu}{S-ARAPUCA}{add def}
\newduneword{xarapu}{X-ARAPUCA}{add def}
\newduneword{feb}{FEB}{front-end board}

==> common/init_orig.tex <==
% This should be \input first thing after \begin{document}

\pagestyle{titlepage}

\date{}

\title{\scshape\Large Snowmass Neutrino Frontier: \\
NFxx Topical Group Report\\
%\vspace{5mm}
\normalsize Description of TG here
\vskip -10pt
\snowmasstitle
}


%\vspace{10mm}

\renewcommand\Authfont{\scshape\small}
\renewcommand\Affilfont{\itshape\footnotesize}

%Authors go here with affiliation indexed by [X]
\author[1]{A.~One$^{\thanks{Lead Editors}}$}
\author[* 2]{A.~Two}
\author[* 3]{A.~Three}
\author[* 4]{A.~Four}

\author[5]{Other Authors}


\vspace{-0.5cm}
%Affiliations go here
\affil[1]{U1, New York, NY 10027}
\affil[2]{U2, Chicago, IL 60616}
\affil[3]{L3, Batavia, IL, USA}
\affil[4]{U4, Cincinnati, OH, USA}

\affil[5]{Other Affilliations}

\maketitle

\renewcommand{\familydefault}{\sfdefault}
\renewcommand{\thepage}{\roman{page}}
\setcounter{page}{0}

\pagestyle{plain} 
\clearpage
\textsf{\tableofcontents}

%\textsf{\listoffigures}
%\clearpage

%\textsf{\listoftables}
%\clearpage

%For acronym list to appear just after TOC, TOF, TOT
%\printnomenclature
%\clearpage

%\iffinal\else
%\textsf{\listoftodos}
%\clearpage
%\fi

\renewcommand{\thepage}{\arabic{page}}
\setcounter{page}{1}

\pagestyle{fancy}

% Set how header/footers look
%\newcommand{\chaptermark}[1]{%
%\markboth{Chapter \thechapter:\# 1}{}}
%\renewcommand{\chaptermark}[1]{%
%\markboth{Chapter \thechapter:\ #1}{}}
\fancyhead{}
%\fancyhead[RO,LE]{\textsf{\footnotesize \thepage}}
\fancyhead[RO]{\textsf{\footnotesize \thepage}}
%\fancyhead[LO,RE]{\textsf{\footnotesize \rightmark}}
\fancyhead[LO]{\textsf{\footnotesize \rightmark}}

\fancyfoot{}
\fancyfoot[RO]{\textsf{\footnotesize Snowmass 2021}}
\fancyfoot[LO]{\textsf{\footnotesize NFxx Topical Group Report}}
\fancypagestyle{plain}{}

\renewcommand{\headrule}{\vspace{-4mm}\color[gray]{0.5}{\rule{\headwidth}{0.5pt}}}

% Not all main documents have any citations.
% When not built in "final" mode, add in one citation just to let the
% document build.
% If, after substantial editing a main document still lacks any
% citations then it should have its whole bibliography removed.
%\ifdefined\isfinal\nocite{}\else\nocite{CD0}\fi
%\nocite{nothing}


% see also preamble.tex
%\input{common/acronyms}



==> common/preamble.tex <==
% stuff before document begins.  

% Most packages are required through dune.cls.  Put hyper-ref related here to assure it's last.
%%% xr won't play nice
% \usepackage{xr-hyper}
\usepackage[pdftex,bookmarks,hidelinks]{hyperref}
\nonfrenchspacing
%\frenchspacing

\usepackage[utf8]{inputenc}
\usepackage{multicol}
\RequirePackage{cite}

%\usepackage{subfigure}

\graphicspath{ {/graphics/} }

\let\OLDthebibliography\thebibliography
\renewcommand\thebibliography[1]{
  \OLDthebibliography{#1}
  \setlength{\parskip}{0pt}
  \setlength{\itemsep}{0pt plus 0.3ex}
}

% make some "if"s for DP and SP.
% They should be set true inside DP or SP volume or chapter mains.
% set try like \dptrue or \sptrue.
% they can be referenced with \ifdp or \ifsp and terminated with \fi.
\newif\ifdp
\newif\ifsp

\input{common/defs.tex}
\input{common/units.tex}
\input{generated/parameters.tex}
%\input{generated/reqdefs.tex}

% For abbrev/acronym lists, see also init.tex for entry point of acronyms.tex.
% \usepackage[intoc]{nomencl}
% \makenomenclature
% \renewcommand{\nomname}{Acronyms, Abbreviations and Terms}
% \setlength{\nomlabelwidth}{0.2\textwidth}

% For glossaries, needs to be loaded *after* hyperref to get clickable links.
\input{common/glossary}

% Do this here to make use of the experiment name and title macro
\hypersetup{
    pdftitle={\expshort TDR \thedocsubtitle},
    pdfauthor={\expshort Collaboration},
    final=true,
    colorlinks=false,
    linktocpage=true,
    linkbordercolor=blue,
    citebordercolor=green,
    urlbordercolor=magenta,
    filecolor=black,
    pdfpagemode=UseOutlines,
    pdfborderstyle={/S/U},  
}





==> common/units.tex <==
% This holds definitions of macros to enforce consistency in units.

% This file is the sole location for such definitions.  Check here to
% learn what there is and add new ones only here.  

% also see defs.tex for names.


% see
%  http://ctan.org/pkg/siunitx
%  http://mirrors.ctan.org/macros/latex/contrib/siunitx/siunitx.pdf

% Examples:
%  % angles
%  \ang{1.5} off-axis
%
%  % just a unit
%  \si{\kilo\tonne}
%
%  % with a value:
%  \SI{10}{\mega\electronvolt}

%  range of values:
% \SIrange{60}{120}{\GeV}

% some shorthand notation
%\DeclareSIUnit \MBq {\mega\Bq}
\DeclareSIUnit \s {\second}
\DeclareSIUnit \MB {\mega\byte}
\DeclareSIUnit \GB {\giga\byte}
\DeclareSIUnit \TB {\tera\byte}
\DeclareSIUnit \PB {\peta\byte}
\DeclareSIUnit \Mbps {\mega\bit/\s}
\DeclareSIUnit \Gbps {\giga\bit/\s}
\DeclareSIUnit \Tbps {\tera\bit/\s}
\DeclareSIUnit \Pbps {\peta\bit/\s}
\DeclareSIUnit \kton {\kilo\tonne} % changed  back to kton
\DeclareSIUnit \kt {\kilo\tonne}
\DeclareSIUnit \Mt {\mega\tonne}
\DeclareSIUnit \eV {\electronvolt}
\DeclareSIUnit \keV {\kilo\electronvolt}
\DeclareSIUnit \MeV {\mega\electronvolt}
\DeclareSIUnit \GeV {\giga\electronvolt}
\DeclareSIUnit \PeV {\peta\electronvolt}
\DeclareSIUnit \EeV {\exa\electronvolt}
\DeclareSIUnit \m {\meter}
\DeclareSIUnit \cm {\centi\meter}
\DeclareSIUnit \in {\inchcommand}
\DeclareSIUnit \km {\kilo\meter}
\DeclareSIUnit \kV {\kilo\volt}
\DeclareSIUnit \kW {\kilo\watt}
\DeclareSIUnit \MW {\mega\watt}
\DeclareSIUnit \MHz {\mega\hertz}
\DeclareSIUnit \mrad {\milli\radian}
\DeclareSIUnit \year {year}
\DeclareSIUnit \POT {POT}
\DeclareSIUnit \sig {$\sigma$}
\DeclareSIUnit\parsec{pc}
\DeclareSIUnit\lightyear{ly}
\DeclareSIUnit\foot{ft}
\DeclareSIUnit\ft{ft}
\DeclareSIUnit \ppb{ppb}
\DeclareSIUnit \ppt{ppt}
\DeclareSIUnit \samples{S}

% for a bare kt-year
\def\ktyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\kt\year}\xspace}
\def\Mtyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\Mt\year}\xspace}
\def\msr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\meter\steradian}\xspace}
\def\ktMWyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\kt\MW\year}\xspace}

% used for hyphen, obsolete now: \newcommand{\SIadj}[2]{\SI[number-unit-product = -]{#1}{#2}}
% change command definition Nov 2017 in case people copy e.g., \ktadj from CDR text.
% E.g., \ktadj{10} now renders the same as \SI{10}{\kt}
\newcommand{\SIadj}[2]{\SI{#1}{#2}}

% Adjective form of some common units (Nov 2107 changed to be same as normal form, no hyphen)
% "the 10-kt detector"

\newcommand{\ktadj}[1]{\SIadj{#1}{\kt}}
% "the 1,300-km baseline"
\newcommand{\kmadj}[1]{\SIadj{#1}{\km}}
% "a 567-keV endpoint"
\newcommand{\keVadj}[1]{\SIadj{#1}{\keV}}
% "Typical 20-MeV event"
\newcommand{\MeVadj}[1]{\SIadj{#1}{\MeV}}
% "Typical 2-GeV event"
\newcommand{\GeVadj}[1]{\SIadj{#1}{\GeV}}
% "the 1.2-MW beam"
\newcommand{\MWadj}[1]{\SIadj{#1}{\MW}}
% "the 700-kW beam"
\newcommand{\kWadj}[1]{\SIadj{#1}{\kW}}
% "the 100-tonne beam"
\newcommand{\tonneadj}[1]{\SIadj{#1}{\tonne}}
% "the 4,850-foot depth beam"
\newcommand{\ftadj}[1]{\SIadj{#1}{\ft}}
%

% Mass exposure, people like to put dots between the units
% \newcommand{\ktyr}[1]{\SI[inter-unit-product=\ensuremath{{}\cdot{}}]{#1}{\kt\year}}
% must make usage of \ktyr above consistent with this one before turning on

% Beam x mass exposure, people like to put dots between the units
\newcommand{\ktmwyr}[1]{\SI[inter-unit-product=\ensuremath{{}\cdot{}}]{#1}{\kt\MW\year}}


==> expanded_authorlist.tex <==
\newcommand{\Editor}{Editor.}
\newcommand{\Contributor}{Primary Contributor.}
%% Do not edit above this line!
%%============================================
%%=========== Instructions ===================
% 1) Add a “newcommand" for any new affiliation in the first block of commands below, please make sure it is added in alphabetical order of institution's name. Can be skipped only if the affiliation already exists.

% 2) Add an \affiliation directive in the same alphabetical order as in 1) to the second block of commands below. Can be skipped only if the affiliation already exists.

% 3) Add author(s) with affiliation(s) in alphabetical order of the author's last name to the 3rd block of commands. 
% 4) Press the “Recompile” button and make sure you see an author list and the authors and affiliations you entered. If not, look through your changes, fix any errors, and recompile again.
%%=========== End of Instructionsش =============

%Authors go here with affiliation indexed by [X]
% 1st Block of Commands
%Please enter a newcommand per affiliation, please make sure they are entered in alphabetical order of institution name. 
\newcommand{\UA}{University at Albany, State University of New New York (SUNY), Albany, NY USA}
\newcommand{\ANL}{Argonne National Laboratory, IL, USA}
\newcommand{\APC}{Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\newcommand{\Atlantico}{Universidad del Atl\'antico, Puerto Colombia, Atl\'antico, Colombia}
\newcommand{\UBERN}{Universt\"at Bern, Bern, Switzerland}
\newcommand{\BEU}{Beykent University, Istanbul, Turkey}
\newcommand{\BU}{Boston University, Boston, MA, USA}
\newcommand{\BNL}{Brookhaven National Laboratory, NY, USA}
\newcommand{\BHU}{Banaras Hindu University, Varanasi, INDIA}
\newcommand{\UoBham}{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\newcommand{\UB}{University of Bristol, Bristol BS8 1TL, United Kingdom}
\newcommand{\UoB}{University of Bucharest, Bucharest, Romania}
\newcommand{\Caltech}{California Institute of Technology, Pasadena, CA, USA}
\newcommand{\UCB}{University of California, Berkeley, Berkeley, CA USA}
\newcommand{\UCD}{University of California, Davis, Davis, CA USA}
\newcommand{\UNC}{University of North Carolina, Chapel Hill, NC USA}
\newcommand{\UCI}{University of California, Irvine, CA, USA}
\newcommand{\JGU}{Johannes Gutenberg University, Mainz, Germany}
\newcommand{\UCSB}{University of California, Santa Barbara, Santa Barbara, CA USA}
\newcommand{\Cambridge}{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\newcommand{\Catania}{University and INFN Sezione di Catania, Catania, Italy}
\newcommand{\CERN}{CERN, 1 Esplanade des Particules, Geneva, Switzerland}
\newcommand{\CIEMAT}{CIEMAT, Centro de Investigaciones Energéticas, Medioambientales y Tecnólogicas, Madrid, Spain}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH, USA}
\newcommand{\CUSB}{Central University of South Bihar, Gaya, INDIA}
\newcommand{\Cinvestav}{Centro de Investigación y de Estudios Avanzados del Instituto Politécnico Nacional (Cinvestav), Mexico City, Mexico}
\newcommand{\Columbia}{Columbia University, New York, NY, USA}
\newcommand{\CSU}{Colorado State University, Fort Collins, CO, USA}
\newcommand{\Duke}{Duke University, Durham, NC, USA}
\newcommand{\Drexel}{Drexel University, Philadelphia, PA, USA}
\newcommand{\EDI}{University of Edinburgh, Edinburgh EH8 9YL, United Kingdom}
\newcommand{\EIA}{Universidad EIA, Envigado, Antioquia, Colombia}
\newcommand{\FCUL}{Faculdade de Ci\^{e}ncias da Universidade de Lisboa, Lisboa, Portugal}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory, Batavia, IL, USA}
\newcommand{\UF}{University of Florida, Gainesville, FL 32611, USA}
\newcommand{\UGR}{University of Granada \& CAFPE, Granada, Spain}
\newcommand{\Harvard}{Harvard University, Cambridge, MA, USA}
\newcommand{\Hawaii}{University of Hawaii, Honolulu, HI, USA}
\newcommand{\Houston}{University of Houston, Houston, TX, USA}
\newcommand{\ISU}{Idaho State University, Pocatello, ID, USA} 
\newcommand{\IU}{Indiana University, Bloomington, IN, USA} 
\newcommand{\IFIC}{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Paterna, Spain}
\newcommand{\IIT}{Illinois Institute of Technology, Chicago, IL, USA}
\newcommand{\IITH}{Indian Institute of Technology Hyderabad, Kandi, Sangareddy, India}
\newcommand{\CzechAcademyofSciences}{Institute of Physics, Czech Academy of Sciences, 182 00 Prague 8, Czech Republic}
\newcommand{\INFNMi}{Istituto Nazionale di Fisica Nucleare, Sezione di Milano, Milano, Italy}
\newcommand{\INFNMiB}{Istituto Nazionale di Fisica Nucleare, Sezione di Milano Bicocca, Milano, Italy}
\newcommand{\INFNGE}{Istituto Nazionale di Fisica Nucleare, Sezione di Genova, Genova, Italy}
\newcommand{\INFNNA}{Universit\`a degli Studi di Napoli ``Federico II'' \& Istituto Nazionale di Fisica Nucleare, Sezione di Napoli, Napoli, Italy}
\newcommand{\Insubria}{Universit{\`a} degli Studi dell'Insubria, Dipartimento di Scienza e Alta Tecnologia, Como, Italy}
\newcommand{\UOH}{University of Hyderabad, Hyderabad - 500046, India}
\newcommand{\Iowa}{University of Iowa, Iowa City, IA, USA}
\newcommand{\ISP}{Instituto Superior Técnico, Lisbon, Portugal}
\newcommand{\IowaU}{Iowa State University, Ames, IA, USA}
\newcommand{\Irfu}{IRFU, CEA Saclay, Gif-sur-Yvette, France}
\newcommand{\Iwate}{Iwate University, Morioka, Iwate, Japan}
\newcommand{\JBNU}{Jeonbuk National University, Jeonju, Jeonbuk, Korea}
\newcommand{\KSU}{Kansas State University, Manhattan, KS, USA}
\newcommand{\Kyiv}{Taras Shevchenko National University of Kyiv, 01601 Kyiv, Ukraine}
\newcommand{\NRCKI}{National Research Center Kurchatov Institute, Moscow, Russian Federation}
\newcommand{\JSU}{Jackson State University, Jackson, MS, USA}
\newcommand{\jnu}{Jawaharlal Nehru University, New Delhi 110067,  India}
\newcommand{\JU}{University of Jammu, J$\&$K, India}
\newcommand{\Lancaster}{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\newcommand{\LBNL}{Lawrence Berkeley National Laboratory, Berkeley, CA USA}
\newcommand{\LLNL}{Lawrence Livermore National Laboratory, Livermore, CA USA}
\newcommand{\Liverpool}{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\newcommand{\LANL}{Los Alamos National Laboratory, Los Alamos, NM, USA}
\newcommand{\LIP}{Laboratório de Instrumentação e Física Experimental de Partículas, Lisboa and Coimbra, Portugal}
\newcommand{\LSU}{Louisiana State University, Baton Rouge, LA, USA}
\newcommand{\Lucknow}{University of Lucknow, Lucknow, Uttar Pradesh, India}
\newcommand{\MIT}{Massachusetts Institute of Technology, Cambridge, MA, USA}
\newcommand{\MPA}{Max Planck Institute for Astrophysics, Garching, Germany}
\newcommand{\UMN}{University of Minnesota, Minneapolis, MN, USA}
\newcommand{\MSU}{Michigan State University, East Lansing, MI, USA}
\newcommand{\Duluth}{University of Minnesota Duluth, Duluth, MN, USA}
\newcommand{\UMiss}{University of Mississippi, University, MS, USA}
\newcommand{\UCNCl}{Universidad Católica del Norte, Antofagasta, Chile}
\newcommand{\UND}{University of North Dakota, Grand Forks, ND, USA}
\newcommand{\Manchester}{University of Manchester, Manchester M13 9PL, United Kingdom}
\newcommand{\ND}{University of Notre Dame, Notre Dame, IN USA}
\newcommand{\UNSPMF}{University of Novi Sad, Faculty of Sciences, Novi Sad, Serbia}
\newcommand{\OakRidge}{Oak Ridge National Laboratory, Oak Ridge, TN, USA}
\newcommand{\OSU}{Ohio State University, Columbus, OH, USA}
\newcommand{\OregonState}{Oregon State University, Corvallis, OR, USA}
\newcommand{\Oxford}{University of Oxford, Oxford, UK}
\newcommand{\PNNL}{Pacific Northwest National Laboratory, Richland, WA, USA}
\newcommand{\UTF}{Universidade Tecnológica Federal do Paraná, Curitiba, PR, Brazil}
\newcommand{\UniPR}{University of Parma, Department of Engineering and Architecture, Parma, Italy}
\newcommand{\Pennsylvania}{Pennsylvania State University, University Park, PA, USA}
\newcommand{\Penn}{University of Pennsylvania, Phildelphia, PA, USA}
\newcommand{\Pisa}{University and INFN Sezione di Pisa, Pisa, Italy}
\newcommand{\Princeton}{Princeton University, Princeton, NJ, USA}
\newcommand{\PAU}{Punjab Agricultural University, Ludhiana, India}
\newcommand{\QMUL}{Queen Mary University of London, London E1 4NS, United Kingdom}
\newcommand{\Rochester}{University of Rochester, Rochester, NY, USA}
\newcommand{\Rutgers}{Rutgers University, Piscataway, NJ, USA}
\newcommand{\SJSU}{San Jos\'{e} State University, San Jos\'{e}, CA, USA}
\newcommand{\Sheffield}{University of Sheffield, Department of Physics and Astronomy, Sheffield S3 7RH, United Kingdom}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Stanford University, Menlo Park, CA, USA}
\newcommand{\SDSMT}{South Dakota School of Mines and Technology, Rapid City, SD, USA}
\newcommand{\SMU}{Southern Methodist University, Dallas, TX, USA}
\newcommand{\SU}{Stockholm University, Stockholm, Sweden}
\newcommand{\SBU}{Stony Brook University, Stony Brook, NY, USA}
\newcommand{\UoS}{University of Sussex, Falmer, East Sussex, UK}
\newcommand{\SYR}{Syracuse University, Syracuse, NY, USA}
\newcommand{\TAU}{Tel-Aviv University, Tel-Aviv, Israel}
\newcommand{\TAMU}{Department of Physics and Astronomy, Texas A\& M University, College Station, TX, USA}

\newcommand{\UGTO}{Universidad de Guanajuato, Leon GTO, MX}
\newcommand{\UTA}{University of Texas, Arlington, TX, USA}
\newcommand{\UTC}{University of Toronto, Toronto, Canada}
\newcommand{\TUNL}{Triangle Universities Nuclear Laboratory, Durham, NC, USA}
\newcommand{\UCL}{University College London, London WC1E 6BT, United Kingdom}
\newcommand{\UNICAMP}{Universidade Estadual de Campinas (UNICAMP), Campinas, SP, Brazil}
\newcommand{\UNIFAL}{Universidade Federal de Alfenas (Unifal-MG), Po\c{c}os de Caldas, MG, Brazil}
\newcommand{\UFSCAR}{Universidade Federal de São Carlos (UFSCar), Araras, SP, Brazil}
\newcommand{\UNIFESP}{Universidade Federal de S\~ao Paulo (UNIFESP), Diadema, SP, Brazil}
\newcommand{\UFABC}{Universidade Federal do ABC (UFABC), Santo André, SP, Brazil}
% Was already defined above. Which version do we prefer?
%\newcommand{\UNIFAL}{Federal University of Alfenas (UNIFAL) - Minas Gerais, Alfenas, MG, Brazil}
\newcommand{\UGA}{University Grenoble Alpes, CNRS, Grenoble INP, LPSC-IN2P3, 38000 Grenoble, France}
\newcommand{\Warwick}{University of Warwick, Coventry, UK}
\newcommand{\Wellesley}{Wellesley College, Physics Department, Wellesley, MA, USA}
\newcommand{\UW}{University of Wisconsin, Madison, WI USA}
\newcommand{\VT}{Center for Neutrino Physics, Virginia Tech, Blacksburg, Virginia, USA}
\newcommand{\YALE}{Yale University, New Haven, CT, USA}
\newcommand{\YorkU}{York University, Toronto, ON, Canada}

\newcommand{\ucb}{Physics Department, University of California at Berkeley, Berkeley, CA 94720-7300
}
\newcommand{\lbnl}{
Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720-8153, USA
}
\newcommand{\jul}{Institut f{\"u}r Kernphysik, Forschungszentrum J{\"u}lich, 52425 J{\"u}lich, Germany
}\newcommand{\penn}{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104-6396
}\newcommand{\fcul}{Universidade de Lisboa, Faculdade de Ci{\^e}ncias (FCUL), Departamento de F{\'i}sica, Campo Grande, Edifício C8, 1749-016 Lisboa, Portugal
}\newcommand{\lip}{Laborat{\'o}rio de Instrumenta{}{\c c}{\~a}o e F{\'i}sica Experimental de Part{\'i}culas (LIP), Av. Prof. Gama Pinto, 2, 1649-003, Lisboa, Portugal
}\newcommand{\chic}{
The Enrico Fermi Institute and Department of Physics, The University of Chicago, Chicago, IL 60637, USA
}\newcommand{\bnl}{
Brookhaven National Laboratory, Upton, New York 11973, USA
}\newcommand{\uh}{
University of Hawai‘i at Manoa, Honolulu, Hawai‘i 96822, USA
}\newcommand{\iowa}{
Department of Physics and Astronomy, Iowa State University, Ames, IA 50011, USA
}\newcommand{\jyv}{
Department of Physics, University of Jyv{\"a}skyl{\"a}, Finland
}\newcommand{\ucd}{
University of California, Davis, 1 Shields Avenue, Davis, CA 95616, USA
}\newcommand{\bu}{
Boston University, Department of Physics, Boston, MA 02215, USA
}\newcommand{\mainz}{
Institute of Physics and Excellence Cluster PRISMA, Johannes Gutenberg-Universit{\"a}t Mainz, 55099 Mainz, Germany
}\newcommand{\ham}{
Institut f{\"u}r Experimentalphysik, Universit{\"a}t Hamburg, 22761 Hamburg, Germany
}\newcommand{\alb}{
University of Alberta, Department of Physics, 4-181 CCIS, Edmonton, AB T6G 2E1, Canada
}\newcommand{\pnnl}{
Pacific Northwest National Laboratory, Richland, WA 99352, USA
}\newcommand{\laur}{
Laurentian University, Department of Physics, 935 Ramsey Lake Road, Sudbury, ON P3E 2C6, Canada
}\newcommand{\lsu}{
Department of Physics and Astronomy, Louisiana State University, Baton Rouge, LA 70803
}\newcommand{\tub}{
Kepler Center for Astro and Particle Physics, Universit{\"a}t T{\"u}bingen, 72076 T{\"u}bingen, Germany
}\newcommand{\sheff}{
University of Sheffield, Physics \& Astronomy, Western Bank, Sheffield S10 2TN, UK
}\newcommand{\qu}{
Queen's University, Department of Physics, Engineering Physics \& Astronomy, Kingston, ON K7L 3N6, Canada
}\newcommand{\snolab}{
SNOLAB, Creighton Mine 9, 1039 Regional Road 24, Sudbury, ON P3Y 1N2, Canada
}\newcommand{\rut}{
Department of Physics and Astronomy, Rutgers, The State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854-8019 USA
}\newcommand{\temp}{
Department of Physics, Temple University, Philadelphia, PA, USA
}\newcommand{\ucla}{
University of California Los Angeles, Department of Physics \& Astronomy, 475 Portola Plaza, Los Angeles, CA 90095-1547, USA
}
\newcommand{\tri}{
SISSA/INFN, Via Bonomea 265, I-34136 Trieste, Italy
}\newcommand{\kav}{
Kavli IPMU (WPI), University of Tokyo, 5-1-5 Kashiwanoha, 277-8583 Kashiwa, Japan
}\newcommand{\kor}{
Center for Underground Physics, Institute for Basic Science, Daejeon 34126, Korea
}\newcommand{\uci}{
University of California, Irvine, Department of Physics, CA 92697, Irvine, USA
}\newcommand{\aach}{
Physikzentrum RWTH Aachen, Otto-Blumenthal-Stra{\ss}e, 52074 Aachen, Germany
}\newcommand{\sbu}{
State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, USA
}\newcommand{\tsing}{
Department of Engineering Physics, Tsinghua University, Beijing 100084, China
}\newcommand{\corn}{
Cornell University, Ithaca, NY, USA
}\newcommand{\boul}{
University of Colorado at Boulder, Department of Physics, Boulder, Colorado, USA
}\newcommand{\dres}{
Institut f{\"u}r Kern und Teilchenphysik, TU Dresden, Zellescher Weg 19, 01069, Dresden, Germany
}
%\newcommand{\mun}{Physik-Department and Excellence Cluster Universe, Technische Universit{\"a}t M{\"u}nchen, 85748 Garching, Germany}
\newcommand{\mun}{Physics Department, Technische Universit{\"a}t M{\"u}nchen, 85748 Garching, Germany
}
\newcommand{\mitnew}{
Massachusetts Institute of Technology, Department of Physics and Laboratory for Nuclear Science, 77 Massachusetts Ave Cambridge, MA 02139, USA
}
\newcommand{\kings}{King’s College London, Department of Physics, Strand Building, Strand, London WC2R 2LS, UK}
\newcommand{\llnl}{
Lawrence Livermore National Laboratory, Livermore, CA 94550, USA
}
\newcommand{\fnal}{
Fermi National Accelerator Laboratory, Batavia, IL 60510, USA
}
\newcommand{\erc}{Department of Physics, Erciyes University, 38030, Kayseri, Turkey
}
\newcommand{\iow}{Department of Physics and Astronomy, The University of Iowa, Iowa City, Iowa, USA}


%\newcommand{\psu}{Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}
%\newcommand{\psup}{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\newcommand{\psu}{Pennsylvania State University, University Park, PA 16802, USA}

\newcommand{\heid}{Ruprecht-Karls-Universitat Heidelberg, Im
Neuenheimer Feld 227, Heidelberg, Germany}

\newcommand{\bart}{Bartoszek Engineering, Aurora, IL 60506, USA}

\newcommand{\ucbne}{Nuclear Engineering Department, University of California at Berkeley, Berkeley, CA 94720-7300
}
% \newcommand{\Other}{Other Affiliation.}

% 2nd Block of Commands
% Enter an affiliation directive for each newcommand you entered above. Please make sure it preserves the alphabetical order above.
%\affiliation{\UA}
%\affiliation{\ANL}
%\affiliation{\APC}
%\affiliation{\Atlantico}
%\affiliation{\UBERN}
%\affiliation{\BEU}
%\affiliation{\BU}
%\affiliation{\BNL}
%\affiliation{\BHU}
%\affiliation{\UB}
%\affiliation{\oB}
%\affiliation{\UoBham}
%\affiliation{\Caltech}
\affiliation{\UCB}
\affiliation{\UCD}
\affiliation{\UNC}
\affiliation{\UCI}
\affiliation{\JGU}
%\affiliation{\UCSB}
%\affiliation{\Cambridge}
%\affiliation{\Catania}
%\affiliation{\CERN}
%\affiliation{\CIEMAT}
%\affiliation{\Cincinnati}
%\affiliation{\CUSB}
%\affiliation{\Cinvestav}
%\affiliation{\Columbia}
%\affiliation{\CSU}
%\affiliation{\Drexel}
%\affiliation{\Duke}
%\affiliation{\EDI}
%\affiliation{\EIA}
%\affiliation{\FCUL}
%\affiliation{\FNAL}
%\affiliation{\UF}
%\affiliation{\UGR}
%\affiliation{\Harvard}
%\affiliation{\Hawaii}
%\affiliation{\Houston}
%\affiliation{\ISU}
%\affiliation{\IU}
%\affiliation{\IFIC}
%\affiliation{\IIT}
%\affiliation{\IITH}
%\affiliation{\CzechAcademyofSciences}
%\affiliation{\INFNMiB}
%\affiliation{\INFNNA}
%\affiliation{\INFNGE}
%\affiliation{\Insubria}
%\affiliation{\UOH}
\affiliation{\Iowa}
%\affiliation{\ISP}
%\affiliation{\IowaU}
%\affiliation{\Irfu}
%\affiliation{\Iwate}
%\affiliation{\jnu}
%\affiliation{\JBNU}
%\affiliation{\JSU}
%\affiliation{\JU}
%\affiliation{\KSU}
%\affiliation{\Kyiv}
%\affiliation{\NRCKI}
%\affiliation{\Lancaster}
%\affiliation{\LBNL}
\affiliation{\LLNL}
%\affiliation{\Liverpool}
%\affiliation{\LANL}
%\affiliation{\LIP}
%\affiliation{\LSU}
%\affiliation{\Lucknow}
%\affiliation{\Manchester}
%\affiliation{\MIT}
%\affiliation{\MPA}
%\affiliation{\UMN}
%\affiliation{\Duluth}
%\affiliation{\UMiss}
%\affiliation{\UCNCl}
%\affiliation{\UND}
%\affiliation{\ND}
%\affiliation{\UNSPMF}
%\affiliation{\OakRidge}
%\affiliation{\OSU}
%\affiliation{\OregonState}
\affiliation{\Oxford}
%\affiliation{\PNNL}
%\affiliation{\UniPR}
\affiliation{\Pennsylvania}
\affiliation{\Penn}
%\affiliation{\UTF}
%\affiliation{\PAU}
%\affiliation{\Pisa}
%\affiliation{\Princeton}
%\affiliation{\QMUL}
%\affiliation{\Rochester}
%\affiliation{\Rutgers}
%\affiliation{\SJSU}
%\affiliation{\Sheffield}
%\affiliation{\SLAC}
%\affiliation{\SDSMT}
%\affiliation{\SMU}
%\affiliation{\SU}
%\affiliation{\SBU}
%\affiliation{\UoS}
%\affiliation{\SYR}
%\affiliation{\TAU}
%\affiliation{\TAMU}
%\affiliation{\UGTO}
%\affiliation{\UTA}
%\affiliation{\UTC}
\affiliation{\TUNL}
%\affiliation{\UCL}
%\affiliation{\UNICAMP}
%\affiliation{\UNIFAL}
%\affiliation{\UFSCAR}
%\affiliation{\UNIFESP}
%\affiliation{\UFABC}
%\affiliation{\UGA}
%\affiliation{\UNIFAL}
%\affiliation{\Warwick}
%\affiliation{\Wellesley}
%\affiliation{\UW}
%\affiliation{\VT}
%\affiliation{\YALE}
%\affiliation{\YorkU}


% \affiliation{\Other}

%3rd Block of Commands, divided by "Editors", "Contributors", and "All Other Authors/Endorsers"

% Lead Editors go here in alphabetical order with affiliation indexed by %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT ADD YOUR NAME TO THIS SECTION unless you were an editor!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \author{\\A.~N.~Author}
% \affiliation{\Other}

\author{Joshua~Klein}
\altaffiliation{\Editor}
\affiliation{\Penn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO NOT ADD YOUR NAME ABOVE THIS LINE unless you were an editor!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO NOT ADD NAME TO THIS NEXT SECTION unless you were a primary contributor!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Contributing authors go here in new alphabetical order with affiliation indexed by \dagger

%\author{A.~Person}
%\altaffiliation{\Contributor}
%\affiliation{\IIT}

\author{Tomi Akindele}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Adam Bernstein}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Steven Biller}
\altaffiliation{\Contributor}
\affiliation{\Oxford}

\author{Nathaniel Bowden}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Jason Brodsky}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{D.F.~Cowen}
\altaffiliation{\Contributor}
\affiliation{\Pennsylvania}

\author{Michael Ford}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Julieta Gruszko}
\altaffiliation{\Contributor}
\affiliation{\UNC}
\affiliation{\TUNL}

\author{Logan Lebanowski}
\altaffiliation{\Contributor}
\affiliation{\Penn}

\author{Aobo Li}
\altaffiliation{\Contributor}
\affiliation{\UNC}
\affiliation{\TUNL}

\author{Viacheslav A. Li}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Wei Mu}
\altaffiliation{\Contributor}
\affiliation{\FNAL}

\author{J. Pedro Ochoa-Ricoux}
\altaffiliation{\Contributor}
\affiliation{\UCI}

\author{Gabriel~D.~Orebi~Gann}
\altaffiliation{\Contributor}
\affiliation{\UCB}
\affiliation{\LBNL}

\author{Mayly Sanchez}
\altaffiliation{\Contributor}
\affiliation{\Iowa}

\author{Robert Svoboda}
\altaffiliation{\Contributor}
\affiliation{\UCD}

\author{Matthew Wetstein}
\altaffiliation{\Contributor}
\affiliation{\Iowa}

\author{Michael Wurm}
\altaffiliation{\Contributor}
\affiliation{\JGU}

\author{Minfang Yeh}
\altaffiliation{\Contributor}
\affiliation{\BNL}

\collaboration{Editors and Contributors}

==> generated/parameters.tex <==
\newcommand{\ndmuidbeamrate}{\SI[round-mode=places,round-precision=1]{20.0}{\hertz}\xspace}

\newcommand{\cosmicmuondatayear}{\SI[round-mode=places,round-precision=0]{20.4289491035}{\tera\byte}\xspace}

\newcommand{\tpcdriftdistance}{\SI[round-mode=places,round-precision=2]{3.6}{\meter}\xspace}

\newcommand{\gdaqchannelnumberfactor}{\num[round-mode=places,round-precision=1]{1.1}\xspace}

\newcommand{\daqsamplerate}{\SI[round-mode=places,round-precision=1]{2.0}{\mega\hertz}\xspace}

\newcommand{\beamspillcycle}{\SI[round-mode=places,round-precision=1]{1.2}{\second}\xspace}

\newcommand{\tpcapaperdriftcell}{\num[round-mode=places,round-precision=2]{0.75}\xspace}

\newcommand{\snbdatavolumezs}{\SI[round-mode=places,round-precision=0]{2.4e-05}{\giga\byte}\xspace}

\newcommand{\beamreprate}{\SI[round-mode=places,round-precision=2]{0.833333333333}{\hertz}\xspace}

\newcommand{\ndrockmuonrate}{\SI[round-mode=places,round-precision=1]{10.0}{\hertz}\xspace}

\newcommand{\snbdataratefs}{\SI[round-mode=places,round-precision=1]{17.5226192958}{\mega\byte\per\second}\xspace}

\newcommand{\dunefsreadoutsize}{\SI[round-mode=places,round-precision=1]{24.8832}{\giga\byte}\xspace}

\newcommand{\betarate}{\SI[round-mode=places,round-precision=1]{11.16}{\mega\hertz}\xspace}

\newcommand{\chargezsthreshold}{\SI[round-mode=places,round-precision=1]{0.5}{\MeV}\xspace}

\newcommand{\tpcmodulemass}{\SI[round-mode=places,round-precision=0]{10.0}{\kilo\tonne}\xspace}

\newcommand{\dunenumberchannels}{\num[round-mode=places,round-precision=0]{1536000.0}\xspace}

\newcommand{\chargemaxsignalnoiseratio}{\num[round-mode=places,round-precision=0]{74.0}\xspace}

\newcommand{\ndecalmass}{\SI[round-mode=places,round-precision=0]{93.0}{\tonne}\xspace}

\newcommand{\cosmicmuondatarate}{\SI[round-mode=places,round-precision=1]{647.36816}{\kilo\byte\per\second}\xspace}

\newcommand{\dunenumberapas}{\num[round-mode=places,round-precision=0]{600.0}\xspace}

\newcommand{\dunefsreadoutrate}{\SI[round-mode=places,round-precision=1]{4.608}{\tera\byte/\second}\xspace}

\newcommand{\ndecalbeamrate}{\SI[round-mode=places,round-precision=1]{18.6}{\hertz}\xspace}

\newcommand{\cosmicmuoneventsize}{\SI[round-mode=places,round-precision=1]{2.5}{\mega\byte}\xspace}

\newcommand{\tpcapapermodule}{\num[round-mode=places,round-precision=0]{150.0}\xspace}

\newcommand{\nddatarate}{\SI[round-mode=places,round-precision=1]{1.0048}{\mega\byte\per\second}\xspace}

\newcommand{\chargehethreshold}{\SI[round-mode=places,round-precision=1]{10.0}{\MeV}\xspace}

\newcommand{\beamhighdatayear}{\SI[round-mode=places,round-precision=0]{21.9254891928}{\giga\byte}\xspace}

\newcommand{\betaratedensity}{\SI[round-mode=places,round-precision=3]{0.279}{\hertz\per\kilo\gram}\xspace}

\newcommand{\cosmicmuoncorrection}{\num[round-mode=places,round-precision=2]{1.36}\xspace}

\newcommand{\snbeventratetpc}{\SI[round-mode=places,round-precision=0]{100.0}{\hertz}\xspace}

\newcommand{\snbcloserfactor}{\num[round-mode=places,round-precision=0]{100.0}\xspace}

\newcommand{\snbeventsize}{\num[round-mode=places,round-precision=0]{48.0}\xspace}

\newcommand{\beamrunfraction}{\num[round-mode=places,round-precision=3]{0.667}\xspace}

\newcommand{\beamdatayearfs}{\SI[round-mode=places,round-precision=0]{218.230533073}{\tera\byte}\xspace}

\newcommand{\tpcfulllength}{\SI[round-mode=places,round-precision=1]{58.0}{\meter}\xspace}

\newcommand{\snbcanddatayearzs}{\SI[round-mode=places,round-precision=0]{200.88}{\giga\byte}\xspace}

\newcommand{\snbdataratehighzs}{\SI[round-mode=places,round-precision=0]{2.4e-05}{\tera\byte/\second}\xspace}

\newcommand{\ndeventrate}{\SI[round-mode=places,round-precision=1]{50.24}{\hertz}\xspace}

\newcommand{\dunefsreadoutsizeyear}{\SI[round-mode=places,round-precision=1]{145.414314891}{\exa\byte}\xspace}

\newcommand{\tpcfullwidth}{\SI[round-mode=places,round-precision=1]{14.5}{\meter}\xspace}

\newcommand{\daqchannelsperapa}{\num[round-mode=places,round-precision=0]{2560.0}\xspace}

\newcommand{\tpcapaheight}{\SI[round-mode=places,round-precision=1]{6.0}{\meter}\xspace}

\newcommand{\ndbytesperchannel}{\SI[round-mode=places,round-precision=0]{5.0}{\byte}\xspace}

\newcommand{\ndmuidmass}{\SI[round-mode=places,round-precision=0]{100.0}{\tonne}\xspace}

\newcommand{\ndmuidchannels}{\num[round-mode=places,round-precision=0]{165888.0}\xspace}

\newcommand{\gdaqtrigsamplespersnhit}{\num[round-mode=places,round-precision=0]{48.0}\xspace}

\newcommand{\beamdataratefs}{\SI[round-mode=places,round-precision=0]{6.915456}{\mega\byte\per\second}\xspace}

\newcommand{\ndbeameventratedensity}{\SI[round-mode=places,round-precision=1]{0.2}{\hertz\per\tonne}\xspace}

\newcommand{\tpcapawidth}{\SI[round-mode=places,round-precision=1]{2.3}{\meter}\xspace}

\newcommand{\cosmicmuonrate}{\SI[round-mode=places,round-precision=3]{0.258947264}{\hertz}\xspace}

\newcommand{\ndsstbeamrate}{\SI[round-mode=places,round-precision=1]{1.6}{\hertz}\xspace}

\newcommand{\tpcdrifttime}{\SI[round-mode=places,round-precision=2]{2.25}{\milli\second}\xspace}

\newcommand{\snbeventsizefs}{\SI[round-mode=places,round-precision=1]{46.08}{\tera\byte}\xspace}

\newcommand{\chargeminsignalnoiseratio}{\num[round-mode=places,round-precision=0]{15.0}\xspace}

\newcommand{\beameventsizecompressed}{\SI[round-mode=places,round-precision=1]{0.1}{\mega\byte}\xspace}

\newcommand{\ndecalchannels}{\num[round-mode=places,round-precision=0]{52224.0}\xspace}

\newcommand{\ndcosmicmuonrate}{\SI[round-mode=places,round-precision=2]{0.04}{\hertz}\xspace}

\newcommand{\ndbeameventrate}{\SI[round-mode=places,round-precision=1]{40.2}{\hertz}\xspace}

\newcommand{\gdaqronetriggeredphysicsdatarate}{\SI[round-mode=places,round-precision=0]{0.8448}{\byte\per\second}\xspace}

\newcommand{\gdaqunit}{\SI[round-mode=places,round-precision=0]{0.825}{\byte}\xspace}

\newcommand{\gdaqbetahighrateAPA}{\SI[round-mode=places,round-precision=0]{500.0}{\kilo\hertz}\xspace}

\newcommand{\dunenumbermodules}{\num[round-mode=places,round-precision=0]{4.0}\xspace}

\newcommand{\daqreadoutchannelsamples}{\num[round-mode=places,round-precision=0]{10800.0}\xspace}

\newcommand{\beameventsize}{\SI[round-mode=places,round-precision=1]{2.5}{\mega\byte}\xspace}

\newcommand{\tpcdriftvelocity}{\SI[round-mode=places,round-precision=1]{1.6}{\milli\meter\per\micro\second}\xspace}

\newcommand{\gdaqronebeamphysicsdatarate}{\SI[round-mode=places,round-precision=0]{41250.0}{\kilo\byte\per\second}\xspace}

\newcommand{\gdaqronedatarate}{\SI[round-mode=places,round-precision=0]{41.5153208448}{\mega\byte\per\second}\xspace}

\newcommand{\ndsstmass}{\SI[round-mode=places,round-precision=0]{8.0}{\tonne}\xspace}

\newcommand{\beamfsdatarate}{\SI[round-mode=places,round-precision=0]{436.461066147}{\peta\byte\per\year}\xspace}

\newcommand{\snbreadouttime}{\SI[round-mode=places,round-precision=1]{10.0}{\second}\xspace}

\newcommand{\gdaqronebetadatarate}{\SI[round-mode=places,round-precision=1]{41.25}{\mega\byte\per\second}\xspace}

\newcommand{\snbcanddataratezs}{\SI[round-mode=places,round-precision=0]{6365.63904105}{\byte\per\second}\xspace}

\newcommand{\gdaqnoncosmicoverheadfactor}{\num[round-mode=places,round-precision=1]{1.5}\xspace}

\newcommand{\gdaqronelowenergyphysicsdatarate}{\SI[round-mode=places,round-precision=0]{7.92}{\kilo\byte\per\second}\xspace}

\newcommand{\gdaqcrrateAPA}{\SI[round-mode=places,round-precision=4]{0.0004}{\hertz}\xspace}

\newcommand{\beamonfraction}{\num[round-mode=places,round-precision=0]{0.0030015}\xspace}

\newcommand{\betadatayear}{\SI[round-mode=places,round-precision=0]{52.8262940816}{\peta\byte}\xspace}

\newcommand{\betainspillyear}{\SI[round-mode=places,round-precision=0]{158.558121686}{\tera\byte}\xspace}

\newcommand{\gdaqtrigcompression}{\num[round-mode=places,round-precision=0]{2.0}\xspace}

\newcommand{\gdaqhighrateAPAs}{\num[round-mode=places,round-precision=0]{100.0}\xspace}

\newcommand{\daqdriftsperreadout}{\num[round-mode=places,round-precision=1]{2.4}\xspace}

\newcommand{\snbdatavolumehighzs}{\SI[round-mode=places,round-precision=0]{0.00024}{\tera\byte}\xspace}

\newcommand{\ndsstchannels}{\num[round-mode=places,round-precision=0]{215040.0}\xspace}

\newcommand{\gdaqroneSNphysicsdatarate}{\SI[round-mode=places,round-precision=0]{257.4}{\kilo\byte\per\second}\xspace}

\newcommand{\beamhighdatarate}{\SI[round-mode=places,round-precision=2]{0.694791666667}{\kilo\byte\per\second}\xspace}

\newcommand{\dunefsreadoutsizeminute}{\SI[round-mode=places,round-precision=1]{276.48}{\tera\byte}\xspace}

\newcommand{\daqchannelspermodule}{\num[round-mode=places,round-precision=0]{384000.0}\xspace}

\newcommand{\gdaqtrigsamplesperbetahit}{\num[round-mode=places,round-precision=0]{24.0}\xspace}

\newcommand{\snbcandrate}{\SI[round-mode=places,round-precision=0]{12.0}{\per\year}\xspace}

\newcommand{\dunedetectormass}{\SI[round-mode=places,round-precision=0]{40.0}{\kilo\tonne}\xspace}

\newcommand{\gdaqAPAchannelspercosmic}{\num[round-mode=places,round-precision=0]{2560.0}\xspace}

\newcommand{\ndeventsize}{\num[round-mode=places,round-precision=0]{4000.0}\xspace}

\newcommand{\snbdatayearfs}{\SI[round-mode=places,round-precision=0]{552.96}{\tera\byte}\xspace}

\newcommand{\dunefsreadoutsizesecond}{\SI[round-mode=places,round-precision=1]{4.608}{\tera\byte}\xspace}

\newcommand{\betainbeamyear}{\SI[round-mode=places,round-precision=0]{79.279060843}{\giga\byte}\xspace}

\newcommand{\gdaqlphighrateAPA}{\SI[round-mode=places,round-precision=0]{200.0}{\hertz}\xspace}

\newcommand{\betaeventsize}{\num[round-mode=places,round-precision=1]{100.0}\xspace}

\newcommand{\betadatarate}{\SI[round-mode=places,round-precision=1]{1.674}{\giga\byte\per\second}\xspace}

\newcommand{\betareadoutsize}{\SI[round-mode=places,round-precision=0]{150.0}{\byte}\xspace}

\newcommand{\snbcandeventsizezs}{\SI[round-mode=places,round-precision=1]{16.74}{\giga\byte}\xspace}

\newcommand{\daqreadouttime}{\SI[round-mode=places,round-precision=1]{5.4}{\milli\second}\xspace}

\newcommand{\cosmicmuonflux}{\SI[round-mode=places,round-precision=2]{5.66e-09}{\hertz\per\centi\meter\squared}\xspace}

\newcommand{\snbdataratezs}{\SI[round-mode=places,round-precision=0]{2.4e-06}{\giga\byte\per\second}\xspace}

\newcommand{\tpcfullheight}{\SI[round-mode=places,round-precision=1]{12.0}{\meter}\xspace}

\newcommand{\gdaqsnhighrateAPA}{\SI[round-mode=places,round-precision=0]{6500.0}{\hertz}\xspace}

\newcommand{\beameventoccupancy}{\num[round-mode=places,round-precision=4]{0.0005}\xspace}

\newcommand{\beamrate}{\SI[round-mode=places,round-precision=0]{8770.19567714}{\per\year}\xspace}

\newcommand{\daqbytespersample}{\SI[round-mode=places,round-precision=1]{1.5}{\byte}\xspace}


==> sections/table-of-LOIs.tex <==
\begin{table}[hbt!]
\begin{centering}
\begin{tabular}{|l|l|l|}
\hline\hline
Target	&  Loading (mass) & Potential Applications\\
\hline
 Indium		 & $>$8\% In  &  Solar $\nu$ \\ 
\hline
 Tellurium 		 & $>$ 6\% Te  &  $0\nu\beta\beta$\\ 
\hline
 Lithium 		 & $0.1$\% $^6$Li  & Reactor $\bar{\nu}$; excellent PSD  \\ 
 &  $>$0.2\% $^6$Li  & Reactor $\bar{\nu}$; super PSD with improved optics \\ 
\hline
 Boron		 & $>$0.5\%   & Dark Matter veto, reator $\bar{\nu}$ \\ 
\hline
 Potassium 		 & $>$1\%  &  Calibration for LS detectors\\ 
\hline
 Iron, Strontium & ppm to 1\%  & Nuclear waste management, \\ 
 &   & enviromental tracers\\ 
\hline
 Gadolinium & 0.1\% Gd  & Dark matter veto \\ 
 &   & Reactor monitoring\\ 
 &   & Reactor $\bar{\nu}$ oscillations\\ 
\hline
\hline
 High-Z elements & 10-15\%Pb  & Solar $\nu$ \\ 
 &   & Calorimeters \\ 
 &   & Medical QA/AC \\ 
\hline\hline
\end{tabular}
\caption{Table of LOIs.\label{tbl:lois}}
\end{centering}
\end{table}

==> snowmass-loi-neutrino.tex <==
%\documentclass[11pt]{article}
%\documentclass[floatfix,prd,epsfig,nofootinbib,superscriptaddress,onecolumn,amssymb]{revtex4}
%\documentclass[11pt]{revtex4}

%\usepackage{slashed}
%\usepackage{graphicx,color}
%\usepackage{epsfig}
%\usepackage{dcolumn}
%\usepackage{bm}
%\usepackage{color}
%\usepackage{siunitx}
% \usepackage{subfigure} removed in favor of "subcaption" package below for additional features. Shouldn't break anything (brodsky3@llnl.gov)
%\usepackage{caption}
%\usepackage{subcaption}
%\usepackage{lineno}

%\usepackage{times}
%\usepackage{geometry}
%\geometry{letterpaper, portrait, margin=1in}  
%\usepackage[utf8]{inputenc}
%\usepackage{enumitem,amssymb}
%\usepackage{ragged2e}
%\usepackage{graphicx}
%\usepackage{subcaption}
%\usepackage{comment}
%\usepackage{multicol}
%\usepackage[usenames]{xcolor} %used for font color              
%\definecolor{xlinkcolor}{cmyk}{1,1,0,0}
%\usepackage{url}
%\usepackage[
% colorlinks=true,    % false: boxed links; true: colored links 
% linkcolor=xlinkcolor,     % color of internal links            
% citecolor=xlinkcolor,     % color of links to bibliography
% filecolor=xlinkcolor,  % color of file links 
% urlcolor=xlinkcolor,      % color of external link
% final=true
%]{hyperref}
%\usepackage[super,sort&compress]{natbib}
%\usepackage{enumitem}
%\setenumerate{itemsep=0mm}

%\setlength{\parskip}{0.5em}
%\def\lsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
%    \raise1pt\hbox{$<$}}}         %less than or approx. symbol
%\def\gsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
%    \raise1pt\hbox{$>$}}}         %greater than or approx. symbol
%    
%\newcommand{\nc}{\newcommand}  
%\newcommand{\beq}{\begin{equation}}  
%\newcommand{\eeq}{\end{equation}}  
%\newcommand{\beqa}{\begin{eqnarray}}  
%\newcommand{\eeqa}{\end{eqnarray}}  
%\newcommand{\bea}{\begin{eqnarray}}  
%\newcommand{\eea}{\end{eqnarray}}  
%\newcommand{\ra}{\rightarrow}  
%\newcommand{\slsh}{\slash\hspace*{-0.22cm}}
%\def\ie{{\it i.e.}}
%\def\eg{{\it e.g.}}
%\def\etc{{\it etc}}
%\def\etal{{\it et al.}}
%\def\ibid{{\it ibid}.}
%\def\to{\rightarrow}
%\def\Re{{\cal R \mskip-4mu \lower.1ex \hbox{\it e}\,}}
%\def\Im{{\cal I \mskip-5mu \lower.1ex \hbox{\it m}\,}}
%\def\be{\begin{equation}}
%\def\ee{\end{equation}}
%\def\bea{\begin{eqnarray}}
%\def\eea{\end{eqnarray}}
%\def\bit{\begin{itemize}}
%\def\eit{\end{itemize}}
%\newcommand{\eref}[1]{(\ref{#1})}
%\newcommand{\Eref}[1]{Eq.~(\ref{#1})}

%\newcommand{\vev}[1]{ \left\langle {#1} \right\rangle }
%\newcommand{\bra}[1]{ \langle {#1} | }
%\newcommand{\ket}[1]{ | {#1} \rangle }
%\newcommand{\fb}{\,{\rm fb}^{-1}}
%\newcommand{\ev}{{\rm eV}}
%\newcommand{\kev}{{\rm keV}}
%\newcommand{\Mev}{{\rm MeV}}
%\newcommand{\gev}{{\rm GeV}}
%\newcommand{\tev}{{\rm TeV}}
%\newcommand{\mev}{{\rm MeV}}
%\newcommand \eos{\textsc{Eos} }
%\newcommand \theia{\textsc{Theia} }
%
%%%  caligraphic letters (for matrix elements, luminosity, etc.)
%
%\def\D{{\cal D}}
%\def\L{{\cal L}}
%\def\M{{\cal M}}
%\def\O{{\cal O}}
%\def\W{{\cal W}}

%%  matrix operations and fractions:

%\def\One{\ensuremath{\bf 1}\xspace}
%\def\hc{\ensuremath{\mbox{\rm h.c.}}\xspace}
%\def\tr{\ensuremath{\mbox{\rm tr}}\xspace}
%\def\half{\ensuremath{\frac{1}{2}}\xspace}
%\def\thalf{\ensuremath{\frac{3}{2}}\xspace}
%\def\third{\ensuremath{\frac{1}{3}}\xspace}
%\def\tthird{\ensuremath{\frac{2}{3}}\xspace}
%
%\begin{document}
%\begin{raggedright} 
%{\Large \textit{Neutrino Topical Group \#10: Neutrino Detectors} \hfill} \\[+0.3em]
%{\large \bf Snowmass 2021 Report Draft} \hfill \\[+1em]
%\end{raggedright}
%
%\normalsize
%
%\noindent {\bf Conveners:}\\
%Josh Klein (University of Pennsylvania) [\href{mailto:jrk@hep.upenn.edu}{jrk@hep.upenn.edu}] \\
%Ana Machado (University of Campinas) [\href{mailto:aameliabm@gmail.com}{aameliabm@gmail.com}] \\
%David Schmitz (University of Chicago) [\href{mailto:dwschmitz@uchicago.edu}{dwschmitz@uchicago.edu}] \\
%Raimund Strauss (Technical University Munich) [\href{mailto:raimund.strauss@mytum.de}{raimund.strauss@mytum.de}] \\
%
%\input{expanded_authorlist.tex}

%\textsf{\tableofcontents}

%\abstract{Please note that this is still a work in progress, and many sections still need to be filled in, and several others will be edited down for length and emphasis}.

%\linenumbers
\section{Introduction}
\label{sec:intro}

    The focus of NF10, ``Neutrino Detectors,'' is on enabling technologies in the context of neutrino detection.  Neutrino physics spans an enormous range of energies and scales: from detection of low-energy cosmic neutrinos, to keV-scale recoils in coherent neutrino scattering, to MeV-scale solar, reactor, and neutrinoless double beta decay events, to GeV and TeV scale detection of neutrinos from accelerators and the atmosphere.  While any particular neutrino experiment tends to focus on just one or two detection technologies---say, ionization and photon detection---the great breadth of neutrino physics means that there is an equally broad spectrum of detection technologies and methodologies.  
    
    At any one time, there are a dozen medium- to large-scale neutrino detectors operating worldwide, several more in the planning or construction phases, and many future detectors planned.  Beyond this are the diverse set of small- to medium-scale prototypes distributed across universities and labs.  Table~\ref{tbl:summary} summarizes many of these, their physic goals, primary detector technologies, and status.
    
    We have in this report focused on new approaches that will enable {\it future neutrino detectors} and thus, experiments that already exist, or are under construction or for which advanced technical designs already exist are not discussed in great detail.  
    
    

\section{Noble Element Detectors}

\subsection{Liquid Argon TPCs}

% review recent developments and current detectors in operation or under construction (MicroBooNE, ICARUS, SBND, ProtoDUNE).  Briefly overview different approaches being developed for future use from standard wire-based, to vertical drift, to ArgonCube.  

%Always looking to expand physics capabilities and reliability for long-term, underground operation, and near and far detector use cases.  

\subsubsection{Charge Readout Technologies}

%CRPs, various pixels, electron multiplication, dual readout (ion detection), and multi-modal pixels. 

%\subsubsection{Charge and Light Pixels}

\subsubsection{Photoionizing Dopants}

%\subsubsection{Underground Liquid Argon}

\subsubsection{Improvements in Simulation, Calibration, and Analysis}

\subsubsection{Gaseous Argon TPCs}

\subsection{Liquid Xenon}


section{Photon-Based Neutrino Detectors}

 Between the last SNOWMASS and now, there has been an explosion of new ideas and new, enabling technologies that will significantly expand the capabilities of next-generation photon-based neutrino detectors.
Detectors that use photons as the primary carrier of interaction information have a long, rich history in neutrino physics, going as far back as the discovery of the neutrino itself.  Large-scale, monolithic detectors that use either Cherenkov or scintillation light have played major roles in nearly every discovery of neutrino oscillation phenomena~\cite{superk,sno,dayabay,kamland,t2k} or observation of astrophysical neutrinos~\cite{kii,sno,imb,borexino,borexinopep,icecube}.  New detectors at even larger scales are being built right now, including JUNO~\cite{juno}, Hyper-Kamiokande~\cite{hyperk}, and DUNE~\cite{dunearapucas}.
    Photon-based detectors have been so successful because they are inexpensive, remarkably versatile, and have dynamic ranges that reach all the way from tens of keV~\cite{snoplus} to PeV~\cite{icecube}.  
    
        The new photon-based technologies that NF10 has surveyed include neutrino physics and astrophysics programs of great breadth: from high-precision accelerator neutrino oscillation measurements, to detection of reactor and solar neutrinos, and even to neutrinoless double beta decay measurements that will probe the normal hiearachy regime.   They will also be valuable for neutrino applications, such as non-proliferation via reactor monitoring.
        
        Of particular community interest is the development of {\it hybrid} Cherenkov/scintillation detectors, which can simultaneously exploit the advantages of Cherenkov light---reconstruction of direction and related high-energy PID---and the advantages of scintillation light---high light-yield, low-threshold detection with low-energy PID. Hybrid Cherenkov/scintillation detectors could have an exceptionally broad dynamic range in a single experiment, allowing them to have both high-energy, accelerator-based sensitivity while also achieving a broad low-energy neutrino physics and astrophysics program.  Recently the Borexino Collaboration~\cite{borexinocherscint} has published results showing that even in a detector with standard scintillator and no special photon sensing or collecting, Cherenkov and scintillation light can be discriminated well enough on a statistical basis that a sub-MeV solar neutrino direction peak can be seen.  Thus the era of hybrid detectors has begun, and many of the enabling technologies described here will make full event-by-event direction reconstruction in such detectors possible.
        
        There were many relevant letters-of-intent, which we summarize in Table~\ref{tbl:photon_lois}, and several white papers including one aimed explicitly at these kinds of detectors and their technologies. Table~\ref{tbl:photon_wps} summarizes the relevant white papers.


\subsection{Enabling Technologies for Hybrid Cherenkov/Scintillation Detectors}

 The physics accessible in large Water Cherenkov (WC) detectors such as Super-Kamiokande (SK) is limited in many areas of interest by the inability to detect particles with energy below the Cherenkov threshold.  One example is the sensitivity to the Diffuse Supernova Neutrino Background (DSNB)~\cite{SK_DSNB:2021} due to backgrounds from low-energy atmospheric neutrino interactions, and reduced signal from the inability to detect positron annihilation, which enhances the prompt signal from the leading reaction $\overline{\nu}_e + p\rightarrow e^{+} + n$. Similarly for proton decay, the kaon from $p\rightarrow \overline{\nu}K^{+}$ is below Cherenkov threshold, and for solar neutrinos the $^{7}$Be and CNO neutrinos are practically undetectable as much of the energy from the neutrino electron scattering reaction is invisible.

Organic liquid scintillators (LS) have been used to enhance sensitivity for particles below Cherenkov threshold, and to provide high light yield and thus narrow energy resolution needed to see monoenergetic signals like the $0\nu$ peak in neutrinoless double beta decay. Liquid scintillators also typically allow excellent discrimination between heavy particles like $\alpha$s or protons and electrons or $\gamma$ rays, through the differences in the scintillation time profile. These detectors thus typically aim for a primarily low-energy program, like reactor antineutrinos (KamLAND, Daya Bay, and JUNO), solar neutrinos (Borexino and SNO+), or neutrinoless double beta decay (KamLAND-Zen and SNO+). 

    Yet the narrow energy resolution and low-energy particle ID of scintillation detectors comes at the cost of the high-energy particle ID possible with Cherenkov light, and the reconstruction of direction from Cherenkov rings which helps identify events from point sources like the Sun.  Most high-energy neutrino physics programs---from accelerator beams or atmospheric neutrinos (or nucleon decay)---use ring imaging and counting to eliminate backgrounds.


Hybrid neutrino detectors, which leverage both the unique topology of Cherenkov light and the high light yield of scintillation, have the potential to revolutionize the field of low- and high-energy neutrino detection, offering unprecedented event imaging capabilities and resulting background rejection.  Such detectors would be more than the sum of scintillation and Cherenkov physics programs, as the information from one source of light leverages background rejection for physics in the other.  One example of this is the rejection of radioactive backgrounds in a low-threshold scintillation measurement of solar neutrinos using direction~\cite{gdogrbonv}; another is the rejection of atmospheric neutrino backgrounds to DSNB neutrinos, by counting Cherenkov rings and using the Cherenkov/scintillation ratio to remove mostly hadronic final states~\cite{dsnb_psd}.
At high energies, it may be possible to use scintillation light to precisely reconstruct the neutrino interaction vertex in a charged-current event, thus helping to eliminate backgrounds from NC $\pi^0$ production.

%These performance characteristics would substantially increase sensitivity to reactor signals, as well as a broad program of fundamental physics.

Discrimination between ``chertons'' and ``scintons'' can be achieved in several ways, each of which has its own advantages and drawbacks, but which ultimately fall into four broad classes: 
\begin{itemize}
\item Make chertons easier to see by increasing the Cherenkov/scintillation ratio, typically through suppression of the scintillation light 
\item Separate chertons from scintons by timing, by using fast photons sensors, or by slowing down the scintillation time profile, or by having a large enough detector that dispersion between ``blue'' scintillation light and broadband Cherenkov light allows them to be resolved
\item Exploiting the differences in the spectra of Cherenkov and scintillation light to distinguish chertons from scintons, either by sorting the photons with devices like dichroicons~\cite{dichroicons}, or using filters on some subset of the photon sensors to exclusively see long-wavelength Cherenkov light.
\item Use the angular distribution of Cherenkov light to identify it, through analysis techniques.
\end{itemize}

    Which approach works best depends on many things, including the dominant backgrounds for the physics of interest, cost, development status, robustness, etc.  The tensions between them typically contrast the required number of detected Cherenkov photons against scintillation light yield; direction reconstruction against vertex resolution; and backgrounds and robustness of new scintillation cocktails against high costs of new photon sensing or collecting devices.  A program of both benchtop R\&D, and mid-scale prototypes is underway to help answer these questions.  In principle, all of the approaches above could be used in a single detector, as they are for the most part not mutually exclusive.
    
    Below we detail the various enabling technologies for hybrid Cherenkov/scintillation neutrino detectors.  Far more detail can be found in the related white paper~\cite{photonwp}.


%The use of a cocktail like water-based liquid scintillator (WbLS) provides a
%favorable ratio of Cherenkov/scintillation light ~\cite{chess}.
%With good enough photon timing, separation purity can be as high as XXXX~ 
%Combining angular
%and timing information allows discrimination between Cherenkov and
%scintillation light for high-energy events even in a standard scintillator like
%LAB-PPO~\cite{chess}.  Slowing scintillator emission time down by using slow
%secondary fluors can also provide excellent separation~\cite{biller}, while using very fast timing~\cite{LAPPDtiming} can pick off the prompt Cherenkov photons from scintillators with faster time profiles.
%Recent R\&D with dichroic filters to sort photons by wavelength has shown
%separation of long-wavelength chertons from the typically shorter-wavelength
%scintons even in LAB-PPO, with only small reductions in the total scintillation
%light~\cite{dichroicons}.  In principle, all of these techniques could be
%deployed together if needed to achieve a particular full physics program.  New
%reconstruction techniques, to leverage the multi-component light detection, are
%being developed and with the fast timing of newly available PMTs and the
%ultrafast timing of LAPPDs (Large Area Picosecond Photon Detectors), allow effective tracking for high-energy
%events and excellent background rejection at low energies.    



\subsubsection{Water-based Liquid Scintillator}
\label{sec:wbls}

The development of Water-based Liquid Scintillator (WbLS)~\cite{wbls} has the potential to signifcantly impact and enhance  hybrid particle detection capabilities.
WbLS is essentially liquid scintillator encapsulated in surfactant micelles that are thermodynamically stable in water (see Fig.~\ref{fig:WbLS}).
By introducing varying amounts (typically 1\%-10\%) of liquid scintillator into water, the liquid yield can be adjusted to allow detection of particles below Cherenkov threshold  while not sacrificing directional capability, cost, or environmental friendliness. First developed at Brookhaven National Lab (BNL), WbLS is a leading candidate for the main target medium for the proposed \theia detector, which would enhance the scientific program at the LBNF significantly, as described in the \theia White Paper ~\cite{theiawp}.

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{figs/WbLS_Micelle2.png}
\caption{Top: Liquid scintillator encapsulated in a surfactant micelles, which are typically around 10 nm in size. Bottom: From right to left: water, 0.5\% WbLS, 1\% WbLS, pure liquid scintillator.}
\label{fig:WbLS}
\end{figure}


\subsubsection{Slow fluors}

The properties of four slow fluors have been studied in the context of LAB-based liquid scintillator mixtures to provide a means to effectively separate Cherenkov light in time from the scintillation signal with high efficiency. This allows for directional and particle ID information while also maintaining good energy resolution. Such an approach is highly economical (i.e. small compared to other experimental costs) and can be readily applied to existing and planned large-scale liquid scintillator instruments without the need of additional hardware development and installation. Using this technique, we have explicitly demonstrated Cherenkov separation on a bench-top scale, showing clear directionality, for electron energies extending below 1 MeV. 

Timing measurements were made using a 90Sr source directed through the sample vial and either towards or away from a measurement PMT. Electrons from supported beta decay of 90Y (Q=2.28 MeV) first pass through a 2mm diameter scintillating fibre coupled to a trigger PMT. Typical electron energies that make it through the fibre and vial wall are less than 1 MeV.

 While the use of slow fluors means that the vertex resolution may be worse than typical large-scale liquid scintillator detectors (but better than typical large-scale Cherenkov detectors), the balance between position resolution, Cherenkov separation purity and energy resolution can be tuned for a particular physics objective by modifying the fluor mixture. This balance is also affected by the presence of fluorescence quenchers, which may be naturally present in the case of loaded scintillator mixtures or could be purposely introduced to change the balance.

 
\subsubsection{Fast Photomultiplier Tubes and LAPPDs}
\label{sec:LAPPD}

Resolving Cherenkov and scintillation light via timing can be done even with ``standard'' scintillation cocktails, because the Cherenkov light is created promptly while scintillation light has both a risetime of hudreds of picoseconds and fall types that are in the multi-nanosecond regime, even without intentionally using a ``slow'' scintillator.
In addition, in large detectors, the dispersion of the broadband Cherenkov light means that many Cherenkov photons can arrive at a photon sensor a nanosecond or more before the scintillation light.

In the past decade there have been significant improvements in the time resolution of even standard photomultiple tubes (PMTs).  Hamamatsu, for example, has developed 8'' high-quantum efficiency PMTs that have transit time spreads (TTS) with FWHM of around 1.5~ns, or $\sigma\sim 700 ps$~\cite{tanner}.  With this kind of resolution, scintillator risetimes of 1~ns or so are slow enough to allow a prompt signal to be seen. Smaller PMTs
already have TTSs in the regime of 250~ps or so, and these can be ``ganged'' together to make larger-area arrays~\cite{chess}.  

The most aggressive approach to timing for photon sensors has been the development of
Large Area Picosecond Photodetectors (LAPPDs). LAPPDs are 20 cm x 20 cm microchannel plate photomultiplier tubes (MCP-PMTs)~\cite{Wiza:1979iia} now in use by the neutrino community and capable of millimeter-scale spatial resolutions, tens of picosecond sPE time resolutions, and gains exceeding $10^6$~\cite{LAPPDtiming}. 
%They bring much needed timing and imaging capabilities to a wide range of applications in fields such as particle physics, nuclear physics, X-ray science, and medical imaging. They also hold great potential in light-based neutrino detection, particularly in combination with imaging optics and dual scintillation-Cherenkov detectors~\cite{Aberle:2013jba}. 

\begin{figure}[ht!]
\centering
\includegraphics[width=0.4\textwidth]{./figs/LAPPDmodfront.jpg}
\includegraphics[width=0.4\textwidth]{./figs/LAPPDmodback.jpg}
\caption{Left: Front view of an ANNIE LAPPD Module. Right: The back of an LAPPD module with the back plate off.}
\label{fig:LAPPDmodule}
\end{figure}

%As imaging photodetectors, capable of resolving correlations between position and timing in a single module, LAPPDs are fundamentally different from conventional photomultipliers. LAPPDs can be used in combination with an wide variety of imaging optics such as plenoptic lens arrays and novel mirror optics to expand area coverage, sort photons by color and polarization, and even recover directional information. The combination of LAPPDs with novel imaging optics has the potential to free future water-based neutrino detectors from typical design constraints, and break away from the idea of the neutrino detector as a simple cylindrical (or spherical) bounding volume with phototubes on the surface. 



\begin{figure}[ht!]
\centering
\includegraphics[width=0.5\textwidth]{./figs/TTS_notlog}
\caption{The Transit Time Spread (TTS distribution) for ANNIE LAPPD-25. The time resolution for the prompt pulses is below 70ps, where roughly 30ps of smearing is due to the pulse duration of the diode laser used.}
\label{fig:LAPPDTTS}
\end{figure}

The combination of spatial and temporal information make LAPPDs ideal for Scintillation-Cherenkov separation. The $<$100 psec resolution of LAPPDs makes it possible to separate between the two components on the basis of timing alone. 
%However, it is also possible to sort different colors and different polarization of light to different areas of a single LAPPD surface.

%The capabilities of LAPPDs not only change how they can be used in designing future neutrino detectors but also places new requirements on Monte Carlo and reconstruction tools. The major existing Monte Carlo packages are hard-coded to assume single-pixel optical readouts. Many available reconstruction tools factorize the charge and timing likelihoods from the pattern-of-light when fitting for track hypotheses. Future development in reconstruction of light patterns should be broadened to enable simultaneous fitting of the positions and timing of the light patterns.

LAPPDs have other very useful applications for neutrino physics other than Cherenkov/scintillation separation. The precision timing capabilities of LAPPDs make possible new stroboscopic techniques that where different energy components of a wide-band neutrino beam can be selected based on the arrival of the neutrinos relative to the beam RF timing. Future neutrino experiments, including possible upgrades to LBNF could enable sufficiently short proton bunches to make this technique viable. At the detector end, this technique requires time resolutions on the order of no more than a few hundred picoseconds. Hybrid Cherenkov-scintillation detectors with LAPPDs are naturally well suited for this level of vertex precision. 

%In order to fully exploit the characteristics of LAPPDs, present and future experiments require waterproof modules containing low-cost, high-channel-count readout electronics to digitize signals close to the sensor. The leap from an individual LAPPD to a system of highly synchronized and deploy-able LAPPD modules is a massive undertaking in its own right. The ANNIE collaboration has successfully developed a first realization of such a system (see Fig~\ref{fig:LAPPDmodule}). In the coming decade, work to continue to streamline and improve on LAPPD modules is critical to their readiness for larger scale deployments. Next steps include fiberoptic communications with the surface electronics, improved self-triggering capabilities, and better optical coupling between the LAPPD and the window of the waterproof module.  

%While LAPPD technology has not yet achieved an economy of scale in terms of price and yields, the HEP community can help play a significant role in continuing to bring down the cost of this technology. R\&D efforts to streamline the fabrication process would make significant headway in making larger scale production lines possible. One possible technique involves sealing top window of the photosensor before making the photocathode and introducing the multi-alkalai vapors through tubes that can later be sealed off. Above all, continued use and testing of LAPPDs in the small- and medium-scale detectors will help support this technology through the final stages of tech transfer process. In the longer run, possible developments in medical imaging and homeland security could provide large and consistent markets for this technology outside of HEP.


\subsubsection{Spectral Sorting and Dichroicons}

 One approach to separating Cherenkov and scintillation light is by discriminating photons by wavelength, as scintillation is typically within a narrow emission band, while Cherenkov is a broad spectrum of light, falling as roughly $1/\lambda^2$. 

A simple approach to doing this would be to add filters in front of some subset of the photon sensors in a detector, filtering out the blue scintillation light and allowing longer-wavelength Cherenkov light to pass.  This has the advantage of simplicity, and in a detector with low photocathode coverage would be reasonable, if the size of the ``red-sensitive'' PMTs were large enough to detect enough long-wavelength Cherenkov photons.  As the coverage increases however, using filters in front of a subset of the PMTs means that some of the scintillation light is lost, and for physics that requires narrow energy resolution, every photon is important.

Dichroicons get around this problem by {\it sorting} photons by wavelength.
As shown in Figure~\ref{fig:dichroicon} below, the dichroicon follows the off-axis parabolic
\begin{figure}[ht!]
\centering
\includegraphics[width=0.35\textwidth]{./figs/dichroicon_nested_schematic.png}
\includegraphics[width=0.45\textwidth]{./figs/fullsetup.pdf}
\caption{Left: Schematic of a “nested” dichroicon configuration, with shortpass filters on the barrel and a longpass filter at the aperture. Right: Dichroicon in benchtop test setup, viewing $^{90}$Sr source embedded in an acrylic block containing LAB-PPO.}
\label{fig:dichroicon}
\end{figure}
design of an ideal Winston light concentrator but is built as a tiled set of
dichroic filters. The filters are used to direct long-wavelength light towards
a central red-sensitive PMT, while transmitting the shorter wavelength light
through the ``barrel'' of the Winston cone to secondary photodetectors. This is
possible because of the remarkable property of the dichroic reflectors, which
reflect one passband of light (below or above a ‘cut-on’ wavelength) while
transmitting its complement, with very little absorption. As shown
schematically in one possible design in Figure~\ref{fig:dichroicon}, the
barrel of the dichroicon is built from shortpass dichroic filters (cutoff
wavelength near 480~nm) and a longpass dichroic filter is placed at the
aperture of the dichroicon. The shortpass filter passes short-wavelength light
while reflecting long-wavelength light; the longpass has the complementary
response. In the ``nested'' design shown, the back PMT detects the short
wavelength light.

There are many possible configurations of the dichroicon; the ones built to
date are not necessarily optimal, and different detectors may have different
needs. The nested photon sensor configuration of the design above requires
more than one photon sensor and is thus most useful when the available
detection area is limited (for example, when the desired coverage is $>50$\%, or
in a segmented detector where each segment is viewed by a single sensor).
Simpler designs could simply offset the dichroicon and its aperture PMT,
collecting the low-yield Cherenkov photons while allowing the scintillation
light to be detected by the rest of the PMT array. Using a pixelated photon
sensor, such as an LAPPD or an array of SiPMs, would also work, with the pixels
then mapping to different wavelength bands. A complementary design—--with
Cherenkov light passing through the barrel and scintillation light reflected
toward the aperture—--might be most useful when ring imaging is a high
priority.  To achieve more than two passbands, the ``nested'' design could be
extended using mutliple dichroicons.

A simulation model of the dichroicon has been developed in {\it Chroma} (See Section~\ref{sec:chroma}) and calibrated against the measurements of a benchtop prototype, for use in simulating dichroicon performance large-scale detectors. This model was simplified and scaled up to use a 20" diameter large area PMT to collect photons passed by the short-pass dichroic filters, and a cylindrical 5” PMT to collect the long wavelength photons reflected by the dichroic filters shown at the top of Fig.~\ref{fig:chromadich}. This dichroicon unit was then tiled around a cylindrical volume to simulate a large-scale neutrino detector, seen from the inside at the bottom of Fig.~\ref{fig:chromadich}. In this model a 50 kt volume of the scintillator LAB with 2g/L of PPO [10] is surrounded by 90\% 
\begin{figure}[ht!]
\centering
\includegraphics[width=0.35\textwidth]{./figs/dichroicon_50kt.png}
\caption{A rendering of the {\it Chroma} geometry for (top)  a dichroicon unit with (left to right) 20” large area PMT, cylindrical 5” long-wavelength PMT, and dirchroic filter con- centrator, and (bottom) the dichroicon units tiled to create a 50 kt neutrino detector, viewed from inside the detector, with the full cylindrical geometry shown in the inset.}
\label{fig:chromadich}
\end{figure}
coverage of simplified dichroicons, which gives effectively 90\% coverage of both long and short wavelength photons, as the dichroic filters allow the long and short PMTs share the same solid angle. Using this model, we have begun to evaluate the impact of spectral photon sorting on future neutrino experiments.

A reconstruction algorithm developed in~\cite{wblsberk} has been modified such that it uses hit time information from all (short and long wavelength) PMTs to perform a position and time fit, and then uses the angular distribution of photons detected on long wavelength PMTs to perform a direction fit. An angular distribution of long-wavelength PMTs that detected photons from 2.6 MeV electrons generated at the center is shown in Fig~\ref{fig:dichcher}, which clearly shows the Cherenkov topology. 
%The angular resolution achieved when applying this algorithm to electrons generated at the center of this simulation is shown in Fig.~\ref{fig:dichang} , and indicates an angular resolution of 35 deg at 5 MeV, which can be compared to the 27 deg resolution achieved by the water-Cherenkov detector SNO [12] at the same energy.
\begin{figure}[ht!]
\centering
\includegraphics[width=0.35\textwidth]{./figs/dichroicon_cherenkov.png}
\caption{Distribution of the cosine of the angle between photons detected by long-wavelength PMTs and the initial direction of a 5 MeV electron simulated at the center of the detector geometry. The Cherenkov topology is clearly visible.}
\label{fig:dichcher}
\end{figure}

Alpha particle identification has been explored by simulating alpha and beta particles with the same quenched energy (number of scintillation photons) and inspecting the signal on the long-wavelength PMTs, which are pri- marily sensitive to Cherenkov photons. A quenched energy comparable to neutrinoless double beta decay in 130Te is chosen to highlight potential background rejection capabilities. The mean number of long-wavelength hits is indeed higher for betas than alphas as shown in Fig.~\ref{fig:dichpid} due to Cherenkov production with betas. The detected long wavelength photons from alphas are all scintillation, and indicate that the filters could be optimized for better rejection of scintillation. Fig.~\ref{fig:dichtime} shows a clear Cherenkov signal in the hit time residuals of betas at early times, which would allow for discrimination of alphas in a neutrinoless double beta decay region of interest. A similar method provides some discrimination between single and double beta events, as can be seen in the $^{130}$Te 0$\nu\beta\beta$ plots in Figs.~\ref{fig:dichpid} and~\ref{fig:dichtime}, which could further constrain backgrounds.
\begin{figure}[ht!]
\centering
\includegraphics[width=0.35\textwidth]{./figs/dichroicon_pid.png}
\caption{Number of long-wavelength PMTs that detected photons for alpha and beta events with the same quenched energy as $^{130}$Te neutrinoless double beta decay, showing alpha/beta discrimination based on Cherenkov photon identification in a 50 kt liquid scintillator detector.}
\label{fig:dichpid}
\end{figure}
\begin{figure}[ht!]
\centering
\includegraphics[width=0.35\textwidth]{./figs/dichroicon_timing.png}
\caption{The hit time residuals of long-wavelength PMTs for the events shown in Fig.~\ref{fig:dichpid}. The Cherenkov is clearly visible at early times for the beta events.}
\label{fig:dichtime}
\end{figure}

\subsubsection{Using Angular Information}

    The ring topology itself can be used to identify Cherenkon photons, essentialy by reconstructing events using PDFs in time and angle.  The CHESS array~\cite{chess} has shown this works for cosmic-ray muons, and work with simulations~\cite{wblsberk} has shown that even at lower energies the separation can be good enough if the scintillation light yield is low (as one would see in a WbLS detector, or a detector with a low level of secondary fluor added). 

\subsubsection{Comparing Cherenkov/scintillation Separation Approaches}

    Any comparison between the approaches discussed above is dangerous because they have all been done on the benchtop, with different sources, photon sensors, analyses, and other conditions.  And because they will each scale differently in large detectors, depending on the target material and size of the detector itself. Nevertheless, it is interesting to see side-by-side so many different successful ways of doing this discrimination which, at the time of the last SNOWMASS, was mostly just an idea.
    Figure~\ref{fig:cherscintcomp} shows distributions from the various approaches side-by-side.

\begin{figure}[ht!]
\centering
\includegraphics[width=0.25\textwidth]{figs/chess_lappd_labppo.pdf} 
\includegraphics[width=0.25\textwidth]{figs/chess_labppo.pdf} 
\includegraphics[width=0.25\textwidth]{./figs/Dichroicon_PTP.png}
\includegraphics[width=0.25\textwidth]{figs/SlowFluor1.pdf} 
\includegraphics[width=0.25\textwidth]{figs/flatdot_lab_timeresid.png} 
\includegraphics[width=0.25\textwidth]{figs/chess_wbls.pdf} 
\caption{The hit time residuals for several different approaches to separating out Cherenkov and scintillation light. \label{fig:cherscintcomp}}
\end{figure}



\subsection{Xe Doping and Arapucas for LAr}

    LAr is a particularly bright scintillator, with around 40,000 photons/MeV with no electric field, and with excellent discrimination between $\beta$s and heavier particles. Because the scintillation light is very short, at 128~nm, it needs to be wavelength shifted to be detected by PMTs or SiPMS, and the wavelength of choice is usually TPB.  Adding Xe to the LAr, however, shifts the light in advance of getting to the TPB, overall increasing light yield. The DUNE Collaboration has performed a large-scale test of this by adding Xe to the ProtoDUNE prototype at CERN's Neutrino Platform~\cite{pdunexe}, showing that in fact the Xe does as expected.  The fact that the shifted light tends to be the LAr triplet state also means that one might be able to do pulse-shape discrimination using spectral discrimination.
    
    Detecting light in LAr, particularly in LAr that has a strong electric field like that in a TPC, can be difficult with PMTs.  A new approach is the development of ARAPUCAs, which are light traps built out of dichroic mirrors and wavelength shifters. Light is shifted via TPB from the ultraviolet into the optical and passes through the mirror. On the other side, PTP is used to shift the light yet again to a band that the dichroic mirror reflects, thus trapping the light.  The advantage of this is now relatively small-area SiPMs can be used to detect the photons, since they have many chances of hitting the sensitive surface.


%\subsubsection{{Advanced }Photon Sensors and Collectors}

\subsection{Isotopic Loading Techniques for Low-energy Physics Programs}

    One of the great ways of expanding and improving the physics programs of photon-based detectors is through the loading of various isotopes.  These isotopes can be the source of the physics itself---as in neutrinoless double beta decay experiments---or leverage additional physics, such as the Gd loading of water to detect neutrons from supernova neutrinos, or $^6$Li to improve pulse-shape discrimination. We discuss some of the possibilities below.
    
    \subsubsection{Metal Loading in WbLS}
    \label{sec:mdwbls}
    
        Water-based liquid scintillator (WbLS) decribed above in Section~\ref{sec:wbls}, as an additional advantage in that loading of many isotopes is possible, using
        a mix of surface-active agents with hydrophilic as well as hydrophobic chelating groups to bridge aqueous (polar) and organic solvents (nonpolar). The principal, performance, and characteristics of WbLS are described in a Section IV. This WbLS allows inorganic metal salt to be first dissolved in water, followed by directly blended into any type of scintillator solvents, such as pseudocumene (PC), linear-alkyl-benzene (LAB), di-isopropylnaphthalene (DIPN), 1-phenyl-1-xylyl-ethane (PXE), cyclohexylbenzene (PCH), regardless the chemical property of each scintillator. WbLS has 100\%  metallic extraction efficiency and is particularly operative in extracting the hydrophilic elements (e.g. Boron, Lithium) into organic solvents, which, due to the high electron affinity of molecular hydrophilicity, often present great challenges using conventional organometallic technology, such as carboxylate, phosphate, or diketones ligands. The metal-doped principal for oil-based WbLS ($>$80\% scintillator) has been successfully demonstrated by PROSPECT experiment, a $\sim$0.1\% 6Lithium-doped DIPN-based WbLS, with good light yield ($>$10,000 ph/MeV) and superior pulse shape discrimination s/B~3).

Metal-doped WbLS devises in several applications for nuclear and particle physics experiments and can be fabricated and deployed at the ton scale.A summary of applications and competences of metallic targets doped in WbLS, either being deployed or still under development, is presented in Table~\ref{tbl:wblsload}.
\begin{table}[hbt!]
\begin{centering}
\begin{tabular}{|l|l|l|}
\hline\hline
Target	&  Loading (mass) & Potential Applications\\
\hline
 Indium		 & $>$8\% In  &  Solar $\nu$ \\ 
\hline
 Tellurium 		 & $>$ 6\% Te  &  $0\nu\beta\beta$\\ 
\hline
 Lithium 		 & $0.1$\% $^6$Li  & Reactor $\bar{\nu}$; excellent PSD  \\ 
 &  $>$0.2\% $^6$Li  & Reactor $\bar{\nu}$; super PSD with improved optics \\ 
\hline
 Boron		 & $>$0.5\%   & Dark Matter veto, reator $\bar{\nu}$ \\ 
\hline
 Potassium 		 & $>$1\%  &  Calibration for LS detectors\\ 
\hline
 Iron, Strontium & ppm to 1\%  & Nuclear waste management, \\ 
 &   & enviromental tracers\\ 
\hline
 Gadolinium & 0.1\% Gd  & Dark matter veto \\ 
 &   & Reactor monitoring\\ 
 &   & Reactor $\bar{\nu}$ oscillations\\ 
\hline
\hline
 High-Z elements & 10-15\%Pb  & Solar $\nu$ \\ 
 &   & Calorimeters \\ 
 &   & Medical QA/AC \\ 
\hline\hline
\end{tabular}
\caption{Examples of metallic targets loaded in Liquid Scintillator and Water-based Liquid Scintillator with projected applications\label{tbl:wblsload}}
\end{centering}
\end{table}

\subsubsection{Te Loading in Liquid Scintillator for $0\nu\beta\beta$}

A method for loading tellurium into organic liquid scintillator has been developed based on the formation of soluble organic compounds derived from telluric acid (Te(OH)6, hereafter TeA) and 1,2-butanediol (BD) in conjunction with N,N-dimethyldodecylamine (DDA), which acts as a stabilisation/solubilisation agent. The chemicals involved can all be purified to high levels, have high flash points and are relatively safe to work with in underground environments. The loading process results in acceptable optical absorbance and light output in larger detectors for loading levels up to several percent Te by weight. Stability of the loading has been demonstrated to be at least on the timescale of years. 


\begin{figure}[htp]
\centering 
\includegraphics[width=0.6\textwidth]{figs/TeLoading4.pdf}
\caption{Relative light levels as a function of percent Te loading for two variants of the technique: TeBD1 (heated solubilization) and TeBD2 (DDA-induced solubilization.} 
\label{fig:SlowFluor4}
\end{figure}


This is an important advance that opens the door to a highly scalable and economical approach for neutrinoless double beta decay. Further advances in Te loading and associated purification techniques could provide a practical path to realising sensitivity to the non-degenerate normal mass ordering.

\subsubsection{$^6$Li Loading in Plastic Scintillator}

Plastic scintillators are comprised of dopants entrained in a polymer matrix. In some cases, the scintillation signal from these dopants can be used to discriminate between particle types, e.g. electromagnetic depositions vs those from heavy ions, via ``Pulse Shape Discrimination'' (PSD)~\cite{ZAITSEVA201288}. Further particle discrimination can be enabled by other dopants that have specific neutron capture reactions, which can also be identified via a combination of energy gating and PSD. For example, when loaded with lithium-6 and high amounts a primary dye along with a secondary dye that shifts the wavelength of scintillation plastic scintillators can use PSD to distinguish between electrons or positrons, neutrons, and thermalized neutron captures~\cite{ ZAITSEVA2013747, MABE201680}. This new class of materials, primarily developed at the Lawrence Livermore National Laboratory,  can provide a combination of important capabilities for future neutrino detectors, particularly those that use Inverse Beta Decay where efficient and distinct detection of the low energy final state neutron is critical. 
At the current stage of development these plastics have broadly similar performance in terms of light yield, optical attenuation, and PSD separation to liquids (e.g. Fig.~\ref{fig:Li6-PSD}). Elements have been produced with greater than 50-cm length and 7.5-cm width, and a commercial vendor is developing a production process (Fig.~\ref{fig:Li6-PS}). 

A key challenge to the production of these $^6$Li-doped PSD plastics is the balance between scintillation properties and solubility of the dopants in the polymer matrix and the polymer precursors (i.e., monomers). 
Typical primary dyes like m-terphenyl (mTP) and 2,5-diphenyloxazole (PPO) have high solubility in monomers like styrene. However, organic salts that contain lithium-6 as the cation do not typically have high solubility in monomers like styrene. 
One option to improve the solubility of these lithium-6 salts is to incorporate a co-monomer with styrene that can dissolve the lithium-6 salts. 
Methacrylic acid is one possible co-monomer that has polar substituents that can solubilize the lithium-6 salts~\cite{osti_1490925,Frangville}. 
This co-monomer has been used primarily with organic salts that contain aliphatic organic groups. When used with dyes that contain heteroatoms like oxygen and nitrogen (e.g., PPO), this co-monomer may detrimentally affect the scintillation performance. 
Another option for soluble lithium-6 salts is to use organic salts with aromatic organic groups that have good solubility in primary dyes like PPO. 
A co-monomer like methyl methacrylate or a small amount of solvent (e.g., tetrahydrofuran) may be necessary to improve solubility of these aromatic lithium-6 salts without drastically reducing scintillation performance~\cite{osti_1490925}.
However, the aromatic groups may absorb energy and affect scintillation performance. 
Additionally, the aromatic acids that are used to synthesize these aromatic salts are solid at room temperature, which makes purification of the lithium-6 salts difficult. 
Overall, the balance of scintillation properties and solubility of dopants that enable multiple modes of PSD remains an interesting challenge to investigate and solve. 


Plastic scintillators with PSD and $^6$Li-doping provide the same capabilities as the PSD $^6$Li-doped liquid scintillator used for  PROSPECT that is described in Sec.~\ref{sec:mdwbls}. 
As described in a recent LOI~\cite{Li6Organic:2021loi}, the new solid form makes self-supporting fine-grained segmentation on a large scale possible, enables light guiding approaches based on air gaps, and eliminates the need for containment vessels and supporting infrastructure. Several detector implementations are proposed and under development using $^6$Li-doped PSD plastics. The SANDD concept (Fig.~\ref{fig:Li6-PS}) has implemented mm-scale segmentation to study reactor antineutrino directionality and cosmogenic background rejection~\cite{Li:2019sof,Sutanto:2021xpo}. Segmentation at the 5--10-cm scale in 2D bar geometries is being developed for efficient, aboveground reactor antineutrino detection (e.g. ROADSTR~\cite{ROADSTR:2021loi}) with the goal of a mobile system appropriate for monitoring applications and measurements at  multiple reactors with correlated systematics.

\begin{figure}[ht]
     \centering
     \begin{subfigure}{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/LiPS-PSD.png}
         \caption{Pulse Shape Discrimination performance of the 5.5~cm $\times$ 5.5~cm $\times$ 50~cm $^6$Li-doped PSD plastic scintillator shown in panel (b) under $^{252}$Cf flood-field illumination , in terms of uncalibrated ADC units. A clear neutron capture feature is observed at about 0.5~MeV$_{ee}$, along with electronic and nuclear recoil separation.}
         \label{fig:Li6-PSD}
     \end{subfigure}
      \hfill
     \begin{subfigure}{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/Li6_PSD_plastic_50_cm.jpg}
          \includegraphics[width=0.6\textwidth]{figs/SANDD_central_module.JPG}
         \caption{Photographs of $^6$Li-doped PSD plastic scintillator examples. {\it Top:} A 5.5~cm $\times$ 5.5~cm $\times$ 50~cm bar produced by Eljen Technology. {\it Bottom:} 64 rods of 5.4~mm $\times$ 5.4~mm$ \times$ 40~cm dimensions, as used in the SANDD central module~\cite{Sutanto:2021xpo}.}
         \label{fig:Li6-PS}
     \end{subfigure}
     \hfill
        \caption{Examples of $^6$Li-doped PSD plastic scintillator.}
        \label{fig:Li6_Scintillators}
\end{figure}

\subsubsection{Quantum Dots}

In recent years new methods for the production of metal loaded LS in neutrino physics were studied involving semiconducting nanocrystals, which are known as “quantum dots” [69]. The optical and electrical properties of the quantum dots are directly proportional to their size, which is typically in the order of few nanometers. The emission band consists of a narrow resonance around the characteristic wavelength of the dot.  Since the dot size can be controlled to high precision in the synthesis, the absorption and re-emission spectrum of the dots can be tuned and optimized for a respective application. In some synthesis methods the quantum dots are already delivered in colloidal suspension with the aromatic solvent toluene at concentrations of several grams per liter.

The most commonly used quantum dot cores are binary alloys such as CdS, CdSe, CdTe, and ZnS. Alternatively, there are also phosphor-based rare-earth dots. Therefore, quantum dots provide a method to dope scintillator with various metals and rare-earth elements. For a cadmium (Cd) based LS there are two different applications in the field of neutrino physics: neutron-enhanced isotopes (113Cd) and $\beta\beta$-decay candidates (106,116Cd). Also Se, Te, and Zn, which are present in common quantum dot cores, have $\beta\beta$-decay candidates. There is also a possibility to tune the scintillator emission spectrum in a way that allows to separate scintillation from Cerenkov light by narrowing scintillation emission from the quantum dots separated from the Cerenkov contribution.

The basic limitations of quantum-dot-doped liquid scintillator in use for particle physics detectors are probably cost and availability in large quantity ($\sim$ ton). The stability tests on typical solutions of quantum dots in concentration at few g/l indicate that larger particles are formed by aggregation in the concentrated solutions over long time scales. This could explain the fact that filtering improves the attenuation length as well as the observation of transparency degradation after several weeks. However, there is room for optimization on the stability and optical performance by improvements in the loading process of quantum dots in scintillator solution. Instead of suspension, incorporating chelating agents or WbLS surface active agents into the mixing procedures could load the quantum dots in organic solvents homogeneously with lengthy stability.





%\subsubsection{Isotopic Loading}

%\subsection{Future Approaches to Readout and DAQ}

\subsection{Improvements in Simulation and Analysis}

    The ever-increasing desire for more precise detectors models and better background rejection has led to development of many new approaches to simulation and analysis.
    There are far too many to include all of them here, but we have focused on a few that were represented in relevant LOIs to NF10.

\subsubsection{GPU-Accelerated Photon Ray Tracing ({\it Chroma})}
\label{sec:chroma}

As large-scale neutrino detectors become ever larger, photon coverage
becomes higher, and photon sensor technology becomes more complex with devices 
like the ARAPUCA~\cite{arapucas}, the dichroicon~\cite{dichroicons}, or 
distributed imaging~\cite{gratta_image}, a major bottleneck in both 
simulation and reconstruction of physics events is the propagation of photons 
through the detector geometry. 
Originally created for the water Cherenkov option for the LBNE experiment, a
fast photon ray-tracer was developed by Stan Seibert and Anthony
LaTorre~\cite{chroma} that improved photon simulation speeds by a factor of 200 over
what GEANT4 itself could do.  In order to achieve such high performance, {\it
Chroma} combines techniques from 3D rendering algorithms with the massively
parallel calculation hardware inside GPUs.  Existing 3D rendering libraries,
while quite sophisticated, cannot be used directly for physics simulation
purposes, as those libraries tend to rely on physically-unrealistic
approximations and shortcuts to improve the appearance of the produced images.
Nevertheless, {\it Chroma} takes similar ideas and applies them within the
context of a physics simulation to improve performance without sacrificing
precision physics.  These techniques map well onto the massively parallel GPUs
found in today's workstations.  A high-end GPU costs approximately \$5000
(twice the cost of a fast consumer-grade CPU), yet provides forty times the raw
floating point performance and ten times the memory bandwidth.  {\it Chroma}
uses the CUDA toolkit, provided by NVIDIA, to directly access the GPU resources
and perform all major calculations.  CUDA-compatible GPUs are being used more
and more in the construction of large supercomputing clusters, which will make
it easier in the future for the work on next-generation neutrino detectors such
as \textsc{Theia}~\cite{theiawp} to use {\it Chroma}.

Nearly all fast 3D rendering systems represent the world geometry using a mesh
of triangles.  Triangle meshes are very simple to represent, and can be used to
approximate any surface shape, limited by how much memory can be devoted to
triangle storage.  With only one surface primitive, there is only code path to
optimize.  In particular, we have adopted the Bounding Volume Hierarchy (BVH)
technique from the graphics world to speed up ray intersection tests with
triangle meshes.  A BVH is a data structure that organizes a spatial
arrangement of shapes (triangles in our case) into a tree of nested boxes.
Rather than test for ray intersection with every triangle in a geometry, the
photon propagator tests for intersection with boxes in the BVH.  If the ray
does not intersect the box, then all of the children of that box can be
skipped, leading to a large reduction in the number of intersection tests
required.  For example, a model of a large, 200 kton water Cherenkov detector
consists of 62 million triangles, but the BVH reduces a typical propagation
step for a photon to 130 box intersection tests and only 2 triangle
intersection tests.

One collateral bonus of {\it Chroma's} speed is that it provides
remarkably beatiful, {\it realtime} detector displays. It is quite easy to
``fly through'' a detector and see it rendered in all of its detailed geometry,
exactly the way the photons themselves will see the detector.
\ref{fig:snoplus} shows a rendering of the SNO+~\cite{snoplus} detector which,
in a static pdf document like this proposal cannot be examined dynamically in
realtime, but was created from that realtime fly-through and simply captured
by screen-shot. The rendering is in fact a 3D image; with red-blue glasses one
can see the relief in the image.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{./figs/snoplus_3d_chroma}
\caption{A screen capture from a realtime, three-dimensional ``movie'' of the
SNO+~\cite{snoplus} detector created with {\it Chroma}, which is best viewed with red-blue 3D glasses. The model shown is exactly the model
used by {\it Chroma}'s physics simulation, albeit with false-color optics for
the display rather than the complete physics the simulation uses.  The PMTs are
fully rendered, including their Winston-cone light
concentrators.\label{fig:snoplus}}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.3\columnwidth]{./figs/updated_simulation_front}
\caption{\label{fig:holder}
The CAD drawing for the 3D-printed dichroic filter holder for the dichroicon~\cite{dichroicons} was directly imported into {\it Chroma}, and used to accurately simulate the orientations of the dichroic filters (shown in red and orange) with respect to the benchtop experiment.}
\end{figure}


The choice of representing geometries in {\it Chroma} as triangle mesh makes it straightforward to import CAD drawings into the optical simulation, as shown in \ref{fig:holder}.
All that is required is that the triangles on the mesh have optical properties assigned to them, which is a trivial operation in the case of a CAD model with uniform properties over its entire surface, but allows for fine-grained position dependent control of material properties as well. %as shown in \ref{fig:pmt_prop}.
This allows anyone with CAD experience to quickly create an arbitrarily complicated simulation without having to learn a new way to represent geometries. 
The ability to rapidly prototype designs makes {\it Chroma} well suited for benchtop studies as well, and with easy scaling up from there to very large detectors,
%., as can be seen in \ref{fig:chess_dichroicon}, which shows preliminary application of the dichroicon to the CHESS~\cite{chess_prc} experiment.
as shown in \ref{fig:theia25}, which includes 3D Large Area Picosecond Photodetectors (LAPPD)~\cite{LAPPDtiming} mixed with standard PMTs in a {\it Chroma} model of the \textsc{Theia}25~\cite{theiawp} detector.
\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{./figs/theia25_lappd_full_pattern}
\caption{\label{fig:theia25}
Next-generation photon detectors like LAPPDs~\cite{LAPPDtiming} are straightforward to simulate and include in larger geometries, as shown in this internal view of a \textsc{Theia}25~\cite{theiawp} model made with {\it Chroma}, which has mixed PMTs and LAPPDs for detecting photons.
The {\it Chroma} framework makes it quick and easy to explore new detector geometries and photon detecting devices.}
\end{figure} 


\subsubsection{GEANT4-based toolkits {\it RAT-PAC}}

RAT-PAC is an open-source GEANT4-based toolkit that offers both micro-physical simulation capabilities and analysis tools for high-precision event modeling, evaluation, and characterization, from benchtop test stands to large-scale detectors.

The RAT-PAC Monte Carlo simulation and analysis suite~\cite{ratpac} is a free and open-source version of the RAT toolkit.  RAT was first written for the Braidwood reactor experiment~\cite{braidwood},
and is now the official simulation and analysis package for  SNO+~\cite{snoplus}, DEAP, and MiniCLEAN~\cite{miniclean} experiments, thus benefiting from shared efforts in development and verification. A GEANT4-based package~\cite{geant4}, RAT-PAC (standing for ``RAT Plus Additional Code'') was branched off from the core RAT development some years ago, to form an open-source version of the code, available for public use.  RAT-PAC forms the basis of the official software for the \theia collaboration~\cite{theiawp}, the proposed third phase of ANNIE~\cite{annie-results}, and for the WATCHMAN collaboration, who are developing a design for the NEO detector to be located at the AIT facility in the UK~\cite{watchman}.

One of the great advantages of the RAT-PAC approach is that its procedural geometry description allows the same code to be used to simulate or analyze data from a large-scale experiment and a small benchtop test-stand.  Figure~\ref{fig:SNOp} shows the detailed geometry of the full ktonne-scale SNO+ detector, and the even larger \theia detector, and Fig.~\ref{fig:CHESS} shows the much smaller CHESS detector at UC Berkeley/LBNL~\cite{chess}. In addition to the flexible geometry descriptions, RAT-PAC takes a micro-physical approach, relying on physical, rather than phenomenological models. For example, individual photons are simulated hitting photon sensors and the resulting timing and charge are evaluated photon-by-photon, rather than by application of a phenomenological risetime correction.  Therefore, simulating both benchtop test stands and large-scale detectors with the same micro-physical detail and the same code means that parameter measurements made by the benchtop are more easily translated into the larger-scale detector.  A measurement of, for example, the light yield of a scintillator cocktail performed in a small-scale setup can be straightforwardly propagated to predict performance in large detectors, complete with systematics associated with optical models or even data acquisition approaches. Comparisons between simulations of Cherenkov and scintillation light generated using RAT-PAC and data from test stands, such as at Penn, CHESS at LBNL, and FlatDot at MIT, show good agreement.  An example from FlatDot is shown in Fig.~\ref{fig:CHESS}~\cite{flatdot}. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/SNOp.png} %\hspace{5mm}
    \includegraphics[width=0.39\textwidth]{figs/theia.png} %\hspace{5mm}
    \caption{(Left)  RAT-PAC generated image of the ktonne-scale SNO+ detector. (Right) RAT-PAC simulation of a high-energy (GeV) electron in the 50-ktonne \theia detector, including full photon tracking.  Blue shows Cherenkov photon track and red shows scintillation.}
    \label{fig:SNOp}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/CHESS.png} %\hspace{5mm}
    \includegraphics[width=0.48\textwidth]{figs/flatdot_edge.pdf}
    \caption{(Left) Photograph of the CHESS PMT array.  (Top centre) CAD image of the full CHESS detector.  (Bottom centre) RAT-PAC generated image of the full CHESS detector.  (Right) RAT-PAC simulations of both Cherenkov \textit{(left)} and scintillation \textit{(right)} signals show good agreement with data from the FlatDot experiment \textit{(bottom)}, up to a normalization factor reflecting the absolute light yield of the liquid scintillator.}
    \label{fig:CHESS}
\end{figure}\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/SNOp.png} %\hspace{5mm}
    \includegraphics[width=0.39\textwidth]{figs/theia.png} %\hspace{5mm}
    \caption{(Left)  RAT-PAC generated image of the ktonne-scale SNO+ detector. (Right) RAT-PAC simulation of a high-energy (GeV) electron in the 50-ktonne \theia detector, including full photon tracking.  Blue shows Cherenkov photon track and red shows scintillation.}
    \label{fig:SNOp}
\end{figure}

%\begin{figure}[ht!]
%    \centering
%    \includegraphics[width=0.5\textwidth]{figs/CHESS.png} %\hspace{5mm}
%    \includegraphics[width=0.48\textwidth]{figs/flatdot_edge.pdf}
%    \caption{(Left) Photograph of the CHESS PMT array.  (Top centre) CAD image of the full CHESS detector.  (Bottom centre) RAT-PAC generated image of the full CHESS detector.  (Right) RAT-PAC simulations of both Cherenkov \textit{(left)} and scintillation \textit{(right)} signals show good agreement with data from the FlatDot experiment \textit{(bottom)}, up to a normalization factor reflecting the absolute light yield of the liquid scintillator.}
%    \label{fig:CHESS}
%\end{figure}

RAT(-PAC) is based on GEANT4.10~\cite{geant4} and the GLG4Sim package written by Glenn Horton-Smith, with custom code for scintillation and neutron absorption processes as well as a complete model of  PMT optics.
RAT(-PAC) handles all stages of event simulation: from the propagation of primary particles; production of optical photons via Cherenkov and scintillation processes; individual photon propagation, including a full optical model of all detector materials;  photon detection at the single PE level, including individual photon detector charge and timing response; and data acquisition including full
customizable simulation of  front end electronics, trigger systems, and event builders.  It also allows root-formatted data to be used as input, and provides simple analysis tools and ways to include many more, as well as a macro command structure for control. Lastly, RAT-PAC also includes the
ability to 
dynamically generate detector configurations via an external database.
%generate configurations via a database.  
Thus, RAT-PAC is a complete package that can be used with small modifications for entire experiments.




\subsubsection{Machine Learning Approaches}

    The applications of machine learning approaches to neutrino detectors in general, and to photon-based neutrino detectors in particular, is enormous.  For photon detectors, these approaches fall into two primary classes: those that are used to create fast simulations, and those that are used for particle ID and background rejection.
    
    \paragraph{Generative Neural Nets}
    
\paragraph{KamNET}
    



\subsection{Prototypes and Large-Scale R\&D Platforms}
\subsubsection{ANNIE}
\label{sec:ANNIE}

The ANNIE (Accelerator Neutrino Neutron Interaction Experiment)~\cite{annieLOI,annie-results,pershingdiss} is located in the Booster Neutrino Beam at Fermilab. This beam is about 93\% pure $\nu_{\mu}$ in neutrino mode and has a spectrum that peaks at about 700 MeV, an energy scale of great interest to current and future neutrino oscillation experiments. While ANNIE's current Phase 2 investigates the combination of a Gd-loaded water target read out by ultrafast LAPPDs, a first insertion of a small WbLS-filled vessel (SANDI) is planned for the upcoming summer break, adding scintillation to the Cherenkov signal at the neutrino interaction vertex. In an eventual Phase 3, the full detection volume is to be filled with WbLS, making ANNIE the first experiment exploring the benefits of the new hybrid detection technique in the reconstruction of GeV-scale beam neutrinos.

\begin{figure}[t]
    \centering
   % \includegraphics[width=0.43\textwidth]{figs/ANNIE_P2.png}
    \includegraphics[width=0.225\textwidth]{figs/ANNIE_fisheye}
    \hfill
    \includegraphics[width=0.43\textwidth]{figs/ANNIE_feat_SANDI}
    \hfill
    \includegraphics[width=0.255\textwidth]{figs/ANNIE_SANDI_vessel}
    
    %\includegraphics[width=0.34\textwidth]{figs/ANNIE_First_Event.png}
    \caption{(left) NTT before installation. The rails allow LAPPDs to be inserted between the PMTs. (center) ANNIE detector setup with envisaged SANDI vessel containing 350\,kg of GdWbLS. (right) Test of SANDI acrylic vessel wrapped in protective plastics at UC Davis.} 
    \label{fig:ANNIE}
\end{figure}
\medskip

\medskip
\noindent{\bf ANNIE program with Gd-water target:} The two main goals of the current ANNIE Phase 2 are the precision measurements of the neutron yield from neutrino interactions at the 1\,GeV scale, and a test of the effectiveness of Large Area Picosecond PhotoDetectors (LAPPDs) in a realistic physics environment (Sec.~\ref{sec:LAPPD}). As illustrated by Figure~\ref{fig:ANNIE}, the current setup of the ANNIE detector comprises a 26-ton Neutrino Target Tank (NTT) equipped with 128 conventional PMTs, a Front Muon Veto (FMV) to reject ``dirt'' muons, and a Muon Range Detector (MRD) to track and range out muons. The water of the NTT was loaded with a mass fraction of 0.1\% of gadolinium (GdS) in early 2019. In January 2021, ANNIE started to take physics data in this basic configuration, while the deployment of first LAPPDs is foreseen for early 2022. The aim is to install in total five LAPPDs before the end of Phase 2 to evaluate their impact on the reconstruction of CC interaction final states as well as vertex reconstruction of the low-energy signals of neutron capture on gadolinium. The conventional PMT array provides a vertex reconstruction of $\Delta r=38\;$cm for CC final-state muons. The full configuration including the LAPPDs and their sub-nanosecond timing is expected to substantially improve this vertex resolution to about $\Delta r=12\;$cm.
\medskip\\
\noindent{\bf Scintillator for ANNIE Neutron Detection Improvement (SANDI):} From simulation studies, we know that $-$ even in the presence of LAPPDs $-$ the vertex resolution suffers from the need to image the ring edge with the conventional PMT array. There is a timing degeneracy in single track particles that makes the vertex location parallel to the track entirely dependent on ring edge imaging. One way to improve on this is to use a slightly scintillating material as neutrino target, resulting in a comparatively small amount of isotropic light emitted from the vertex that can be separated from Cherenkov light by timing and topology. 

To explore the potential benefit for event reconstruction, ANNIE plans to insert a 3'$\times$3' cylindrical vessel (SANDI) containing about 350\,kg of gadolinium-loaded Water-based Liquid Scintillator (GdWbLS) into the center of the NTT water volume (Figure~\ref{fig:ANNIE}). In addition, one or more of the five LAPPDs may be moved to the backward hemisphere. A deployment of several weeks will allow us to confirm models for track reconstruction and to identify additional scintillation light emitted by the hadronic recoil at the vertex. First simulation studies show that the inclusion of this signal will indeed lead to an improvement in reconstruction capability. While the muon energy reconstruction is dominated by the information from the (unchanged) MRD, the additional information from the GdWbLS volume improves the neutrino energy reconstruction from ($\Delta E/E\sim15\%$ to $11\%$).  
\medskip\\
\noindent {\bf Future full GdWbLS phase:} Following a successful SANDI test, ANNIE plans to propose a Phase 3 that features a complete replacement of the Gd-water with GdWbLS. Neutron captures in GdWbLS feature a substantially increased light output (factor $\sim$3) compared to Gd-water, greatly improving neutron detection efficiency ($\to\,\geq90\%$) and spatial resolution for the capture vertex ($\to\,\sim40\,$cm). This will enhance not only the precision of neutron multiplicity measurements but also bears the chance to reconstruct the neutron energy spectrum by their capture position relative to the production vertex. A full calorimetric measurement of the cross-section (including vertex hadronic energy) may also be possible. 

With these ambitious goals in mind, ANNIE is investigating the possibility to reconstruct the inner part of the NTT to make it compatible with WbLS, including encapsulation of PMTs and other components, in addition to the first-ever deployment of a WbLS liquid recirculation system. Systems based on nanofiltration and phase separation technology are being developed for Eos and Theia (Sects.~\ref{sec:Eos} and \ref{sec:Theia}). ANNIE Phase 3 will be a significant step towards realization of hybrid optical detectors in addition to making neutron-inclusive neutrino cross-section measurements of unprecedented scope and quality. 

\subsubsection{NuDOT}
\label{sec:NuDot}
NuDot is a mid-scale prototype designed to demonstrate timing-based Cherenkov/scintillation separation in a realistic experimental geometry, focusing on techniques applicable to searches for neutrinoless double-beta decay ($0\nu\beta\beta$). It builds on the successful demonstration of this approach in the FlatDot test stand~\cite{flatdot}. It is currently undergoing detector commissioning, with its initial physics data-taking campaign expected to begin by Summer 2022. 

\begin{figure}[]
    \centering
    \includegraphics[width=\textwidth]{figs/NuDot.png} %\hspace{5mm}
    \caption{\textit{From left to right:} A RAT-PAC simulation of electron tracks in the collimated $\beta$ source and coupled liquid scintillator cuvette used for ``dry" surface data-taking; a RAT-PAC simulation of Cherenkov light tracks for a 1\,MeV $\beta$ in NuDot; a rendering of a section view of the NuDot detector; a photo of NuDot, before the calibration system was deployed and the sphere was made light-tight for commissioning runs.}
    \label{fig:NuDot}
\end{figure}

The NuDot design, shown in Fig.~\ref{fig:NuDot}, relies on a combination of 59 8"-diameter PMTs (primarily a combination of EMI Model D642 and Hamamatsu Model R1408 PMTs previously used by the MACRO experiment) and 151 2"-diameter PMTs (Hamamatsu Module R13089, with an average transit time spread of 200\,ps) to achieve high light collection efficiency and fast-timing capability. These detectors surround a 36"-diameter acrylic sphere that will be filled with a LAB-based liquid scintillator cocktail, with the entire assembly immersed in a mineral oil tank to provide shielding and optical coupling. Detector calibration and the first two phases of data-taking will be conducted using a remotely-controlled $4\pi$ calibration system with 3 independent axes of motion. In addition to an LED source used for gain and pulse-shape calibrations, this system holds a collimated $\beta$-emitting $^{90}$Sr needle source that can be adjusted to shine on any point on the NuDot sphere from any point along the sphere diameter, allowing tests of the NuDot Cherenkov/scintillation separation capability as a function of position and direction. 

NuDot has 3 planned phases of operation, the first two of which are conducted prior to underground deployment:

\begin{enumerate}
    \item ``Dry" runs at Bates Research and Engineering Center: a small cuvette of liquid is coupled directly to the collimated source, allowing for calibration of the PMT timing response and pulse shape with water Cherenkov data, followed by C/s separation tests with a variety of liquid scintillator cocktails.
    \item Liquid scintillator- and mineral-oil-filled runs at Triangle Universities Nuclear Laboratories: following the completion of phase 1 data taking, NuDot will be moved to TUNL for any needed detector upgrades and liquid-filling. The goal of this phase is to demonstrate NuDot's C/s separation and energy reconstruction capability in the final operational configuration using the calibration system. 
    \item Underground proof-of-concept measurement: in phase 3, NuDot will be re-deployed underground for a proof-of-concept measurement. The current baseline is to conduct a $2\nu\beta\beta$ decay measurement, but alternatives like $\beta + $/EC searches are under consideration.
\end{enumerate}
The isotope and isotope-loading technique that will be used in phase 3 has not yet been selected. The NuDot Collaboration is currently conducting R\&D measurements of quantum-dot-loaded liquid scintillator cocktails that use perovskite wavelength shifters (see Ref.~\cite{perovskite}), but is also considering high-concentration Te loading and pressurized Xe loading options.

As described in Section~\ref{sec:KamNet}, the novel spatiotemporal neural network model KamNet has the ability to maximally extract information based on event topology in spherical LS detectors. We plan to leverage KamNet to achieve various analysis goals in NuDot including event tagging, position/directionality reconstruction and Cherenkov/Scintillation separation.

\subsubsection{Eos}
    \label{sec:Eos}

Successful detection of Cherenkov light from highly scintillating media has been achieved in CHESS, and complemented with an extensive characterisation program at LBNL, BNL, LLNL, and Davis.  These measurements inform large-scale Monte Carlo models, which are used to predict performance in kton-scale detectors. Ton-scale deployments of novel scintillators (ANNIE, BNL) are planned to test production, deployment, and recirculation.  

While bench-top measurements have been, and will continue to be used to measure microphysical properties of novel scintillators and photon detection technology, all demonstrations of event reconstruction and the resulting background rejection capabilities are purely Monte Carlo driven.  Data-driven demonstrations of the event imaging capabilities of hybrid detector technology is a critical step to realising a large detector for both fundamental physics and nonproliferation applications.

The proposed \eos prototype is a few-ton scale detector, designed to hold a range of novel scintillators, coupled with an array of photon detection options and the ability to deploy a range of low-energy calibration sources.  \eos will be constructed, calibrated and tested in Berkeley.  Assuming a successful surface deployment,  \eos could later be re-deployed underground, for example at SURF or SNOLAB, or at an alternative off-site location such as a reactor or test beam for further characterization of detector response to a range of particle interactions. \eos represents significant risk reduction for a large-scale deployment of (Wb)LS and novel detection technology.

\eos will be sufficiently large to use time-of-flight based reconstruction, and to fully contain a range of low-energy events ($\alpha$, $\beta$, $\gamma$, n) for detailed event-level characterisation.  \eos represents a balance of sufficient size for full event characterization, complemented with economy of scale, and flexibility to adapt for multiple target materials and photon detection options.

The primary goal of \eos is to validate performance predictions for large-scale hybrid neutrino detectors by performing a data-driven demonstration of low-energy event reconstruction leveraging both Cherenkov and scintillation light simultaneously.  By comparing data to model predictions, and allowing certain detector configuration parameters to vary -- such as the fraction of LS in a WbLS target cocktail, or by using PMTs with differing TTS, or deployment of dichroicons -- the predictive power of the model can be validated.  This validated microphysical model of hybrid neutrino detectors can then be used by the neutrino community for design optimization of next-generation hybrid detectors.

 \eos will provide an important test bed to the community, for testing alternative target media, photon detectors, and readout technology and methodology, and assessing the impact of these novel developments on detector performance.  
 
After the conclusion of operations at LBNL, \eos could be redeployed at an off-site location.  This would take place after the end of the primary project period, and successful completion of the project objective. Options include:
\begin{itemize}
\item Underground deployment, for example at SURF or SNOLAB, where scintillator handling procedures are well vetted and understood, and we have relationships of long standing.  This would allow more precise measurements in a low-background environment.
\item Deployment at a reactor for low-energy neutrino reconstruction.  This provides a near-field demonstration of the remote reactor monitoring concept.
\item Deployment at a test beam for hadronic event reconstruction, or a neutron source such as the Spallation Neutron Source at ORNL for neutron studies, useful for advanced event identification and background characterization.
\end{itemize}


%\subsection{New and Novel Detector Ideas}





\newpage

\section{Low-Threshold Neutrino Detectors}

\subsection{Common challenges of low-energy neutrino detectors}

This section will be part of the panel discussion 'energy bins' at the NF workshop at ONRL.  
We will collect the different approaches of  experimental efforts in the field of low-energy neutrino detection concering  1) improving resolution, 2) reducing backgrounds 3) increasing target mass and 4) understanding detector response. The final version of section 4.1 will give a comprehensive picture of the community efforts to exploit the low energy neutrino frontier. 

The following sections 4.2 - 4.4 will give a full overview of the running and planned low threshold neutrino  experiments, as well as describe the R\&D projects from submitted LOIs. Currently it consists of text section from SNOWMASS White papers, which will be shortened significantly for the final version. 

\subsubsection{Improving resolution and threshold}

Presentation of different approaches and  discussion in the "energy bin $<$1MeV" panel discussion. 

\subsubsection{Understanding and rejecting backgrounds}
Presentation of different techniques for background reduction in the "energy bin $<$1MeV" panel discussion. 

\subsubsection{Increasing target mass and detector scalability}
Presentation of different approaches to scale up taarget mass and number of readout channels in the "energy bin $<$1MeV" panel discussion. 
\subsubsection{Understanding low-energy detector response}
Presentation of calibration techniques to understand the (sub-)keV energy response of neutrino detectors in the "energy bin $<$1MeV" panel discussion. 


\subsection{The eV frontier of neutrino detectors}
\subsubsection{Cryogenic particle detectors for CEvNS}
%MINER, RICOCHET, NUCLEUS 
%BullKIDS, KIDs, MMC microcalometry, carbon detectors
\bigskip
\noindent 
\underline{MINER}: The Mitchell Institute Neutrino Experiment at Reactor (MI$\nu$ER) experiment was launched to use cryogenic germanium and silicon detectors with a low nuclear recoil energy thresholds to register nuclear recoils of coherent elastic neutrino-nucleus scattering (CE$\nu$NS) at a TRIGA research nuclear reactor at the Texas A\&M University~\cite{Agnolet:2016zir}. This reactor has a movable core (1\,m to 10\,m) that will allow precision studies of very short baseline neutrino oscillation by comparing rates as a function of distance and largely eliminating reactor flux uncertainties. Close proximity of the detector to the reactor core, combined with multiple low threshold detectors with event-by-event discrimination between the dominant electromagnetic background and the nuclear recoil signal provides sensitivity to BSM physics, sterile neutrinos that oscillate away on a few-meter scale, and above all a highly sensitive probe for applied reactor monitoring for safeguards and non-proliferation. Planned deployment of the MIN$\nu$ER experimental set up at the South Texas Project (3 GW) power reactor will provide significant further improvement in measurement sensitivity. 


\bigskip
\noindent 
\underline{NUCLEUS}: The NUCLEUS experiment aims for a detection of CE$\nu$NS using CaWO$_4$ cryogenic calorimeters with nuclear recoil thresholds around 20~eV. This unique feature demonstrated in an early prototype~\cite{Strauss:2017cuu,Strauss:2017cam,Angloher:2017sxg} will allow observation of the majority of tungsten recoils induced by reactor antineutrinos by accessing unprecedentedly low energies, taking full advantage of the coherent cross-section boost. The first experimental phase will deploy a 10~g cryogenic target~\cite{Rothe:2019aii} composed of approximately 6~g CaWO$_4$ and 4~g Al$_2$O$_3$ in a new experimental location~\cite{Angloher:2019flc} at the Chooz nuclear power plant in France. The two target materials feature widely different CE$\nu$NS cross-sections but a comparable neutron response, useful for in-situ measurement of potentially dangerous nuclear-recoil backgrounds.\\ 
The experimental setup will consist of a dry dilution refrigerator, a compact passive shielding made of neutron moderators and lead, active muon~\cite{Wagner:2022iqf} and gamma anticoincidence veto detectors as well as an integrated LED-based calibration system. The setup is under construction for commissioning in Munich in 2022 before deployment at the reactor site planned from 2023 on. 

\bigskip
\noindent 
\underline{Ricochet}: The Ricochet neutrino experiment aims to measure neutrinos produced from nuclear reactors by using cryogenic bolometers to identify the signature nuclear recoil from CE$\nu$NS~\cite{Ricochet:2021rjo}.  In order to overcome the high level of electromagnetic background present at low energies, Ricochet will make use of particle identification in order to discriminate between electron and nuclear recoils.  

The future Ricochet experiment will be deployed at the ILL-H7 site in Grenoble, France. The H7 site starts at about 8~m from the ILL reactor core that provides a nominal nuclear power of 58.3~MW, leading to a neutrino flux at the Ricochet{} detectors 8.8~m from the reactor core of about 1.2$\times$10$^{12}$~cm$^{-2}$s$^{-1}$. %The reactor is operated in cycles of typically 50 days duration with reactor-off periods sufficiently long to measure reactor-independent backgrounds, such as internal radioactivity or cosmogenic induced backgrounds with high statistics.  It is located below a water channel providing about \SI{15}{\m} water equivalent (m.w.e.) against cosmic radiation. It is not fed by a neutron beam and is well-shielded against irradiation from the reactor and neighboring instruments (IN20 and D19). The site is well-characterized in terms of backgrounds, and the operation of the STEREO neutrino experiment at this site has been successfully demonstrated~\cite{STEREO:2018blj}.

The experiment will make use of two detector technologies/targets.
The CryoCube will consist of an array of 27 ($3\times3\times3$) high purity germanium crystal detectors, encapsulated in a radio-pure infrared-tight copper box suspended below a lead shield inside the crysotat~\cite{RICOCHET:2021gkf}. %Each detector mass is about 38\,g to reach a total target mass around one kilogram. A low-energy threshold is desired as the discovery potential scales exponentially with lowering the energy threshold. Considering a 50\,eV energy threshold, about 12.8\,evts/kg/day of CE$\nu$NS\xspace interactions is expected in the CryoCube detector array.
%To reach such threshold, the CryoCube detectors will be equipped with germanium neutron transmutation doped sensors (NTD). To achieve particle identification, the detectors will have a double heat and ionization readout. Ionization measurement is realized thanks to aluminum electrodes allowing to apply an electric field and collect signals from the ionization electron-hole pairs drifting across the crystal. With an anticipated particle identification threshold of about 100\,eV, thanks to the combination of a 10\,eV and 20\,eVee (electron-equivalent) heat and ionization baseline resolutions (RMS), the CryoCube detector array should lead to a CE$\nu$NS\xspace detection significance after one ILL reactor cycle (50-days) between 4.3--17.3~$\sigma$, depending on the final background level achieved.

Q-Array -- the complimentary detector array within Ricochet -- will consist of 9 cubes of superconducting zinc cubes, each with a mass of about 35\,g, as its target. Using superconductors as the primary detector is a novel technology which is expected to provide detection sensitivity theoretically down to the Cooper pair binding energy.  The expected discrimination mechanism begins with the different efficiency of quasiparticle (QP) production (breaking Cooper pairs) by electron recoils (higher QP production) vs.~nuclear recoils (lower QP production). % The initial phonon production from the recoil is followed by a slower phonon production as QPs relax to the ground state.  The relative ratio between initial phonons and QP-induced phonons thereby gives rise to a usefully discriminating pulse shape.  Transition edge sensors (TES) will be used for the readout of the phonon signals from these superconducting bolometers. Initial prototype TES chips with a transition temperature of \SI{80}{\milli\K} were developed by Argonne National Laboratory for this use. Using results from these sensors, a second version was designed and fabricated, with a transition temperature of $\sim$20~mK. These devices are under testing~\cite{RanLTD} and a significant decrease in sensor threshold is expected. 

%A Hexa-Dry 200 Ultra-quiet cryostat from the CryoConcept Company, France, will be used to house the detector assembly. It is a dry cryogen-free cryostat with cold stages at \SI{50}{\K}, \SI{4}{\K}, \SI{1}{\K}, \SIlist{100;10}{\milli \K}, with the \SI{10}{\milli \K} stage designed to hold the detectors. The \SI{1}{\K} stage provides enough cooling power for the cold front-end electronics and also holds the cold shielding. Tests of the cryostat architechture has shown that this technology provides reduced vibration levels~\cite{Olivieri:2017lqz}, which is necessary for the optimal operation of the detectors. 

%The background level at the ILL site is expected to be high, due to the proximity to the nuclear reactor core ($\approx$8~meters), the neighboring experiments emitting large amounts of gammas and neutrons (IN20 and D19). Despite the presence of the $\approx$15 m.w.e. artificial overburden provided by the water transfer channel of the reactor directly above the experiment, the site remains exposed to cosmic radiation. As we expect to observe about 12.8 CE$\nu$NS\xspace events/kg/day, a highly efficient background mitigation strategy is mandatory. As a result, Ricochet aims for an electronic recoil background at the level of 100~events/day/keV/kg.  Such an electronic background level should be efficiently rejected thanks to our detectors' particle identification capabilities. However, as such discrimination doesn't hold for neutron induced nuclear recoil, the latter are expected to be our ultimate background. We are therefore aiming for a nuclear recoil background level around 5~events/kg/day to ensure a favorable CE$\nu$NS\xspace signal to noise ratio.  

%The Ricochet shielding will be divided into two parts: a \SI{300}{\K} outer shielding and a cold inner one (not shown). The outer passive shielding consists of \SI{20}{\cm} lead and \SI{35}{\cm} borated polyethylene. The cold inner shielding consists of \SI{13}{\cm} Pb/Cu and 8 layers of \SI{2.75}{\cm} polyethylene and 1~cm copper each.   Additionally, a third (external) \SI{35}{\cm} thick layer of polyethylene on top of the outer lead layer and \SI{8}{\mm} thick polyethylene layers mounted on each thermal screens will be used to reduce neutron spallation in the lead shielding and further improve the shielding tightness, respectively. The outer shielding will be made of three parts which will be installed on rails to allow accessing the cryostat. Lastly, muon induced gamma and neutron backgrounds will be further reduced thanks to a surrounding muon-veto allowing rejecting events in temporal coincidence with muons going through the experimental setup. 

Ricochet is currently scheduled to see ``first light" in 2023.




\subsubsection{CCD-based detectors for CEvNS}
%CONNIE, vIOLETTA

\bigskip
\noindent 
\underline{CONNIE}: The Coherent Neutrino-Nucleus Interaction Experiment (CONNIE) uses low-noise fully depleted charge-coupled devices (CCDs) with the goal of measuring low-energy recoils from CE$\nu$NS of reactor antineutrinos with silicon nuclei~\cite{Aguilar-Arevalo:2019jlr}. The CCD detectors  can operate at a nuclear recoil threshold of approximately 30 eV, where the conversion from electron equivalent to silicon recoil energy is given by the so-called quenching
factor, from which measurements at low energies ($\approx 0.7$ keV) and new theoretical approaches are used \cite{QFmeasurementsSi, QFtheorynew, Sarkis2021}.

\par CONNIE has reported results from its analysis with a detector array of 8 CCDs with a fiducial mass of 36.2 g, and a total exposure of 2.2 kg-days. In an analysis of the difference between the reactor-on and reactor-off spectra, no excess events are found at low energies, yielding upper limits at 95\% confidence level on the~CE$\nu$NS~rate. In the lowest-energy range analyzed by CONNIE, $50-180$ eV, the expected limit is 34 (39) times the standard model prediction, depending on whether the Sarkis or the Chavarria quenching factor is assumed. The CE$\nu$NS limits from CONNIE are shown in Figure~\ref{fig:connie}. 

\bigskip
\noindent 
\underline{vIOLETTA}:
\textit{to be added}

\subsubsection{Detectors for neutrino mass}
%ECHO, HELMES, several LOIs

\bigskip
\noindent 
\underline{ECHO}:
\textit{to be added}

\bigskip
\noindent 
\underline{HOLMES}:
\textit{to be added}

\bigskip
\noindent 
\underline{LOIs subitted on the topic}:
\textit{to be added}


\subsubsection{Future detectors for relic neutrinos}
\bigskip
\noindent 
\underline{PTOLEMY}:
\textit{to be added}

\subsubsection{New detector concepts}
\begin{itemize}
\item Paleo detectors


Paleo-detectors use the nuclear damage tracks recorded in natural minerals over geological time-scales to detect weakly-interacting particles over exposures much larger than what is feasible in conventional terrestrial detectors \cite{Baum:2018tfw,Drukier:2018pdy}. Unlike conventional experiments which measure nuclear recoils in real time, paleo-detectors measure the number of events integrated over the age of the mineral, reaching up to a billion years for minerals routinely found on Earth. The sources of the keV-scale nuclear recoils which can be recovered as tracks is rich, including atmospheric neutrinos \cite{Jordan:2020gxx}, solar neutrinos \cite{Tapia-Arellano:2021cml}, supernova neutrinos \cite{Baum:2019fqm}, as well as dark matter \cite{Baum:2021jak,Baum:2021chx}. Low-energy neutrino and dark matter tracks are initiated dominantly via CE$\nu$NS (quasi-elastic charged-current interactions are more applicable for high-energy neutrinos). 


\item Passive detectors
%Color centers, lattive dislocations

The PALEOCCENE concept~\cite{Cogswell:2021qlq} offers the potential for room-temperature, passive and robust detectors in the gram to kilogram range for the detection of low-energy nuclear recoil events. Nuclear recoil events can be caused by neutron scattering, coherent elastic neutrino nucleus scattering (CEvNS) or dark matter scattering and therefore, PALEOCCENE could find applications in all three areas. Nuclear recoils result in damage to the crystal lattice and some of these damage sites can become optically active, so-called color centers. The formation energy for these damage sites is in the range of a few tens of electronvolt and sets the intrinsic nuclear recoil detection threshold. In order to be sensitive to rare low-energy events optical detection of the fluorescence of single color centers in bulk volumes is envisaged by using so-called light sheet microscopy. Color centers are known to occur in a wide range of materials and thus, it appears plausible that a range of materials could be suitable for the PALEOECCENE approach. A multi-disciplinary collaboration of experts in particle, solid state and nuclear physics, as well as dark matter detection and nuclear engineering has started an R\&D program to investigate the feasibility of this concept.
\textit{to be continued}

\item Snowball detectors
%Metastable water
\item Directional detectors for low-energy neutrino physics
%CYGNUS, ArgonTPC, 

\bigskip
\noindent 
\underline{DRIFT}: 
The goal of the Directional Recoil Identification From Tracks (DRIFT) collaboration was the detection of a directional signal from Weakly Interacting Massive Particle (WIMP), halo, dark matter~\cite{PhysRevD.61.101301}. In order to accomplish this goal a unique, low-pressure, Negative Ion Time Projection Chamber (NITPC) technology was developed. The negative-ion drift allowed DRIFT NITPCs to have the lowest energy threshold and best inherent directional sensitivity of any limit-setting, directional dark matter detector. In addition, all of DRIFT's recent limits have been background-free. As a consequence, DRIFT's sensitivity to dark matter is almost 1,000 times better than other directional WIMP detectors~\cite{battat2017low}.
\textit{to be continued}

\bigskip
\noindent 
\underline{CYGNUS}: 
CYGNUS is a proposed modular and multi-site network of large-scale gas time projection chambers~\cite{Vahsen:2020pzb}. The primary goal of the CYGNUS experiment is to perform a direction-dependent search for dark matter, which has been shown to be one of the only ways to convincingly prove the galactic origin of a detected signal~\cite{Mayet:2016zxu,Vahsen:2021gnb}. Directionality is also the best means of circumventing the neutrino fog~\cite{Grothaus:2014hja,OHare:2015utx}, but requires that good performance can be achieved at the sub-10-keV nuclear recoil energies where the majority of CE$\nu$NS events coming from solar neutrinos would lie. 
\textit{to be continued}

\bigskip
\noindent 
\underline{LOI on ArgonTPC}: 


\end{itemize}


\subsection{Optimized conventional detectors to exploit CEvNS}
\subsubsection{HPGe detectors }
%CONUS, nuGEN, TEXONO, etc. 

\bigskip
\noindent 
\underline{CONUS}: The CONUS (COherent elastic Neutrino nUcleus Scattering) experiment employs four 1\,kg low energy threshold high-purity point-contact Germanium detectors to look for CE$\nu$NS. The experiment is located at the commercial nuclear power plant of Brokdorf, Germany, in a distance of 17.1\,m from the reactor core with a maximum thermal power of 3.9\,GW. With the electrically cooled spectrometers an energy resolution of 150-160eV (ionization energy, full width at half maximum ionization energy) at the 10.4\,keV K-shell X-ray of $^{71}$Ge/$^{68}$Ge is achieved \cite{bonet2021large}. The energy threshold is $\leq$1.875\,keV for nuclear recoils. With the onion-like shield consisting of layers of lead, borated polyethylene and a muon anti-coincidence veto a background level of $\sim$10\,counts/kg/d below 1\,keV ionization energy is achieved at reactor site \cite{bonet2021full}.
With the data collected in 2018 and 2019 an upper limit on CE$\nu$NS was derived in dependence of the quenching factor (ratio between detected ionization energy and recoil energy) in germanium \cite{bonet2021constraints}. For a quenching factor of k=0.16, this corresponds to a limit of 0.34\,kgd$^{-1}$ at 90\% confidence level (factor 17 above the standard model prediction). From the same data, limits on various BSM models \cite{CONUS:2021dwh} as well as the neutrino magnetic moment (from neutrino electron scattering) \cite{bonet2022first} were evaluated. With the data collected afterwards significant improvements on these limits are expected.
The quenching factor for germanium at low recoil energies is not well known and large discrepancies between the existing measurements persist. Recently, the CONUS collaboration carried out an own quenching measurement \cite{bonhomme2022direct} to significantly reduce this major systematic uncertainty. 
The final data collection run started in 2021 with several upgrades enhancing the sensitivity for a CE$\nu$NS detection. Significant improvements on the stability of the environment parameters were achieved. For the first time pulse shape information are collected as well with the intent to discriminate signals from background. The nuclear power plant shut down permanently at the beginning of 2022, which provides the opportunity to reduce the statistical uncertainty and improve the background understanding.

\bigskip
\noindent 
\underline{Dresden}: The experiment consists of a low-noise 3 kg p-type point contact germanium detector which has been installed and operated at the Dresden-II power reactor, near Chicago, at about 10 meters from its 2.96 GW$_{th}$ core~\cite{Colaresi:2021kus}. The detector are enclosed by a compact shielding made of several layers of active vetos and passive shielding material. The results from an upgraded setup suggest a preference for a CE$\nu$NS component in the data, when being compared to a background only model~\cite{Colaresi:2022obx}.

\bigskip
\noindent 
\underline{nuGen}: The nuGEN experiment aims at the detection of CE$\nu$NS with low-background, low-threshold HPGe detectors installed at a distance of $\sim10$\,m to one of the 3.1\,GW$_{th}$ reactors at the Kalinin Nuclear Power Plant (KNPP) in Russia. The detectors are surrounded by a compact passive shielding and an active muon veto, which are installed on a movable platform to modify the distance to the reactor core. nuGEN has been installed on-site in 2019 and preliminary data from first science runs have been presented~\cite{nuGEN_mag7}. 

\bigskip
\noindent 
\underline{TEXONO}:



\subsubsection{Scintillation detectors }
%CsI, NaI, Neon, 

\underline{NEON}: The Neutrino Elastic-scattering Observation on NaI(Tl) (NEON) experiment uses high-light yield NaI(Tl) crystals to observe the CE$\nu$NS events at a distance of 24\,m from the core of the Hanbit nuclear reactor in Korea. 
Commercial reactors produce a large number of anti-neutrinos with a thermal power of 2.8\,GW, and the on-going NEOS sterile neutrino program~\cite{Ko:2016owz} provides a systematic understanding of the environment.
\textit{to be continued}


\bigskip
\noindent 
\underline{several LOIs on the topic}:


\subsubsection{Bubble chambers  }

\bigskip
\noindent 
\underline{LOI Xe bubble chambers}

\subsubsection{Gaseous detectors }
\bigskip
\noindent 
\underline{NEWS-G}:

\subsubsection{Liquid noble gas detectors}


\bigskip
\noindent 
\underline{RED-100}: RED-100 is a two-phase xenon emission detector built to observe the coherent elastic scattering of reactor electron antineutrinos off xenon atomic nuclei~\cite{Akimov:2017hee}. The mass of the detector medium is 160 kg in the sensitive volume, and about 100 kg in the fiducial volume --- the largest value among detectors developed for CE$\nu$NS observations at reactors. The capability of detector full-scale operation in the background conditions caused by cosmic radiation has been demonstrated in a ground-level laboratory~\cite{Akimov:2019ogx}. The detector was deployed at the Kalinin NPP in 2021 at 19~m distance under the 3~GW reactor core (50~m.w.e. overburden) and acquired both reactor on and off data in January and February of 2022 with an energy threshold of about 1~keV$_{nr}$.

\subsection{Dark Matter detectors for next-generation neutrino measurements}

As described above, neutrinos from the astrophysical sources like the Sun and supernovae as well as from the atmospheric cosmic-ray-showers produce nuclear recoils via CE$\nu$NS, leading to signals in future dark matter detectors. 
The eventual presence of an unshieldable background in multiton-scale dark matter detectors has been anticipated for some time~\cite{Cabrera:1984rr,Drukier:1986tm,Monroe:2007xp,Vergados:2008jp,Strigari:2009bq,Gutlein:2010tq,Gelmini:2018ogy}, and is thought to present a major obstacle for improving the sensitivity of these experiments. The central problem is that for many of the most commonly sought-after dark matter models produce nuclear recoil signals that look remarkably similar to the CE$\nu$NS recoil energy spectra generated by natural neutrino sources. Due to the finite systematic uncertainty on the fluxes of those sources eventually a feeble-enough DM signal could disappear under the expected variation in the neutrino event rate, and because its signal would not be distinct enough from the background no positive identification of dark matter would be possible. Naively this implies that there is a ``floor'' to the sensitivity of direct detection experiments~\cite{Billard:2013qya}. 

%Since the dark matter and CE$\nu$NS signals are not exactly identical--- it is not impossible to search for dark matter in the presence of a CE$\nu$NS background, but it does entail significant reduction in experiment's sensitivity. This observation has been called ``neutrino fog''~\cite{OHare:2021utq}. One approach for visualising the nature of this fog is shown in the left-hand panel of Fig.~\ref{fig:8BXenon}, where the color displayed encodes the ``opacity'' of the neutrino fog in different parts of the spin-independent DM-nucleon cross section parameter space. One can appreciate here that major sources of neutrino that need to be understood better to aid the search for dark matter are $^7$Be, $^8$B and atmospheric neutrinos, as the height of this fog in cross section is crucially dependent on the size of the systematic uncertainty on those fluxes~\cite{Ruppin:2014bra}. Neutrino floor considerations play an important role when considering the feasibility of future experiments, as decreased sensitivity to DM signals in vicinity of neutrino background also hinder the increase in experimental sensitivity with scaling in detector exposure~(e.g.~\cite{Dent:2016wor,Gelmini:2018ogy}). There are several approaches for circumventing the neutrino floor if an experiment can access additional information to further discriminate the dark matter signal and neutrino background, including the use of annual modulation~\cite{Davis:2014ama}, target complementarity~\cite{Ruppin:2014bra,Gelmini:2018ogy,Gaspert:2021gyj,OHare:2020lva}, and directionality~\cite{OHare:2015utx,Grothaus:2014hja,Mayet:2016zxu,OHare:2017rag,Franarin:2016ppr,Vahsen:2020pzb,Vahsen:2021gnb,Sassi:2021umf}. It should also be emphasized that any additional uncertainties in the neutrino signals~\cite{OHare:2016pjy,AristizabalSierra:2017joc,Gonzalez-Garcia:2018dep,Papoulias:2018uzy,AristizabalSierra:2021kht} beyond the systematic uncertainties on the flux will raise the height of the neutrino fog. Since the signals of different types of dark matter-nucleus interactions do not identically align with the CE$\nu$NS signal, depending on the scenario the neutrino fog could be much lower, or absent entirely~\cite{Dent:2016iht, Dent:2016wor,Gelmini:2018ogy,Essig:2018tss,Wyenberg:2018eyv}. For example, inelastic dark matter scattering that could be naturally associated with models of multi-component dark sectors could help lift the signal degeneracy of the neutrino floor~\cite{Gelmini:2018ogy}.

%Many upcoming experiments will be sensitive to CE$\nu$NS and are expected to enter the neutrino fog, such as XENONnT~\citep{aprile2020projected}, LZ~\citep{akerib2020projected} and DARWIN~\citep{Aalbers:2016jon,Aalbers:2022dzr}. Here we discuss the several experiments that will be sensitive to~\cevns~in the forthcoming years. 
%Solar neutriinos and source measurements
\subsubsection{Multi-ton liquid noble detectors}

\bigskip
\noindent 
\underline{XENON}: 
The XENON1T experiment operated a dual-phase time projection chamber (TPC) filled with 3.2 tonnes of ultra-pure liquid xenon (LXe). The TPC contained 2.0 tonnes of LXe that is sensitive to ionization electrons (S2) and scintillation photons (S1) produced by interactions therein. In a fiducial volume with 1.0 tonnes of LXe, a background level down to $(76\pm2)\,\mathrm{events}/(\mathrm{tonne}\times\mathrm{year}\times\mathrm{keV})$ has been achieved.
\textit{to be continued}

\bigskip
\noindent 
\underline{LUX-ZEPLIN}: 
LUX-ZEPLIN (LZ) is a dual-phase xenon TPC with a 7-tonne active mass located 1 mile underground at the Sanford Underground Research Facility (SURF) in Lead, South Dakota. %The experiment is currently on commissioning. %Although t
The LZ detector was designed to search for interactions of particle dark matter in the mass range from 1 GeV/c$^2$ to 10 TeV/c$^2$.
Because the CE$\nu$NS process can produce low-energy nuclear recoil signals  similar to those produced by low-mass WIMPs, 
LZ will also be sensitive to 
%Coherent Elastic neutrino-nucleus scattering (\cevns) for neutrinos of energies at the MeV-GeV scale. The \cevns in LZ produce low-energy nuclear recoil signature identical to WIMPs at the keV scale. Two main prospective natural sources of 
astrophysical sources of neutrinos such as solar $^8$B neutrinos and atmospheric neutrinos. Over the full 15.34 tonne-year exposure, LZ is expected to observe 0.65 events from atmospheric neutrinos and 36 events from $^8$B neutrino %under a projected detector condition 
in its WIMP search campaigns~\citep{akerib2020projected}.
\textit{to be continued}


\bigskip
\noindent 
\underline{DARWIN}: 
DARWIN (DARk matter WImp search with liquid xenoN) is a proposed next-generation dark matter experiment that will operate 50\,t (40\,t active) of xenon in a cylindrical time projection chamber with 2.6\,m in diameter and height~\cite{Aalbers:2022dzr}. The TPC will be placed in a double-walled cryostat vessel surrounded by neutron and muon vetoes. While DARWIN's primary goal is to observe particle dark matter in the $\sim$1\,GeV-100\,TeV mass range, it will also be able to measure the solar $^{8}$B neutrino flux, as well as atmospheric and supernovae neutrinos via CE$\nu$NS.\textit{to be continued}

\bigskip
\noindent 
\underline{DarkSide}: 



\subsubsection{Large-scale cryogenic detectors}

\bigskip
\noindent 
\underline{SuperCMDS}:


\bigskip
\noindent 
\underline{CRESST-III}: 


\bigskip
\noindent 
\underline{EDELWEISS}: 


\bigskip
\noindent 
\underline{RES-NOVA}: 
RES-NOVA is a newly proposed experiment for the detection of neutrinos from astrophysical sources~\cite{Pattavina:2020cqc}. RES-NOVA will employ an array of archaeological Pb-based cryogenic detectors sensitive to SN neutrino emission from the entire Milky Way Galaxy. Its modular design will be suited for the detection of nearby SN explosions ($<$3~kpc)~\cite{RES-NOVA:2021gqp}.





\newpage
\section{Next-Generation and Novel Large-Scale Detector Ideas}

\subsection{Theia}
New developments in liquid scintillators, high-efficiency, fast photon detectors, and chromatic photon sorting have opened up the possibility for building a large-scale detector that can discriminate between Cherenkov and scintillation signals. Such a detector could exploit these two distinct signals to observe particle direction and species using Cherenkov light while also having the excellent energy resolution and low threshold of a scintillator detector. Situated in a deep underground laboratory, and utilizing new techniques in computing and reconstruction techniques, such a detector could achieve unprecedented levels of background rejection, thus enabling a rich physics program that would span topics in nuclear, high-energy, and astrophysics, and across a dynamic range from hundreds of keV to many GeV. The scientific program would include observations of low- and high-energy solar neutrinos, determination of neutrino mass ordering and measurement of the neutrino CP violating phase $\delta$, observations of diffuse supernova neutrinos and neutrinos from a supernova burst, sensitive searches for nucleon decay and, ultimately, a search for NeutrinoLess Double Beta Decay (NLDBD) with sensitivity reaching the normal ordering regime of neutrino mass phase space.

\theia is a detector concept that incorporates these new technologies in a practical and affordable way to accomplish the science goals described above. We consider two scenarios, one in which \theia would reside in a cavern the size and shape of the caverns intended to be excavated for the Deep Underground Neutrino Experiment (DUNE) which we call \theia-25, and a larger 100 ktonne version (\theia-100) that could achieve an even broader and more sensitive scientific program.

    \begin{figure}[htp!]
\centering
\includegraphics[width=0.95\textwidth]{figs/theia25_surf}
\includegraphics[width=0.36\textwidth]{figs/theia25_int.png}
\includegraphics[width=0.26\textwidth]{figs/theia100_ext.png}
\includegraphics[width=0.36\textwidth]{figs/theia100_int.png}
\caption{The \theia detector.  
{\it Top  panel:} \theia-25 sited in the planned fourth DUNE cavern; 
{\it Lower left panel:} an interior view of \theia-25 modeled using the Chroma optical simulation package~\cite{chroma}; 
{\it Lower middle panel:} exterior view of \theia-100 in Chroma;
{\it Lower right panel:} an interior view of \theia-100 in Chroma.  In all cases, \theia has been modelled with 86\% coverage using standard 10-inch PMTs, and 4\% coverage with LAPPDs, uniformly distributed, for  illustrative purposes.  Taken from~\cite{theiawp}.}
\label{f:detector}
\end{figure}

In the \textsc{Theia} reference design, the target material would be water-based liquid scintillator (WbLS) described  in Section~\ref{sec:wbls}, which has an advantage for a big detector in its  long attenuation lengths. For much of the low-energy program of \textsc{Theia}, the WbLS would need to be made radiopure at levels not far from what can be done in an organic scintillator.   %The \textsc{Theia} white paper examined two possible geometries, shown in Figure~\ref{fig:theia}: a large (100 ktonne fiducial) right-cylinder, and a smaller (25 ktonne fiducial) letterbox-shaped detector, which could fit inside a cavern like that being built as part of LBNF.   
    

The broadband neutrino beam being built for the Long Baseline Neutrino Facility (LBNF)
~\cite{lbnf} and the Deep Underground Neutrino Experiment (DUNE)~\cite{dunecdr} offers an opportunity for world-leading long-baseline neutrino oscillation measurements. Due to advances in Cherenkov ring reconstruction techniques, a \theia detector in the LBNF beam would have good sensitivity to neutrino oscillation parameters, including CP violation (CPV), with a relatively modestly-sized detector. 
In addition to this long-baseline neutrino program, \theia will also contribute to atmospheric neutrino measurements and searches for nucleon decay, particularly in the difficult $p\rightarrow K^+ + \overline{\nu}$ and $N\rightarrow 3\nu$ modes.


	\theia will also make a definitive measurement of the solar CNO neutrinos,
which have recently been detected exclusively by Borexino~\cite{bxcno}, but without enough precision to distinguish between competing models of the Sun's metallicity.
\theia will also provide a high-statistics, low-threshold ($\sim$ 3~MeV)
measurement of the shape of the $^8$B solar neutrinos and thus search for new
physics in the MSW-vacuum transition region~\cite{friedland2004, minakata2012}. Antineutrinos produced in the
crust and mantle of the Earth will be measured precisely by \theia with statistical uncertainly far exceeding all detectors to date. %\theia will measure the 
%antineutrinos from distant nuclear reactors. 

Should a supernova occur during
\theia  operations, a high-statistics detection of the $\bar{\nu}_e$ flux will be
made---literally complementary to the  detection of the $\nu_e$ flux in the DUNE liquid argon
detectors. The simultaneous detection of both messengers---and detection of an optical, x-ray, or gamma ray component will enable a great wealth of neutrino physics
and supernova astrophysics. With a very deep location and with the detection of a combination of scintillation and Cherenkov light, \theia will have world-leading sensitivity to make a detection of the Diffuse Supernova Neutrino Background (DSNB) antineutrino flux. The most ambitious goal,
which would likely come in a future phase, is a search for Neutrinoless double beta decay (NLDBD), with a total isotopic mass of 10 tonnes or more, and with decay lifetime sensitivity in excess of $10^{28}$ years~\cite{theiawp, biller_normal}.


\theia is able to achieve this broad range of physics by exploiting new
technologies to act simultaneously as a (low-energy) scintillation detector and
a (high-energy) Cherenkov detector. Scintillation light provides the energy
resolution necessary to get above the majority of radioactive backgrounds and
provides the ability to see slow-moving recoils; Cherenkov light enables event
direction reconstruction which provides particle ID at high energies and
background discrimination at low-energies. Thus, the scientific program benefits in many cases on
the ability of \theia to discriminate efficiently and precisely between the ``scintons'' (scintillator photons)
and ``chertons'' (Cherenkov photons). 

    A major advantage of \theia is that the target can be modified in a phased program to address the science priorities. In addition, since a major cost of \theia is expected to be photosensors, investments in \textsc{Theia25} instrumentation can be transferred directly over to \textsc{Theia100}. Thus, \theia can be realized in phases, with an initial phase consisting of lightly-doped scintillator and very fast photosensors, followed by a second phase with enhanced photon detection to enable a very low energy solar neutrino program, followed by a third phase that could include doping with a $0\nu\beta\beta$ isotope and perhaps an internal containment vessel. %Table~\ref{tbl:phases} lists the primary physics targets and the general configuration required to achieve those physics goals for each phase.


\subsection{LiquidO}

LiquidO is a new approach to detecting neutrinos that, in contrast with conventional liquid scintillator detectors, relies on using an opaque scintillator medium as the primary neutrino target~\cite{Cabrera:2019kxi}. The scintillators that can be best used by LiquidO have a short scattering length and a medium to long absorption length, an example of which has already been successfully produced~\cite{Buck:2019tsa}. In such a medium, the photons produced by the opaque scintillator undergo a random walk process near their creation point and are trapped in so-called {\it light balls} around each energy deposition point. The light is collected by a dense array of wavelength-shifting fibres that traverses the volume and that is readout by photo-sensors in the periphery. Silicon photomultipliers (SiPMs) are well-suited to this purpose given their affordable price, high efficiency, and excellent time resolution. 

\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.90\textwidth]{./figs/LiquidO1.png}  
%\includegraphics[width=0.38\textwidth]{./JUNO_Spectrum_Cropped.pdf} 
\caption{\label{fig:lozfig} Left: energy depositions of a simulated 1~MeV kinetic energy positron in a LiquidO detector with a regular 1~cm fibre pitch running along the $z$ direction. Panel (a) shows the $x$-$y$ projection, while panel (b) shows the full three-dimensional extent. The fibres are represented in green. Right: true number of photons hitting the fibres, each of which is represented by a pixel, in the opaque and transparent scintillator scenarios. In the former case, the scintillator is assumed to have a 5~mm scattering length and a 5~m absorption length. Figure obtained from Ref.~\cite{Cabrera:2019kxi}.}
\end{center}
\end{figure}

%\begin{wrapfigure}{R}{0cm}
\begin{figure}
%    \centering
    \includegraphics[width=8cm]{./figs/LiquidO2.png}
    \caption{Simulated 2~MeV gamma (left) and electron (right) in the same detector configuration of Fig.~\ref{fig:lozfig}. Figure obtained from Ref.~\cite{Cabrera:2019kxi}.
    \label{fig:gammaelectron}}
\end{figure}
%\end{wrapfigure}

A full description of LiquidO, its expected performance, first experimental demonstration, and potential applications, can be found in Ref.~\cite{Cabrera:2019kxi}. Fig.~\ref{fig:lozfig} illustrates LiquidO's performance using a simulated positron with 1~MeV of kinetic energy. Here, the simplest configuration with fibres running only along one direction ($z$) is assumed. The true energy depositions of the positron are shown on the left panels, with (a) showing the $x$-$y$ projection and (b) the full three-dimensional extent. Panel (c) shows the number of true photons hitting each fibre in a 1-cm-pitch lattice when a scintillator with a 5~mm scattering length is used. The positron's loss of kinetic energy produces a light-ball at the vertex of the event. The two back-to-back gamma-rays resulting from its annihilation lose energy via Compton scattering, leaving two trails of smaller light balls that detach from the central one. A comparison is made in panel (d) of the light pattern collected by the same fibre array when using a transparent scintillator. Despite the use of fibres, the event topology is almost entirely washed out, illustrating the key role played by the scintillator's opacity in self-segmenting the detector.

The clear event topology of $\sim$MeV positrons in LiquidO stands in contrast with that of other events, as illustrated in Fig.~\ref{fig:gammaelectron}. At these energies, gammas lose their energy primarily via the Compton effect and produce trails of light balls over many tens of cm, whereas electrons produce single light balls. At higher energies (more than $\sim$10~MeV for electrons), charged particles have enough kinetic energy to travel several cm or more in the detector, producing sequences of point-like energy depositions that form clear tracks. As a result, many other interactions, from cosmic ray muons to charged and neutral current neutrino interactions of various energies, could also be precisely reconstructed in LiquidO. In this way, this detector technology combines some of the advantages of conventional liquid scintillator detectors with those of tracking detectors.


\subsection{ArTEMIS}

Distinguishing Cherenkov and scintillation (C/S) photons is challenging in organic liquid scintillators because the short-wavelength end of the Cherenkov spectrum, where most of the photons reside, is buried by the more intense scintillation spectrum.  In contrast, liquid Ar (LAr) scintillates narrowly around 128 nm, leaving the broad Cherenkov spectrum isolated above this wavelength, which is readily detected by common devices such as PMTs.  The scintillation photons can be detected with the same devices upon coating their photosensitive surface with a wavelength shifter like PTB.  
The narrow range of scintillation photons ensures that the uncoated PMTs see purely Cherenkov light.  This pure sample of Cherenkov photons can be used to cleanly reconstruct the position, direction, and energy of events from several MeV and above, depending on the PMT photocoverage and efficiency.  The photons detected by the TPB-coated PMTs would be primarily from scintillation due to its far greater yield and could be used to independently reconstruct the position and energy of events as low as a few MeV.  Using both photon samples together would provide more robust particle ID and reconstruction. 


Relative to liquid Ar time projection chambers like those proposed for DUNE, this type of detector would provide the same particle interaction channels while requiring simpler hardware (no charge readout) and event analysis (like a scintillator or Cherenkov detector).  Collaborators at Penn and Berkeley are studying the capabilities of a LAr detector to distinguish C/S photons.  GPU-accelerated simulations of a large liquid Ar detector with TPB-coated and -uncoated PMTs is performed using the Chroma package and pyrat wrapper.

\subsection{SLIPs}

The construction of large-scale liquid scintillator detectors is complicated by the need to separate the scintillation region from photomultiplier tubes (PMTs) due to their intrinsic radioactivity. This is generally done using acrylic and/or nylon barriers, whose own intrinsic activity can also lead to substantial cuts to the fiducial detection volume for a number of low energy (~MeV) studies. Such barrier constructions also become increasingly difficult and expensive for larger detector volumes, with JUNO already pushing the boundaries of what might be achievable. The SLIPS concept is to do away with such physical barriers entirely by instead mounting PMTs on the bottom of a wide cavity and covering them with a distillable, lipophobic liquid, above which a less dense scintillator is layered. Liquids such as various ethylene glycols are good candidates for the bottom layer as they provide a good refractive index match to a number of liquid scintillator solvents. Thin, opaque and highly reflective (>90\%) surfaces are used near the top and side areas of the detector to provide a buffer region against radioactivity from the walls and to reflect scintillation light back to the bottom PMT array, where the time-separated reflected signals are used to reconstruct the 3D vertex position as well as the event energy. A conceptual design can be seen in Figure~\ref{fig:SLIPS1}. Initial simulation studies indicate that good position and energy reconstruction can be achieved with this approach. The notion is to use a shallow layer of scintillator relative to the cavity width, where the vertical depth of scintillator is chosen to be much less than the optical absorption length and can be optimised to balance fiducial volume, light level and reconstruction accuracy.

\begin{figure}[htp]
\centering 
\includegraphics[width=0.9\textwidth]{figs/SLIPS1.pdf} 
\caption{SLIPS design. Left - cross-sectional side view; right - top view.} 
\label{fig:SLIPS1}
\end{figure}

%\begin{figure}[htp]
%\centering 
%\includegraphics[width=0.5\textwidth]{figs/SLIPS2.pdf} 
%\caption{Simplified analytical model of the relative fraction of produced light detected vs extinction length/scintillator depth ratio.} 
%\label{fig:SLIPS2}
%\end{figure}


Initial simulations have been carried out assuming a densely packed array of R5912-100 HQE PMTs in a pillbox-shaped detector with a diameter of 50m, an ethylene glycol layer extending 2m above the PMTs, a scintillator layer composed of LAB + 2g/L PPO, and 90\% specular reflective surfaces. Figure \ref{fig:SLIPS3} shows the resulting number of detected photons from a 1 MeV electron as a function of event position for vertical scintillator heights of both 5m and 10m. These correspond to fiducial volumes of $\sim$8kT and 16kT, respectively. 

\begin{figure}[htp]
\centering 
\includegraphics[width=0.9\textwidth]{figs/SLIPS3.pdf} 
\caption{Detected number of photoelectrons for a 1 MeV electron for the simulated configuration as a function of $\rho$ (cylindrical radius from the centre of the detector) and $z$ (vertical height relative to the centre of the scintillator layer). The left plot is for a scintillator layer height of 5m and the right is for a height of 10m.} 
\label{fig:SLIPS3}
\end{figure}

%Figure \ref{fig:SLIPS4} shows timing and spatial distributions of PMT hits for an individual 3 MeV electron at different locations in the scintillator volume of 10m height. Distinctive reflection peaks and correlations with the spatial position can be clearly seen. Hit density distributions in the x-y plane are also particularly distinct for this geometric configuration and can be also used to provide good localisation. Initial studies suggest a position resolution comparable to that achieved by current conventional LS detectors.

%\begin{figure}[htp]
%\centering 
%\includegraphics[width=0.9\textwidth]{figs/SLIPS4.pdf} 
%\caption{Relative times of PMT hits vs PMT y coordinate for a 3 MeV electron generated at different positions within a scintillator volume of height 10m.} 
%\label{fig:SLIPS4}
%\end{figure}


\subsection{Deuterium Bubble Chambers}

    For neutrino interaction studies.
    
\subsection{Project8}

    Novel approach to measuring tritium endpoint for absolute neutrino mass.
    
    
\subsection{Detectors for the Forward Physics Facility at the LHC}    

\subsection{Space-Based Neutrino Detection}
Neutrino spacecraft





\bibliographystyle{hieeetr}
\bibliography{refs}

\end{document}


